Automating Model Comparison in Factor Graphs

Bayesian state and parameter estimation have been automated effectively in a variety of probabilistic programming languages. The process of model comparison on the other hand, which still requires error-prone and time-consuming manual derivations, is often overlooked despite its importance. This paper efficiently automates Bayesian model averaging, selection, and combination by message passing on a Forney-style factor graph with a custom mixture node. Parameter and state inference, and model comparison can then be executed simultaneously using message passing with scale factors. This approach shortens the model design cycle and allows for the straightforward extension to hierarchical and temporal model priors to accommodate for modeling complicated time-varying processes.

==> content/archive/01-introduction.tex <==


% In this paper, we make Bayesian model comparison techniques more accessible, by efficiently automating them using message passing-based probabilistic inference.
% Specifically, we construct a mixture model out of the models that we wish to compare and perform probabilistic inference in this model through message passing \cite{loeliger_factor_2007} with scale factors \cite[Ch.6]{reller_state-space_2013}, \cite{nguyen_efficient_2022}.
% Importantly, instead of treating probabilistic inference and model comparison as two separate processes, we treat them as a single automatable message passing procedure on a single probabilistic model.
% Benefiting from the modularity and extensibility of the used factor graphs, the model prior $p(m)$ can straightforwardly be extended into a hierarchical dynamical model, leading to a novel class of model comparison algorithms.

% Next to this approach, \cite{minka_gates_2008} has introduced the concept of "gates", which allow for the specification of mixture models that submit to message passing-based inference. \bdv{not clear in phrasing how this relates to MC.}
% Despite the universality of their approach, gates include functional dependencies, such as conditional probability distributions, which might be undesirable if these are unavailable. \bdv{also a bit unclear.}
% Furthermore, their models do not support exact inference but instead rely on variational inference \cite{winn_variational_2004, winn_variational_2005, dauwels_variational_2007} and expectation propagation \cite{minka_expectation_2001}.
% As a result, the mixture selection variable is only updated based on the local contributions to the model performance, disregarding the performance contributions of the rest of the models.
% Only taking into account local contributions can be very sensitive to the initialization of the inference algorithm, which has the potential to yield suboptimal inference results.

% This mechanism is different from the "pick"-factors in \cite{minka_gates_2008} as we perform model comparison based on the model evidence of the entire acyclic graph and not just on a local contribution. 


% \bdv{Here the introduction breaks from establishing the Problem to stekching Solution proposal. At this point you should have explained the problem, why it is interesting (why MC is interesting has not been explained, only that it is "ubiquitous"), and why it is important (because both gates and Kamary's "mixture model estimation" (KMME) have issues). You should say at this point what is your concrete Problem Statement. Then continue in next paragraph with sketch of our Solution Proposal.}



==> content/archive/03-factorgraphs.tex <==
% \section{Factor graphs and message passing} 
% Factor graphs are a class of probabilistic graphical models.
% Here we use Forney-style factor graphs as introduced in \cite{forney_codes_2001} with notational conventions adopted from \cite{loeliger_introduction_2004} to visualize our models.
% Forney-style factor graphs are undirected graphical models that visualize the factorization of a function as a graph, where nodes and edges represent factors and variables, respectively.
% An edge connects to a node only if the variable associated with the edge is an argument of the function associated with the node.
% For a more thorough review of factor graphs, we refer the interested reader to \cite{loeliger_introduction_2004, loeliger_factor_2007}.

% Probabilistic inference concerns calculating marginal distributions in the probabilistic model.
% The calculation of the marginal distribution of some variable requires integration over all nuisance variables in the model.
% Because of the factorization in the model, this global integration can be performed by smaller localized computations, which summarize parts of the model.
% The results of these computations are called messages and are propagated over the edges of the graph.
% The sum-product message $\vec{\mu}_{s_j}(s_j)$ \cite{kschischang_factor_2001} flowing out of some node $f(s_1, s_2, \ldots, s_K)$ with incoming messages $\vec{\mu}_{s_k}(s_k)$, where $s_k \in s_{\backslash j}$, is given by 
% \begin{equation}
%     \vec{\mu}_{s_j}(s_j) = \int f(s_1, s_2, \ldots, s_K) \prod_{k \neq j } \vec{\mu}_{s_k}(s_k) \ \mathrm{d}s_{\backslash j}.
% \end{equation}
% We represent the edges by arbitrarily directed arrows in order to distinguish between forward and backward messages propagating in or against the direction of an edge $s_j$ as $\vec{\mu}_{s_j}(s_j)$ and $\cev{\mu}_{s_j}(s_j)$, respectively.
% For common factor-message pairs, these messages have been derived in \cite[Ch.6]{reller_state-space_2013} and \cite{nguyen_efficient_2022}.

% Importantly, in contrast to other works in literature, the scaling of the messages is not neglected.
% Therefore, a message $\vec{\mu}_{s_j}(s_j)$ can be decomposed as
% \begin{equation}
%     \vec{\mu}_{s_j}(s_j) = \vec{\beta}_{s_j} \, \vec{p}_{s_j}(s_j),
% \end{equation}
% where $\vec{p}_{s_j}(s_j)$ denotes the probability distribution representing the normalized functional form of the message $\vec{\mu}_{s_j}(s_j)$. 
% The term $\vec{\beta}_{s_j}$ denotes the scaling of the message $\vec{\mu}_{s_j}(s_j)$ and is also known as a scale factor.

% From the colliding messages the marginal distributions $p(s_j\midi D)$ and the model evidence $p(D)$ can be jointly computed at any edge in the graph as in \cite[Ch.6]{reller_state-space_2013} and \cite{nguyen_efficient_2022} according to
% \begin{equation}
%     p(s_j \midi D) \, p(D) = \vec{\mu}_{s_j}(s_j) \, \cev{\mu}_{s_j}(s_j).
% \end{equation}
% The model evidence can be identified as the scaling of the joint distribution $p(s_j, D)$, because $p(s_j\midi D)$ itself is normalized, as
% \begin{equation} 
%     p(D) = \int \vec{\mu}_{s_j}(s_j) \, \cev{\mu}_{s_j}(s_j) \, \mathrm{d}s_j .
% \end{equation}


% \subsection{Constrained Bethe free energy} 
% Probabilistic inference in a single model $f(\bm{s})$ involves computing the model evidence and the posterior distribution over the variables $\bm{s}$.
% The posterior distribution $p(\bm{s})$ of model $f(\bm{s})$ in \eqref{eq:ffg} can be found as
% \begin{equation} 
%     p(\bm{s}) = \frac{f(\bm{s})}{Z},
% \end{equation}
% where the normalization constant or model evidence $Z$ is defined as $Z=\int f(\bm{s})\mathrm{d}\bm{s}$\footnote{Integrals are taken over the support over the variables. If a variable is discrete-valued, integral operators will be replaced with summation operators. For a consistent exposition of our work, we use integral operators throughout the paper.}. \bdv{This is not wrong, just a bit awkward way of presenting the problem. You skip over the fact that the model $f(\bm{s})$ is factorized as prior times likelihood, which must be transferred to the factorization posterior times evidence. }

% In practice, however, the computation of this normalization constant and therefore the posterior distribution is intractable.
% Variational inference provides a generalized view that supports probabilistic inference in these types of models by approximating the exact \bdv{true = Bayes-optimal?}\bart{Addressed, rephrased} posterior $p(\bm{s})$ by a variational posterior $q(\bm{s})$ that is constrained to be within a family of distributions $q\in \mathcal{Q}$.
% Variational inference optimizes (the parameters of) the variational distribution $q(\bm{s})$ by minimizing the variational free energy (VFE) defined as
% \begin{equation} 
%     \mathrm{F}[q, f] = \mathbb{E}_{q(\bm{s})} \left[ \ln \frac{q(\bm{s})}{f(\bm{s})} \right] = \mathrm{KL}\left[q(\bm{s}) \,\|\, p(\bm{s})\right] - \log Z
% \end{equation}
% through for example coordinate or stochastic gradient descent. \bdv{... or by any other means. It does not have to be coordinate or stochastic gradient descent.}\bart{Addressed, rephrased}

% In practice, the variational posterior $q(\bm{s})$ is often factorized for tractability.
% A versatile factorization of $q(\bm{s})$ is the Bethe factorization \cite{yedidia_bethe_2001}, defined in an FFG \bdv{only in a terminated FFG, you'll have to explain in the previous section what a TFFG is.} by
% \begin{equation}
%     q(\bm{s}) = \prod_{a \in \mathcal{V}} q_a(\bm{s}_a) \prod_{i \in \mathcal{E}} q_i(s_i)^{-1},
% \end{equation}
% which factorizes the variational posterior as the product of node-local joint posterior distributions, in which overlapping contributions between nodes are compensated for. \bdv{huh?}
% This specific factorization decomposes the VFE into the sum of node-local free energy contributions and edge-specific (differential) entropies $\mathrm{H}$, which is better known as the Bethe free energy (BFE) \citetemp{ref}
% \begin{equation}
%     \mathrm{F}_\mathrm{B}[q,f] = - \sum_{a\in\mathcal{V}}\mathbb{E}_{q_a(\bm{s}_a)}\left[\ln f_a(\bm{s}_a)\right] - \sum_{a\in\mathcal{V}}\mathrm{H}[q_a(\bm{a}_a)] + \sum_{i\in\mathcal{E}}\mathrm{H}[q_i(s_i)],
% \end{equation}
% This factorization approximates the VFE and equals the VFE for tree-structured graphs containing no cycles. \bdv{\eqref{eq:Bethe-constraint} does not necessarily lead to a normalized distribution so I think you should always add the normalization, marginalization and consistency constraints before introducing the BFE.}

% The Bethe free energy provides a universal objective for performing probabilistic inference \cite{senoz_variational_2021}.
% Optimization of \eqref{eq:bfe} with respect to $q_a(\bm{s}_a)$ and $q_i(s_i)$ leads to variational posteriors which approximate the exact posteriors and to a Bethe free energy that more closely bounds the model evidence as in \eqref{eq:vfe}.
% Importantly, by adding constraints to the BFE functional, a variety of inference algorithms can be recovered \cite{senoz_variational_2021}.
% As an example consider the case where we wish to optimize the BFE and would like the marginal distributions to satisfy the normalization and marginalization conditions
% \begin{subequations}
% \begin{align}
% 
%         \int q_a(\bm{s}_a) \diff \bm{s}_a &= 1,   &&\forall\, a \in \mathcal{V} \\
% 
%         \int q_a(\bm{s}_a) \diff \bm{s}_{a\backslash i} &= q_i(s_i). &&\forall\, a\in\mathcal{V}, i\in\mathcal{E}(a)
% \end{align}
% \end{subequations}
% \bdv{I dont think these constraints are examples, but rather they are an essential part of BFE def. Examples of additional constraints are form and factorization constraints.}
% When both constraints are active, normalization of the edge-specific marginals $q_i(s_i)$ is implied.
% These conditions can be enforced during optimization of the BFE by constructing the Lagrangian or CBFE functional
% \begin{equation} 
%     \mathrm{L}[q,f] = \mathrm{F}_\mathrm{B}[q,f] + \sum_{a \in \mathcal{V}} \psi_a\left(\int q_a(\bm{s}_a) \diff \bm{s}_a - 1\right) + \sum_{a\in\mathcal{V}} \sum_{i\in\mathcal{E}(a)} \int \lambda_{ai}(s_i) \left(\int q_a(\bm{s}_a) \diff \bm{s}_{a\backslash i} - q_i(s_i)\right) \diff s_i,
% \end{equation}
% with Lagrange multipliers $\psi_a$ and $\lambda_{ai}(s_i)$.
% With these specific constraints, optimization of this specific CBFE functional recovers the celebrated sum-product (belief propagation) algorithm \cite{senoz_variational_2021} \cite{pearl_reverend_1982, kschischang_factor_2001}.
% Additional constraints give rise to different inference algorithms, such as variational message passing \cite{winn_variational_2005, dauwels_variational_2007} and expectation propagation \cite{minka_expectation_2001}.
% By combining different local constraints hybrid inference schemes can be obtained.
% We highly recommend the interested reader to \cite{senoz_variational_2021} for an overview of these local constraints and their implications for the resulting inference algorithm.


% After reviewing factor graphs in Section~\ref{sec:methods:factorgraphs}, the remainder of this section can be read from two complementary perspectives.
% The bottom-up perspective, comprising Sections~\ref{sec:methods:CBFE} and \ref{sec:methods:constraints}, derives model comparison by message passing from first principles based on a CBFE minimization procedure.
% The top-down perspective, comprising Section \ref{sec:methods:scalefactors}, shows how Bayes' rule for model comparison in \eqref{eq:bayes} can be interpreted as a message passing procedure using scale factors \cite[Ch.6]{reller_state-space_2013}, \cite{nguyen_efficient_2022}, which aligns with the outcomes of the bottom-up perspective.


% This subsection will interpret the presented message passing update rules of Section~\ref{sec:methods:constraints} using scale factors, in the case where we restrict ourselves to exact inference in trees.
% Concretely, we will show that the previously derived update rules can also be derived from Bayes' rule in \eqref{eq:bayes} from a top-down perspective and illustrate how this can be efficiently realized using message passing with scale factors.
% Consequently, the process of model selection and posterior computations are unified under the efficient message passing framework.
% Before connecting these approaches, we will provide a brief review of sum-product message passing and introduce scale factors.

% Consider the global integration of the factorizable model $f(\bm{s})$ in \eqref{eq:ffg} over all variables except for $s_j$ as $\int f(\bm{s}) \diff \bm{s}_{\backslash j}$.
% This large global integration can be performed through a set of smaller local computations as a result of the assumed factorization of $f(\bm{s})$ in \eqref{eq:ffg}.
% These smaller local computations can be considered to summarize the parts of the graph that is being integrated over and are termed messages, which graphically can be interpreted to propagate over the edges in the graph
% These messages are denoted by $\mu$ and can be locally computed on the graph.
% The sum-product message $\vec{\mu}_{s_j}(s_j)$ flowing out of the node $f_a(s_1, s_2, \ldots, s_K)$ with incoming messages $\vec{\mu}_{s_k}(s_k)$ is given by \cite{kschischang_factor_2001}
% \begin{equation}
%     \vec{\mu}_{s_j}(s_j) = \int f_a(s_1, s_2, \ldots, s_K) \prod_{k \neq j } \vec{\mu}_{s_k}(s_k) \ \mathrm{d}\bm{s}_{\backslash j}.
% \end{equation}
% Derivations of this message passing update rule under the same CBFE minimization procedure from Section~\ref{sec:methods:CBFE} are presented in \cite{senoz_variational_2021}.
% We represent edges in the graph by arbitrarily directed arrows in order to distinguish between forward and backward messages propagating in or against the direction of an edge $s_j$ as $\vec{\mu}_{s_j}(s_j)$ and $\cev{\mu}_{s_j}(s_j)$, respectively.
% Following this approach, the global integration reduces to the product of the messages of the variable of interest as $\int f(\bm{s}) \mathrm{d}\bm{s}_{\backslash j} = \vec{\mu}_{s_j}(s_j) \cev{\mu}_{s_j}(s_j)$ for acyclic models.

% The previously discussed integration $\int f(\bm{s}) \diff \bm{s}_j$ can be represented differently through substitution of \eqref{eq:posterior} as
% \begin{equation}
%     \int f(\bm{s}) \diff \bm{s}_{\backslash j} = Z \int p(\bm{s}) \diff \bm{s}_{\backslash j} = Z p(s_j),
% \end{equation}
% where $p(s_j)$ is the marginal distribution of $s_j$.
% The implications of this result are significant: the product of two colliding messages $\vec{\mu}_{s_j}(s_j) \cev{\mu}_{s_j}(s_j)$ results in the scaled marginal distribution $Z p(s_j)$.
% Because of the normalization property of $p(s_j)$ it is possible to obtain both the normalized posterior $p(s_j)$ as the model evidence or normalization constant $Z$ on any edge in the graph.
% What enables this computation is the scaling of the messages resulting from the equality in \eqref{eq:methods:sp}.
% As a result, the messages $\vec{\mu}_{s_j}(s_j)$ can be decomposed as 
% \begin{equation}
%     \vec{\mu}_{s_j}(s_j) = \vec{\beta}_{s_j} \vec{p}_{s_j}(s_j),
% \end{equation}
% where $\vec{p}_{s_j}(s_j)$ denotes the probability distribution representing the normalized functional form of the message $\vec{\mu}_{s_j}(s_j)$. 
% The term $\vec{\beta}_{s_j}$ denotes the scaling of the message $\vec{\mu}_{s_j}(s_j)$, also known as the scale factor.
% Scale factors can be interpreted as local summaries of the model evidence  that are passed along the graph.

% Consider one of the models on the left of Figure~\ref{fig:models}.
% If these models are acyclic and submit to exact inference, then the model evidence for each model, i.e. $Z_k = p(\mathcal{D} \midi m=\bm{e}_k)$ in \eqref{eq:bayes}, can be computed on all edges, but also around all nodes.
% This means that for each of the different combinations $y \times \{x_1, x_2,\ldots, x_K\}$ on the right of Figure~\ref{fig:models}, representing the different models, the model evidence can be computed using scale factors.
% As a result, the model evidence $p(D \midi m)$ in \eqref{eq:bayes} can be represented as
% \begin{equation}
%     p(D\midi m) = \prod_{k=1}^K\left(\int \vec{\mu}_{x_k}(x_k) f_k(y, x_k) \cev{\mu}_y(y)\right)^{m_k},
% \end{equation}
% whose functional form can be recognized as a scaled categorical distribution.
% The model evidence term simultaneously resembles the backwards message $\cev{\mu}_m(m)$, containing the information about $m$ based on the data $D$.
% Similarly, the model prior $p(m)$ equals the forward message $\vec{\mu}_m(m)$, in the case that there is no hierarchical prior on $m$.
% From these observations, the product of the model posterior and marginal model evidence in Bayes' rule can be computed as 
% \begin{equation}
%     p(m \midi D) p(D) = \vec{\mu}_m(m) \prod_{k=1}^K \left(\int \vec{\mu}_{x_k}(x_k) f_k(y,x_k) \cev{\mu}_y(y)\right)^{m_k},
% \end{equation}
% where scale factors allow for exact computation of the model evidences of the distinct model combinations.

% \bart{Todo: Add connection to previous section}

% The choice of including the factors $f_k(y, x_k)$ inside the node of Figure~\ref{fig:models} might seem to be a restrictive choice.
% This namely would require having a hierarchical model, which might not always be the case.
% However, without loss of generality the factors can be assumed to be Dirac delta functions\footnote{Assuming continuous random variables. For discrete variables the Dirac delta function can be substituted for the Kronecker delta function.} as $f_k(y, x_k) = \delta(y - x_k)$, acting as an equality node that forces variables $y$ and $x_k$ to be equal.
% In practice, this choice creates a multiplexer node that switches between edges, whose simplified update rules are presented in Table~\ref{tab:node}.

% Commonly the VFE is further constrained by assuming a Bethe factorization over $q(\bm{s}_k \midi m_k)$, yielding the Bethe free energy, which equals the VFE for acyclic graphs.
% If phrased as a constrained Bethe free energy minimization procedure \cite{senoz_variational_2021}, we can recover a common message passing schemes, such as sum-product message passing or belief propagation, (structured) variational message passing, expectation maximization and may more depending the local factorization and functional form constraints over the approximate posterior distributions in the graph. \citetemp{add refs here}

% \begin{subequations}
%     \begin{equation}
%         \int q(\bm{s}_a \midi m_k) \diff \bm{s}_a = 1,
%     \end{equation}
%     \begin{equation}
%         \int q(\bm{s}_a \midi m_k) \diff \bm{s}_{a\backslash i} = q(s_i \midi m_k),
%     \end{equation}
% \end{subequations}



% \begin{equation}
%     q(m) = \frac{\vec{\mu}_m(m) \cev{\mu}_m(m)}{\int \vec{\mu}_m(m) \cev{\mu}_m(m) \diff m}
% \end{equation}


% \subsection{Conditional constraints}
% \bart{outdated subsection}
% In this section we will derive custom message passing update rules based on a new set of local BFE constraints.
% These update rules align with the process of model comparison and can be implemented efficiently using scale factors, as we will describe in Section~\ref{sec:methods:scalefactors}.
% Our approach combines a set of $K$ models into a single mixture model where the model indicator $m$ is treated as another variable inside our model that might itself include hierarchical or temporal dynamics.

% \begin{figure}[t]
%      \centering
%      \begin{subfigure}{0.45\linewidth}
%          \centering
%          \input{figures/models-separate.tikz}
%         
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}{0.45\linewidth}
%          \centering
%          \input{figures/models-joint.tikz}
%          
%      \end{subfigure}
%     \caption{(left) Overview of the traditional process of model comparison. Here inference is performed in a set of $K$ models after which the models are compared. These models may partially overlap in both variables as in structure. Specifically, in this example the variable $y$ and the model attached to the corresponding edge are identical for all models. On the contrary \bdv{In contrast, ...}, the nodes $f_k$, variables $x_k$ and attached model structures are assumed to differ between the different models. (right) \bdv{The right graph does not visualize that $m$ is the "selection" variable.} Our approach to model comparison based on message passing. The different models are combined into a single graph representing a mixture model, where the model selection variable $m$ specifies the component assignment. The nodes at the boundary of the identical and distinctive model structures are captured into a single composite node $f(y, \bm{x}, m)$ of \eqref{eq:comparisonfactor}. \bdv{to be precise, doesnt loeliger use the term composite node rather than compound node?}\bart{Addressed, yes you are right} \bdv{Isnt this very related to "Gates" by Minka? We should include a ref and explain relation.}}
%     
% \end{figure}

% Figure~\ref{fig:models} sketches the specific situation that we consider in this paper.
% We consider a set of $K$ tree-structured models, whose structures are partially identical.
% We furthermore assume that each of these models can be split into two disjoint model sections, which are connected by a single edge.
% One model section captures the model structure that is identical for all $K$ models, whereas the other section contains the remaining part of the model.
% This split allows for combining the identical sections into the single shared likelihood model of the mixture model.
% The distinctive model structures are then used as the component priors. 
% The categorization of the shared sections in terms of likelihood model and the distinctive parts as component priors has been made to aid understanding, but can be swapped without loss of generality.

% Consider the variable $y$ that is shared amongst all $K$ models.
% We assume that this variable $y$ is connected to the factor $f_k(y, x_k)$ depending on the model, indexed by $k$.
% The dependence on a single variable $x_k$ might seem restrictive, but we will show in Section~\ref{sec:methods:scalefactors} how this can be generalized to any model.
% From the distinctive factor nodes $f_k(y, x_k)$ that are connected to the shared variable $y$, a compound node can be created as in Figure~\ref{fig:models} that forms the core of the mixture model.
% This node function is specified as
% \begin{equation}
%     f(y, \bm{x}, m) = \prod_{k=1}^K f_k(y, x_k)^{m_k},
% \end{equation}
% where the model selection variable $m$ comprises a 1-of-$K$ binary vector with elements $m_k\in\{0, 1\}$ constrained by $\sum_{k=1}^K m_k = 1$.

% With the definition of this compound node, we will closely follow the optimization approach as stipulated in \cite{senoz_variational_2021} for deriving the new message passing update rules.
% The global optimization of \eqref{eq:bfe} over $q(\bm{s})$ is split into the local optimization of multiple interdependent local objectives.
% Specifically, we subdivide the entire model into separate node- and edge-induced subgraphs and optimize the local beliefs, i.e. $q_a(\bm{s}_a)$ or $q_i(s_i)$, over the related terms of \eqref{eq:bfe}.

% \begin{figure}
%      \centering
%      \begin{subfigure}{0.45\linewidth}
%          \centering
%          \input{figures/subgraph-node.tikz}
%          
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}{0.45\linewidth}
%          \centering
%          \input{figures/subgraph-edge.tikz}
%         
%      \end{subfigure}
%      \caption{(left) Example of a node-induced subgraph. (right) Example of an edge-induced subgraph.}
%      
% \end{figure}

% As a first step, consider an edge-induced subgraph as depicted in Figure~\ref{fig:subgraphs}.
% Optimization of $q_i(s_i)$ with respect to the relevant terms in \eqref{eq:bfe-lagrangian} leads to the local optimization problem involving the entropy of $q_i(s_i)$ and the relevant normalization and marginalization constraints from \eqref{eq:methods:constraints}.
% Functional optimization over $q_i(s_i)$ gives rise to the results depicted in the following lemma from \cite{senoz_variational_2021}:

% \begin{lemma}
% Given a terminated Forney-style factor graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, consider an edge-induced subgraph $\mathcal{G}(i)$. The stationary points of the Lagrangian \eqref{eq:bfe-lagrangian} as a functional of $q_i(s_i)$
% \begin{equation}
%     \mathrm{F}_i[q_i(s_i)] = \mathrm{H}[q_i(s_i)] + \psi_i \left[\int q_i(s_i) \diff s_i - 1\right] + \sum_{a \in \mathcal{V}(i)} \int \lambda_{ai}(s_i) \left[\int q_a(\bm{s}_a) \diff \bm{s}_{a\backslash i} - q_i(s_i)\right] \diff s_i + C_i,
% \end{equation}
% where $C_i$ collects all terms independent of $q_i(s_i)$, are of the form
% \begin{equation}
%      q_i(s_i) = \frac{\displaystyle\vec{\mu}_{s_i}(s_i) \cev{\mu}_{s_i}(s_i)}{\displaystyle\int \vec{\mu}_{s_i}(s_i) \cev{\mu}_{s_i}(s_i) \diff s_i}.
% \end{equation}
% \end{lemma}
% \begin{proof}
%     see \cite[Appendix D.2]{senoz_variational_2021}
% \end{proof}

% With these results, we will follow a similar approach for computing the joint variational posterior $q_a(y,\bm{x}, m)$ around the subgraph that is induced by the compound factor node $f(y, \bm{x}, m)$ in \eqref{eq:comparisonfactor} and Figure~\ref{fig:models}.
% Aside from the relevant terms of the BFE in \eqref{eq:bfe}, we add the normalization constraint
% \begin{equation}
%     \int q_a(y, \bm{x}, m) \diff y \diff \bm{x} \diff m = 1
% \end{equation}
% \bdv{$m$ is discrete, use sum.}
% to the local Langrangian, in addition to the marginalization constraints
% \begin{subequations}
%     \begin{equation}
%         \int q_a(y, \bm{x}, m) \diff y \diff \bm{x} = q(m),
%     \end{equation}
%     \begin{equation}
%         \int \lambda_y(y) \left(\int q_a(y, \bm{x}, m) \diff \bm{x} \diff m - q(y) \right) \diff y,
%     \end{equation}
%     \begin{equation}
%         \int \prod_{k=1}^K \left(\int \lambda_k(x_k) \left(\int q_a(y,\bm{x}, m) \diff y \diff \bm{x}_{\backslash k} - q(x_k) \right)\diff x_k\right)^{m_k} \diff m.
%     \end{equation}
% \end{subequations}

% The first and second marginalization constraints \eqref{eq:constraints:m} and \eqref{eq:constraints:y} do not deviate from the general structure in \eqref{eq:methods:constraints:marginalization}.
% However, the third marginalization constraint \eqref{eq:constraints:x} requires further explanation.
% Intuitively this constraint enforces that marginalization of $q_a(y,\bm{x},m)$ over $y$, $\bm{x}_{\backslash k}$ and $m$ yields the marginal distribution $q(x_k)$, for all possible model selection configurations $m$.
% Functional optimization of the relevant terms in \eqref{eq:bfe} combined with the constraints from \eqref{eq:constraints:node:normalization} and \eqref{eq:constraints:node:marginalization} leads to the following lemma:
% \bdv{Great approach! I really like how you derive the update equations formally through the CBFE framework. Gives it all a very solid foundation.}
% \begin{lemma}
% Given a terminated Forney-style factor graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, consider the node-induced subgraph $\mathcal{G}(a)$ with factor node function \eqref{eq:comparisonfactor} and variational joint posterior $q_a(y, \bm{x}, m)$. The stationary points of the Lagrangian 
% \begin{equation}
%     \begin{split}
%         \mathrm{L}_a[q_a, f] 
%         &= \mathbb{E}_{q_a(y, \bm{x},m)}\left[\ln\frac{q_a(y, \bm{x},m)}{f(y,\bm{x},m)}\right] + \psi \left(\int q_a(y, \bm{x}, m) \diff y \diff \bm{x} \diff m - 1 \right)\\
%         &\qquad + \int \lambda_m(m) \left(\int q_a(y, \bm{x}, m) \diff y \diff \bm{x} - q(m)\right)\diff m \\
%         &\qquad + \int \lambda_y(y) \left(\int q_a(y, \bm{x}, m) \diff \bm{x} \diff m - q(y) \right) \diff y \\
%         &\qquad + \int \prod_{k=1}^K \left(\int \lambda_k(x_k) \left(\int q_a(y,\bm{x}, m) \diff y \diff \bm{x}_{\backslash k} - q(x_k) \right)\diff x_k\right)^{m_k} \diff m + C_a,
%     \end{split}
% \end{equation}
% where $C_a$ collects all terms independent of $q_a(y, \bm{x}, m)$, are of the form
% \begin{equation} 
%     q_a(y, \bm{x}, m) = \frac{\displaystyle \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(\vec{\mu}_k(x_k) f_k(y,x_k)\big)^{m_k}}{\displaystyle \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(\vec{\mu}_k(x_k) f_k(y,x_k)\big)^{m_k} \diff y \diff \bm{x} \diff y}.
% \end{equation}
% \end{lemma}
% \begin{proof}
% See appendix {\color{red}{TODO}}
% \end{proof}





% \begin{theorem}
% Given a terminated Forney-style factor graph $\mathcal{G} = 
% (\mathcal{V}, \mathcal{E})$, consider the induced subgraph $\mathcal{G}(a,i)$. 
% The local stationary solutions are given by \eqref{eq:qi} and \eqref{eq:qa}, from which the messages towards $y$ can be determined as
% \begin{equation}
%     \vec{\mu}_y(y) \propto \sum_{k=1}^K \vec{\mu}_m(e_k) \int \vec{\mu}_{x_k}(x_k) f_k(y,x_k) \diff x_k.
% \end{equation}
% \end{theorem}

% \begin{theorem}
% Given a terminated Forney-style factor graph $\mathcal{G} = 
% (\mathcal{V}, \mathcal{E})$, consider the induced subgraph $\mathcal{G}(a,i)$. 
% The local stationary solutions are given by \eqref{eq:qi} and \eqref{eq:qa}, from which the messages towards $x_i$ can be determined as
% \begin{equation}
%     \vec{\mu}_{x_i}(x_i) = \vec{\mu}_m(e_i) \int f_i(y, x_i) \cev{\mu}_y(y) \diff y.
% \end{equation}
% \end{theorem}

% \begin{theorem}
% Given a terminated Forney-style factor graph $\mathcal{G} = 
% (\mathcal{V}, \mathcal{E})$, consider the induced subgraph $\mathcal{G}(a,i)$. 
% The local stationary solutions are given by \eqref{eq:qi} and \eqref{eq:qa}, from which the messages towards $m$ can be determined as
% \begin{equation}
%     \cev{\mu}_m(m) = \prod_{k=1}^K \left(\int \vec{\mu}_k(x_k) f_k(y,x_k) \cev{\mu}_y(y) \diff x_k \diff y\right)^{m_k}
% \end{equation}
% \end{theorem}

% Continuing the example of Section~\ref{sec:background:factorgraphs}, the marginal distribution $p(s_2\mid y=\hat{y})$ in the model described by \eqref{eq:ffg:example_factorization} can be computed as 
% \begin{equation}\label{eq:sum-product:example}
%     \begin{split}
%         p(s_2) 
%         &\propto \int f(s_1,s_2,s_3,s_4) \mathrm{d}s_{\backslash 2}, \\
%         &= \underbrace{\int \underbrace{f_a(s_1)}_{\vec{\mu}_{s_1}(s_1)} f_b(s_1,s_2)  \mathrm{d}s_1}_{\vec{\mu}_{s_2}(s_2)} \underbrace{\int \underbrace{f_c(s_3)}_{\cev{\mu}_{s_3}(s_3)} f_d(s_2,s_3,s_4)  \mathrm{d}s_3 \mathrm{d}s_4}_{\cev{\mu}_{s_2}(s_2)}.
%     \end{split}
% \end{equation}
% Here, the global integration is decomposed into the product of nested integrations, representing sum-product messages, as illustrated in Figure~\ref{fig:methods:example_ffg}.


% \subsection{Forney-style factor graphs} \label{sec:methods:factorgraphs}
% A factor graph is a specific type of probabilistic graphical model.
% Here we use the Forney-style factor graph (FFG) framework as introduced in \cite{forney_codes_2001} with notational conventions adopted from \cite{loeliger_introduction_2004} to visualize our models.
% An FFG can be used to represent a factorized function
% \begin{equation} \label{eq:ffg}
%     f(\bm{s}) =\prod_{a\in\mathcal{V}} f_a(\bm{s}_a),
% \end{equation}
% where $\bm{s}$ collects all variables in the function.
% The subset $\bm{s}_a \subseteq \bm{s}$ contains all argument variables of a single factor $f_a$.
% FFGs visualize the factorization of such a function as a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where nodes $\mathcal{V}$ and edges $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ represent factors and variables, respectively.
% An edge connects to a node only if the variable associated with the edge is an argument of the factor associated with the node.
% As an example consider the model $f(s_1,s_2,s_3,s_4)$ with factorization
% \begin{equation} \label{eq:ffg:example_factorization}
%     f(s_1,s_2,s_3,s_4) = f_a(s_1) f_b(s_1,s_2) f_c(s_3) f_d(s_2,s_3,s_4)
% \end{equation}
% The FFG representation of \eqref{eq:ffg:example_factorization} is shown in Fig.~\ref{fig:methods:example_ffg}.
% For a more thorough review of factor graphs, we refer the interested reader to \cite{loeliger_introduction_2004, loeliger_factor_2007}.

% \begin{figure}[t]
%     \centering
%     \input{figures/example_ffg.tikz}
%     \caption{A Forney-style factor graph representation of the factorized function in \eqref{eq:ffg:example_factorization}. The messages correspond to the terms in \eqref{eq:sum-product:example}.}
%     \label{fig:methods:example_ffg}
% \end{figure}

% % Throughout this paper, we will adopt the notational conventions as exposed in \cite{senoz_variational_2021}. \bdv{I don't think you use Ismail's notation for messages, which is more like Loeliger. From Ismail, you use the graph subset notation.} \bart{Indeed}
% Nodes are indexed by the variables $a$, $b$, and $c$, where edges are indexed by $i$, $j$, and $k$ unless stated otherwise.
% The set of edges connected to node $a\in\mathcal{V}$ is denoted by $\mathcal{E}(a)$ and the set of nodes connected to edge $i\in\mathcal{E}$ is referred to as $\mathcal{V}(i)$.

% In an FFG, nodes can be connected to an arbitrary amount of edges.
% However, edges are constrained to be connected to at most two nodes.
% For variables that are an argument in more than two factors, this constraint can be satisfied through the use of "equality" nodes.
% In an equality node with function $f(s_i, s_i^\prime, s_i^{\prime\prime}) = \delta(s_i - s_i^\prime)\delta(s_i - s_i^{\prime\prime})$, the belief over a variable $s_i$ is constrained to be equal to the beliefs over its variable copies $s_i^\prime$ and $s_i^{\prime\prime}$.
% By chaining together equality nodes a variable can be duplicated to an arbitrary number of nodes. 


% \subsection{Sum-product message passing} \label{sec:methods:sum-product}
% Probabilistic inference in the submodels $f_k$ and the overcoupling model containing the factor $f_m$ can be efficiently realized using message passing. \bdv{I would not mix a review of message passing with novelty about message passing over the one-hot variable $m$. Just discuss a short derivation of sum-product rule based on the graph in Fig.~\ref{fig:methods:example_ffg}.}
% Consider the global integration of the general factorizable model $f(\bm{s})$ in \eqref{eq:ffg} over all variables except for $s_j$ as $\int f(\bm{s}) \diff \bm{s}_{\backslash j}$.
% This large global integration can be performed through a set of smaller local computations as a result of the assumed factorization of $f(\bm{s})$ in \eqref{eq:ffg}.
% These smaller local computations can be considered to summarize the part of the graph that is being integrated over and are termed messages, which graphically can be interpreted to propagate over the edges in the graph.
% These messages are denoted by $\mu$ and can be locally computed on the graph.
% The sum-product message $\vec{\mu}_{s_j}(s_j)$ flowing out of the node $f_a(\bm{s}_a)$ with incoming messages $\vec{\mu}_{s_i}(s_i)$ is given by \cite{kschischang_factor_2001}
% \begin{equation}\label{eq:sp}
%     \vec{\mu}_{s_j}(s_j) = \int f_a(\bm{s}_a) \prod_{i \neq j } \vec{\mu}_{s_i}(s_i) \ \mathrm{d}\bm{s}_{a\backslash j}.
% \end{equation}
%  We represent edges in the graph by arbitrarily directed arrows in order to distinguish between forward and backward messages propagating in or against the direction of an edge $s_j$ as $\vec{\mu}_{s_j}(s_j)$ and $\cev{\mu}_{s_j}(s_j)$, respectively.
% Following this approach, the global integration reduces to the product of the messages of the variable of interest as $\int f(\bm{s}) \mathrm{d}\bm{s}_{\backslash j} = \vec{\mu}_{s_j}(s_j) \cev{\mu}_{s_j}(s_j)$ for acyclic models.
% Posterior distributions on edges and around nodes can then be computed according to
% \begin{equation}\label{eq:marginaledge}
%     q(s_j) = \frac{\vec{\mu}_{s_j}(s_j)\cev{\mu}_{s_j}(s_j)}{\displaystyle \int \vec{\mu}_{s_j}(s_j)\cev{\mu}_{s_j}(s_j) \diff s_j}
% \end{equation}
% and
% \begin{equation}\label{eq:marginalfactor}
%     q(\bm{s}_a) = \frac{\displaystyle f_a(\bm{s}_a) \prod_{i \in \mathcal{E}(a)} \vec{\mu}_{s_i}(s_i)}{\displaystyle \int f_a(\bm{s}_a) \prod_{i \in \mathcal{E}(a)} \vec{\mu}_{s_i}(s_i) \diff \bm{s}_a},
% \end{equation}
% respectively \cite{senoz_variational_2021}.

% Continuing the example of Section~\ref{sec:methods:factorgraphs}, the exact posterior distribution $p(s_2)$ in the model described by \eqref{eq:ffg:example_factorization} can be computed as 
% \begin{equation}\label{eq:sum-product:example}
%     \begin{split}
%         p(s_2) 
%         &\propto \int f(s_1,s_2,s_3,s_4) \mathrm{d}s_{\backslash 2}, \\
%         &= \underbrace{\int \underbrace{f_a(s_1)}_{\vec{\mu}_{s_1}(s_1)} f_b(s_1,s_2)  \mathrm{d}s_1}_{\vec{\mu}_{s_2}(s_2)} \underbrace{\int \underbrace{f_c(s_3)}_{\cev{\mu}_{s_3}(s_3)} f_d(s_2,s_3,s_4)  \mathrm{d}s_3 \mathrm{d}s_4}_{\cev{\mu}_{s_2}(s_2)}.
%     \end{split}
% \end{equation}
% Here, the global integration is decomposed into the product of nested integrations, representing sum-product messages, as illustrated in Figure~\ref{fig:methods:example_ffg}.
% \tvdl{With a picture in Sec.~\ref{sec:methods:factorgraphs} you could refer to it. Or even move the entire previous paragraph to that section and explain messages as resulting from the distributive rule.}\bart{Addressed}

% \tvdl{Perhaps start a new subsection on scaling factors here.}\bart{Addressed}
% Derivations of the message passing update rule in \eqref{eq:sp} by phrasing inference as a constrained Bethe free energy minimization procedure are presented in \cite{senoz_variational_2021}.
% Through a similar procedure one can obtain alternative message passing algorithms such as variational message passing \cite{winn_variational_2004, winn_variational_2005, dauwels_variational_2007}, expectation propagation \cite{minka_expectation_2001}, expectation maximization \cite{dauwels_ex

==> content/archive/04-averaging.tex <==
\section{Bayesian model averaging} \label{sec:averaging}
% Bayesian model averaging computes \eqref{eq:bayes} by determining the posterior probabilities of the 1-of-$K$ binary model selection vector $m = [m_1, m_2, \ldots, m_K]^\top$, with $m_k \in \{0, 1\}$ and $\sum_k m_k = 1$.
% As mentioned in the introduction, this operation is often decoupled from the inference procedure in the individual models.
% In this paper we will perform both operations jointly, by introducing the multiplexer factor node function
% \begin{equation}
%     f(y, x_1, \ldots, x_K, m) = \prod_{k=1}^K \delta(y - x_k)^{m_k},
% \end{equation}
% where $\delta(\cdot)$ denotes the Dirac delta distribution and where $y$ represents the output of the factor node and $x_k$ the inputs to the factor node.
% Intuitively, variables $y$ and $x_k$ are constrained to be equal if $m_k=1$, which can also be regarded as a generic mixture model with selector variable $m$.
% Each individual combination of the structures connected to $x_k$ and $y$ represents one of the $K$ models used for model comparison.
% The graph connected to the edge $y$ can be regarded as the likelihood model that is being shared among all models, whereas the parts connected to $x_k$ are model specific.
% Table~\ref{tab:node} visualizes this factor node and shows the derived outgoing messages according to \eqref{eq:sum-product-message}.

% Upon closer inspection, the derived message 
% \begin{equation}
%     \cev{\mu}_m(m) = \prod_{k=1}^K \left(\int \vec{\mu}_{x_k}(y) \cev{\mu}_y(y) \mathrm{d}y\right)^{m_k} = \prod_{k=1}^k p(D\midi m_k)^{m_k},
% \end{equation}
% in Table~\ref{tab:node} represents an unnormalized categorical distribution, with scale factor $\cev{\beta}_m = \sum_k p(D\midi m_k)$.
% Importantly, here we leverage the scale factors to compute the model evidence for the different input-output combinations locally inside of the factor node using \eqref{eq:scalefactors-evidence}.
% The normalized distribution $\cev{p}_m(m)$ coincides with the model evidence term $p(D\midi m)$ in \eqref{eq:bayes}.
% Additionally, in the message passing framework the prior term $p(m)$ in \eqref{eq:bayes} can straightforwardly be generalized to incoming message $\vec{\mu}_m(m)$.
% The marginal model evidence $p(m)$ in \eqref{eq:bayes} can be found using \eqref{eq:scalefactors-evidence}.

% \begin{table}[t]
%     \caption{Table containing (top) the Forney-style factor graph representation of the multiplexer ($\mathrm{MUX}$) node. (bottom) The derived outgoing messages for the multiplexer node. The backward message towards $m$ resembles a scaled categorical distribution. $e_k$ denotes the $k^\text{th}$ Cartesian standard unit vector.}
%     \label{tab:node}
%     \centering
%     \input{tables/node}
% \end{table}

% Although this mixture model concept for performing Bayesian model averaging is advocated for in \cite{kamary_testing_2018, keller_bayesian_2018}, our perspective on Bayesian model averaging does not make any strong assumptions on the probabilistic models connecting to the factor node in Table~\ref{tab:node}.
% This allows for the straightforward extension towards dynamical and hierarchical structures over $m$, $y$ and $x_k$.
% The only constraint imposed on our approach is that we should be able to compute scale factors for the incoming messages.
% Both \cite[Ch.6]{reller_state-space_2013} and \cite{nguyen_efficient_2022} introduce a variety of analytical rules for computing these scale factors for different message-node combinations, although there are also plenty of approximation methods available, such as sampling.


==> content/archive/04-methods.tex <==
% This section introduces the theoretical foundation that allows for treating Bayesian model averaging, selection and combination as a message passing procedure in Section~\ref{sec:comparison}.
% After reviewing factor graphs in Section~\ref{sec:background:factorgraphs}, we specify a variational optimization objective for multiple models at once in Section~\ref{sec:methods:WVFE}.
% We will show that optimization of the model selection variable can be rephrased as a probabilistic inference procedure on a separate graph with a factor node encapsulating the model-specific performance metrics.
% Section~\ref{sec:methods:sum-product} then describes how to perform exact probabilistic inference in these models through message passing, followed by an introduction of scale factors in Section~\ref{sec:methods:scalefactors}
% Finally, Section~\ref{sec:methods:mixture} introduces a factor node with custom message passing update that allows for jointly performing Bayesian model comparison with marginal computations.


% Under the above assumption on tractability and acyclicity and Theorem~\ref{theorem:sf} we obtain the relationship
% \begin{equation}\label{eq:exactF}
%     \exp(-\mathrm{F}_k[q,f]) = Z_k = \int\vec{\mu}_{s_j\vert m_k}(s_j) \cev{\mu}_{s_j\vert m_k}(s_j) \diff s_j
% \end{equation}
% for all $s_j\in\bm{s}_k$.
% In the message subscript we have added the explicit conditioning on the selected model in order to distinguish between messages toward variables that appear in multiple models.
% \tvdl{The above equation seems pivotal to your argument, perhaps explain the implications a bit more, what have you gained by doing this?}\bart{Reshuffled text}
% The implications of \eqref{eq:exactF} are that the VFE and normalization constant can be computed locally for all models using sum-product message passing with scale factors.

% Before continuing our discussion, let us first formally define the model selection variable $m$, which comprises a 1-of-$K$ binary vector with elements $m_k\in\{0, 1\}$ constrained by $\sum_{k=1}^K m_k = 1$.
% In the remainder of this paper conditioning on the variable $m_k$ is shorthand notation for $m_k=1$, i.e. $q(\cdot \midi m_k) \triangleq q(\cdot \midi m_k = 1)$.
% \bdv{I would introduce a different notation (or font) for the information $m_k = 1$, rather than abusing $m_k$. Eg, let $\mathsf{m}_k$ represent the information $m_k = 1$. So, you will get $p(\bm{s}_k\midi \mathsf{m}_k) = p(\bm{s}_k\midi m_k=1)$}\bart{Let's discuss}


% \bdv{There is some non-trivial mixing of normalized and unnormalized factors here. Let's be very careful. I think you want something like
% \begin{align*}
%     p(\bm{s},m) &= p(m) p(\bm{s}|m) \\
%     &= p(m) \prod_k p_k(\bm{s}_k)^{m_k} \\ &= p(m) \prod_k Z_k^{-m_k} f_k(\bm{s}_k)^{m_k} \\
% \end{align*}
% and then possibly introduce some definitions like:
% \begin{align*}
%     Z^{-1} &\triangleq \prod_k Z_k^{-m_k} \\
%     f(\bm{s}|m) &\triangleq \prod_k f_k(\bm{s}_k)^{m_k}
% \end{align*}
% which leads to 
% $$f(\bm{s},m) = Z \cdot p(\bm{s},m) = p(m) f(\bm{s}|m)$$
% If you want to work with unnormalized models $f_k$ and discuss modelling comparison issues, then you should not drop the evidences $Z_k$ from the notation.
% } 
% specifying a mixture model over the individual models $f_k(\bm{s}_k)$, with a prior $p(m)$ on the model selection variable $m$.
% \tvdl{The choice for the joint model as a harmonic average of submodels is quite specific and deserves some more motivation.}\bart{Addressed, rephrased introductory sentence. Agreed that motivation is missing. I am not sure whether it is a harmonic average (not sure how that is defined), but it actually is a mixture model (similarly as in the GammaMM paper), since $m$ is one-hot. (i.e. it actually is a categorical distribution whose realizations are models)} and corresponding approximate posterior distribution $q(\bm{s}, m)=q(m) \prod_{k=1}^Kq(\bm{s}_k \midi m_k)$, where $\bm{s} = \bigcup_{k=1}^K \bm{s}_k$ includes all variables, except for $m$.
% Let us define the weighted VFE $\mathrm{F}_m$ as the VFE of the joint model $f(\bm{s}, m)$ as
% \begin{equation} \label{eq:wvfe}
% \begin{split}
%     \mathrm{F}_m[q,f] 
%     &= \mathbb{E}_{q(s, m)}\left[\ln \frac{q(s, m)}{p(y, s, m)}\right], \\
%     &= \mathbb{E}_{q(m)}\left[\ln \frac{q(m)}{p(m)}\right] + \mathbb{E}_{q(m)}\left[\prod_{k=1}^K\big(\mathrm{F}_k[q,f]\big)^{m_k}\right],
% \end{split}
% \end{equation}
% in which the joint variational posterior $q(\bm{s},m)$ factorizes as $q(\bm{s}, m) = q(m) \prod_{k=1}^K q(\bm{s} \mid m_k)^{m_k}$.

% \bdv{This derivation is not clear to me. I would like to see this derivation in this paper. I am concerned about manipulations with unnormalized models $f_k$ and ignoring $Z_k$.}
% \bdv{It is odd that in first line you do expectation over $(\bm{s},m)$ and in 2nd line only over $m$.}
% \bart{Derivations in appendix?}

% \tvdl{Shouldn't there be a sum instead of a product in the second step (and further), since the iteration is now outside the log? And shouldn't it become a multiplication instead of an exponentiation when you pull it out the log?}\bart{Normally you are indeed right. However, since $m$ is one-hot we can perform some tricks, e.g. $$\ln \prod_k a_k^{m_k} = \sum_k m_k \ln a_k = \prod_k \ln a_k^{m_k}$$, since only a single $m$ can be active at a time. By marginalizing over $q(m)$, we obtain a mixture distribution with all components present}
% \tvdl{I removed a double $q(\bm{s}, m)$ in the first line, please verify.}
% \bart{Good catch! Correct indeed.}
% \tvdl{Is the step to the second line correct? Are you allowed to pull out the exponent $m_k$ that only appears in the joint model to also cover the variational distribution, or does this step require an additional assumption like $q(\bm{s}_k|m_k) = q(\bm{s}_k)^{m_k}$?}
% \bart{I could also remove the second line if it causes confusion. The main result is in the last line.}

 \bdv{Indeed! Very nice observation. Basically, the approach that you work on here can be used to implement active inference. Moreover, this observation is key to considering model structure adaptation a search process that is driven by active inference.}

 \bdv{let's get rid of the $f$ in the argument of $F$ if you're not minimizing over $f$. I also think that you should drop the subscript $m$ from $F$. By minimizing over $q$, you update beliefs $q(m)$ over $m$. Here, $m$ is not a fixed indicator but a variable.}
\bdv{I am generally not excited about using $m$ as a subscript (not for $f$ and also not for $F$. I dont mind $k$ as a subscript to indicate a function for model $m_k$. But we entertain prior beliefs $p(m)$ and posterior beliefs $q(m)$ over $m$.}

The above definition of the weighted VFE in \eqref{eq:WVFE} is slightly restrictive.
In this definition, we assume a single prior distribution $p(m)$ over $m$ for illustrative purposes. \bdv{You did never mention nor used the fact that $p(m)$ must be fixed, or non-hierarchical. So I would delete the remark about restrictive but keep pursuing the idea (as you do below) that $p(m)$ may be complex and time-varying.}

\bdv{I would have expected a graph on $p(m) f_m(m)$, not an FFG with $f_a$. Let's separate the review on SP MP from derivations about FE in mixture models as the latter is part of novelty in this paper. }


% This subgraph and connected structure can be considered to be a model on its own encompassing the individual submodels $f_k$.
% Specifically, in the general case, we would be considering the subgraph as depicted in Figure~\ref{fig:subgraph-m}, with corresponding VFE. 
% \begin{figure}[t]
%     \centering
%     \input{figures/subgraph-m.tikz}
%     \caption{Subgraph of the model selection parameter $m$. The factor node function $f_m$ is defined in \eqref{eq:factor:VFE}.}
%     \label{fig:subgraph-m}
% \end{figure}

% \tvdl{Since $q(\bm{s}_o | m_k) = q(\bm{s}_o)^{m_k}$, I'd choose one of those (throughout the paper). Also, I find the intuition behind $\bm{s}_o$ and this equation difficult to grasp, a figure might help, also for later reference in the definition of $f_o$.}\bart{I see that there is some confusion in notation. I added a clarifying sentence above.}

\bdv{Again, I am concerned about introducing unnormalized models without evidences $Z_k$ and proceedings to apply rules of probability theory. If you apply any PT rules, please use normalized distributions.}

% \tvdl{I don't understand the variable assignment in Fig.~\ref{fig:models}. In the right figure, the same variable $s_j$ seems defined on multiple edges. Conditioning relates to node definitions, not variable assignment. Perhaps use a double subscript instead?}\bart{I understand the confusion and I have tried to clarify it a bit more in the caption.}

\tvdl{This definition implies that "the model submits to exact inference" is an additional requirement, which cannot be tested at the time of definition. Here the proof of the pudding (model definition) is in the eating it (inference). Do you need to offer this additional qualification, or is it enough that the FFGs are acyclic?}\bart{Removed this condition. To discuss}

==> content/archive/05-selection.tex <==
\section{Bayesian model selection} \label{sec:selection}
% In Bayesian model selection the goal is to just select the model with the largest a posteriori probability.
% Bayesian model selection can be derived as a special case from the Bayesian model averaging procedure in Section~\ref{sec:averaging} by constraining \cite{senoz_variational_2021} the model posterior distribution $p(m \midi D)$ to
% \begin{equation}
%     q(m) = \delta(m-e_k) \text{ where } k = \argmax_k \vec{\mu}_m(e_k) \cev{\mu}_m(e_k),
% \end{equation}
% where $e_k$ represents the $k^\text{th}$ Cartesian standard unit vector.
% Effectively, first the model posterior distribution $p(m\mid D)$ is computed after which the posterior is fixed to the model with the largest model evidence.
% This local constraint on the posterior and the corresponding message passing scheme can also be interpreted as a local expectation-maximization scheme \cite{dauwels_expectation_2005, senoz_variational_2021} or as a specific type of intervention \cite{pearl_causality_2009}.
% Nodes adjacent to the edge $m$ will no longer receive incoming messages $\mu_m(m)$, but instead receive $q(m)$ for their computations.

\bdv{This is all good, but you introduce and explain sum-product MP in the background section and here we're doing VMP with constraints a la Senoz in the CBFE paper. That's quite a jump. } \bart{I don't want to dive into form constraints in this paper. The message passing will remain sum-product, so no VMP. I can add a visualization of the MP-scheme around a delta-constraint (mu in, q out) to clarify the description in the text.}

% Finally, we end by describing how Dirichlet processes can be cast in factor graphs using message passing in Section~\ref{sec:comparison:dirichlet}.


==> content/archive/06-combination.tex <==
\section{Bayesian model combination} \label{sec:combination}
% A common misconception is that Bayesian model averaging always yields the most optimal set of models \cite{bishop_pattern_2006, minka_bayesian_2000}.
% Instead, Bayesian model averaging always converges to a single model that yields the largest model evidence.
% If the data generating model is part of the available set of models, then Bayesian model averaging will select this model, leading to optimal performance.
% However, if this is not the case, then the chosen model can be suboptimal and often there exists a linear combination of the available set of models that yields a better data fit.
% Bayesian model combination \cite{monteith_turning_2011} tackles this problem and tries to find the best possible linear combination of models that maximizes the model evidence.

% \subsection{Combination estimation using Dirichlet priors}
% VMP \cite{dauwels_variational_2007}
% local \cite{senoz_variational_2021}
% \begin{equation}
%     p(m) = p(c) \prod_{n=1}^N p(m_n \midi c),
% \end{equation}
% with $p(m_n \midi c) = \mathrm{Cat}(m_n \midi c)$ and $p(c) = \mathrm{Dir}(c \midi \alpha)$
% \begin{equation}
%     p(m, c \midi D) \approx q(m,c) = q(c) \prod_{n=1}^N q(m_n)
% \end{equation}
% with $q(c) = \mathrm{Dir}(c \midi \hat{\alpha})$ and $q(m_n) = \mathrm{Cat}(m_n \midi \hat{\beta}_n)$.

==> content/archive/07-discussion.tex <==
% \tvdl{Good discussion. You might consider grounding it more in the literature, by including more appropriate references here and there (esp. the last paragraph). This then shows that these ideas for future research are not just an intellectual exercise, but actually things that people are looking for.}\bart{Addressed}

==> content/archive/A1-derivations.tex <==
\section{Derivations}

\subsection{Variational posterior}
\begin{equation}
    q(y,\bm{x},m)
\end{equation}


\subsection{Node factorization}
\begin{equation}
    f(y, \bm{x}, m) = \prod_{k=1}^K f_k(y, x_k)^{m_k}
\end{equation}


\subsection{Node-local Bethe free energy}
\begin{equation}
    \mathrm{F}[q,f] 
    &= \int q(y, \bm{x}, m) \ln \frac{q(y,\bm{x},m)}{f(y, \bm{x}, m)} \diff y \diff \bm{x} \diff m
\end{equation}


\subsection{Constraints}
\begin{subequations}
    \begin{equation}
        \int q(y, \bm{x}, m) \diff y \diff \bm{x} \diff m = 1
    \end{equation}
    \begin{equation}
        \int q(y, \bm{x}, m) \diff y \diff \bm{x} = q(m)
    \end{equation}
    \begin{equation}
        \int q(y, \bm{x}, m) \diff \bm{x} \diff m = q(y)
    \end{equation}
    \begin{equation}
        \int q(y, \bm{x}, m) \delta(m-e_k) \diff y \diff \bm{x}_{\backslash k} \diff m = q(x_k, m=e_k) \qquad \text{for }k=1,2,\ldots,K
    \end{equation}
\end{subequations}


\subsection{Lagrangians}

\subsubsection{Node-induced Lagrangian}
\begin{equation}
    \begin{split}
        \mathrm{L}_f[q,f]
        &= \mathrm{F}[q,f] \\
        &\quad + \psi \left( \int q(y, \bm{x}, m) \diff y \diff \bm{x} \diff m - 1 \right) \\
        &\quad + \int \lambda_m(m) \left( \int q(y, \bm{x}, m) \diff y \diff \bm{x} - q(m)\right) \diff m \\
        &\quad + \int \lambda_y(y) \left(\int q(y, \bm{x}, m) \diff \bm{x} \diff m - q(y)\right) \diff y \\
        &\quad + \sum_{k=1}^K \int \lambda_{x_k}(x_k) \left( \int q(y, \bm{x}, m) \delta(m-e_k) \diff y \diff \bm{x}_{\backslash k} \diff m - q(x_k,m=e_k) \right) \diff x_k
    \end{split}
\end{equation}

\subsubsection{Edge-induced Lagrangian for $m$}
\begin{equation}
    \begin{split}
        \mathrm{L}_m[q,f] = \mathrm{H}[q(m)] 
        &+ \psi_m \left(\int q(m) \diff m - 1\right) + \int \lambda_m^\star(m) \left( \int q(m, \bm{s}) \diff \bm{s} - q(m)\right) \diff m \\
        &+ \int \lambda_m(m) \left(\int q(y, \bm{x}, m) \diff y \diff \bm{x} - q(m)\right) \diff m
    \end{split}
\end{equation}

\subsubsection{Edge-induced Lagrangian for $y$}
\begin{equation}
    \begin{split}
        \mathrm{L}_y[q,f] = \mathrm{H}[q(y)] 
        &+ \psi_y \left(\int q(y) \diff y - 1\right) + \int \lambda_y^\star(y) \left( \int q(y, \bm{s}) \diff \bm{s} - q(y)\right) \diff y \\
        &+ \int \lambda_y(y) \left(\int q(y, \bm{x}, m) \diff \bm{x} \diff m - q(y)\right) \diff y
    \end{split}
\end{equation}

\subsubsection{Edge-induced Lagrangian for $x_k$ with $m=e_k$}
\begin{equation}
    \begin{split}
        \mathrm{L}_{x_k}[q,f] = \mathrm{H}[q(x_k, m=e_k)] 
        &+ \psi_{x_k} \left(\int q(x_k, m=e_k) \diff x_k - q(m=e_k)\right) \\
        &+ \int \lambda_{x_k}^\star(x_k) \left( \int q(x_k, \bm{s}, m=e_k) \diff \bm{s} - q(x_k, m=e_k)\right) \diff x_k \\
        &+ \int \lambda_{x_k}(x_k) \left(\int q(y, \bm{x}, m)\delta(m-e_k) \diff y \diff \bm{x}_{\backslash k} \diff m - q(x_k, m=e_k)\right) \diff x_k
    \end{split}
\end{equation}

\subsection{Stationary points}

\subsubsection{Stationary point for $q(y,x,m)$}
\begin{equation}
    \begin{split}
        &\frac{\diff \mathrm{L}_f[q + \varepsilon \phi]}{\diff \varepsilon}\bigg\vert_{\varepsilon=0} \\
        &= \frac{\diff}{\diff \varepsilon} \Bigg[ \int \big( q(y,\bm{x}, m) + \varepsilon \phi(y,\bm{x},m)\big) \ln \frac{q(y,\bm{x}, m) + \varepsilon \phi(y,\bm{x},m)}{f(y, \bm{x},m)} \diff y \diff \bm{x} \diff m \\
        &\qquad \qquad + \psi \left( \int \big( q(y,\bm{x}, m) + \varepsilon \phi(y,\bm{x},m)\big) \diff y \diff \bm{x} \diff m - 1 \right) \\
        &\qquad \qquad + \int \lambda_m(m) \left( \int \big( q(y,\bm{x}, m) + \varepsilon \phi(y,\bm{x},m)\big) \diff y \diff \bm{x} - q(m)\right) \diff m \\
        &\qquad \qquad + \int \lambda_y(y) \left(\int \big( q(y,\bm{x}, m) + \varepsilon \phi(y,\bm{x},m)\big) \diff \bm{x} \diff m - q(y)\right) \diff y\\
        &\qquad \qquad + \sum_{k=1}^K \int \lambda_{x_k}(x_k) \left( \int \big( q(y,\bm{x}, m) + \varepsilon \phi(y,\bm{x},m)\big) \delta(m-e_k) \diff y \diff \bm{x}_{\backslash k} \diff m - q(x_k, m=e_k) \right) \diff x_k \Bigg]_{\varepsilon=0} \\
        &= \Bigg[ \int \phi(y, \bm{x}, m) \ln \frac{q(y, \bm{x}, m) + \varepsilon \phi(y, \bm{x},m)}{f(y, \bm{x}, m)} \diff y \diff \bm{x} \diff m + \int \phi(y, \bm{x}, m) \diff y \diff \bm{x} \diff m \\
        &\qquad \qquad + \psi\int \phi(y, \bm{x}, m) \diff y \diff \bm{x} \diff m + \int \lambda_m(m) \phi(y, \bm{x}, m) \diff y \diff \bm{x} \diff m \\
        &\qquad \qquad + \int \lambda_y(y) \phi(y,\bm{x},m) \diff y \diff \bm{x} \diff m + \sum_{k=1}^K \int \lambda_{x_k}(x_k) \phi(y,\bm{x},m) \delta(m-e_k) \diff y \diff \bm{x} \diff m \Bigg]_{\varepsilon=0}\\
        &= \int \phi(y, \bm{x}, m) \underbrace{\left(\ln \frac{q(y,\bm{x},m)}{f(y,\bm{x},m)} + 1 + \psi + \lambda_m(m) + \lambda_y(y) + \sum_{k=1}^K \lambda_{x_k}(x_k) \delta(m-e_k)\right)}_{\frac{\delta \mathrm{L}}{\delta q}} \diff y \diff \bm{x} \diff m
    \end{split}
\end{equation}
\begin{equation}
    \frac{\delta \mathrm{L}}{\delta q} = \ln \frac{q(y,\bm{x},m)}{f(y,\bm{x},m)} + 1 + \psi + \lambda_m(m) + \lambda_y(y) + \sum_{k=1}^K \lambda_{x_k}(x_k) \delta(m-e_k) = 0
\end{equation}
\begin{equation}
    q(y, \bm{x}, m) = f(y,\bm{x}, m) \exp\{-1 - \psi\} \exp\{-\lambda_m(m)\}\exp\{-\lambda_y(y)\}\prod_{k=1}^K \exp\{-\lambda_{x_k}(x_k)\}^{m_k}
\end{equation}
Using normalization constraint:
\begin{equation}
    q(y, \bm{x}, m) = \frac{\displaystyle \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k}}{\displaystyle \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff y \diff \bm{x} \diff m}
\end{equation}


\subsubsection{Stationary point for $q(m)$}
\begin{equation}
    \begin{split}
        &\frac{\diff \mathrm{L}_m[q + \varepsilon \phi]}{\diff \varepsilon} \Bigg\vert_{\epsilon=0} \\
        &= \frac{\diff}{\diff \varepsilon} \Bigg[ - \int \big(q(m) + \varepsilon \phi(m) \big) \ln \big(q(m) + \varepsilon \phi(m)\big) \diff m + \psi_m \left(\int \big(q(m) + \varepsilon \phi(m)\big) \diff m - 1\right) \\
        &\qquad \qquad + \int \lambda_m^\star(m) \left(\int q(m, \bm{s}) \diff \bm{s} - \big(q(m)+\varepsilon\phi(m)\big)\right)\diff m \\
        &\qquad \qquad + \int \lambda_m(m) \left(\int q(y, \bm{x}, m) \diff y \diff \bm{x} - \big(q(m) + \varepsilon \phi(m)\big)\right) \diff m \Bigg]_{\varepsilon=0} \\
        &= \Bigg[ - \int \phi(m) \ln \big(q(m) + \varepsilon \phi(m)\big)\diff m - \int \phi(m) \diff m + \psi_m \int \phi(m) \diff m \\
        &\qquad \qquad - \int \lambda_m^\star (m) \phi(m) \diff m  - \int \lambda_m(m) \phi(m) \diff m\Bigg]_{\varepsilon=0} \\
        &= \int \phi(m) \underbrace{\bigg( -\ln q(m) - 1 + \psi_m - \lambda^\star_m(m) - \lambda_m(m)\bigg)}_{\frac{\delta \mathrm{L}}{\delta q}} \diff m
    \end{split}
\end{equation}
\begin{equation}
    \frac{\delta \mathrm{L}}{\delta q} = -\ln q(m) - 1 +\psi_m -\lambda_m^\star(m) - \lambda_m(m) = 0
\end{equation}
\begin{equation}
    q(m) = \exp\{-1 + \psi_m\}\exp\{-\lambda_m^\star(m)\}\exp\{-\lambda_m(m)\}
\end{equation}
\begin{equation}
    q(m) = \frac{\vec{\mu}_m(m)\cev{\mu}_m(m)}{\exp\{1 - \psi_m\}} = \frac{\vec{\mu}_m(m)\cev{\mu}_m(m)}{\int \vec{\mu}_m(m)\cev{\mu}_m(m) \diff m}
\end{equation}

\subsubsection{Stationary point for $q(y)$}
\begin{equation}
    \begin{split}
        &\frac{\diff \mathrm{L}_y[q + \varepsilon \phi]}{\diff \varepsilon} \Bigg\vert_{\epsilon=0} \\
        &= \frac{\diff}{\diff \varepsilon} \Bigg[ - \int \big(q(y) + \varepsilon \phi(y) \big) \ln \big(q(y) + \varepsilon \phi(y)\big) \diff y + \psi_y \left(\int \big(q(y) + \varepsilon \phi(y)\big) \diff y - 1\right) \\
        &\qquad \qquad + \int \lambda_y^\star(y) \left(\int q(y, \bm{s}) \diff \bm{s} - \big(q(y)+\varepsilon\phi(y)\big)\right)\diff y \\
        &\qquad \qquad + \int \lambda_y(y) \left(\int q(y, \bm{x}, m) \diff \bm{x} \diff m - \big(q(y) + \varepsilon \phi(y)\big)\right) \diff y \Bigg]_{\varepsilon=0} \\
        &= \Bigg[ - \int \phi(y) \ln \big(q(y) + \varepsilon \phi(y)\big)\diff y - \int \phi(y) \diff y + \psi_y \int \phi(y) \diff y \\
        &\qquad \qquad - \int \lambda_y^\star (y) \phi(y) \diff m  - \int \lambda_y(y) \phi(y) \diff y\Bigg]_{\varepsilon=0} \\
        &= \int \phi(y) \underbrace{\bigg( -\ln q(y) - 1 + \psi_y - \lambda^\star_y(y) - \lambda_y(y)\bigg)}_{\frac{\delta \mathrm{L}}{\delta q}} \diff y
    \end{split}
\end{equation}
\begin{equation}
    \frac{\delta \mathrm{L}}{\delta q} = -\ln q(y) - 1 +\psi_y -\lambda_y^\star(y) - \lambda_y(y) = 0
\end{equation}
\begin{equation}
    q(y) = \exp\{-1 + \psi_y\}\exp\{-\lambda_y^\star(y)\}\exp\{-\lambda_y(y)\}
\end{equation}
\begin{equation}
    q(y) = \frac{\vec{\mu}_y(y) \cev{\mu}_y(y)}{\exp\{1-\psi_y\}} = \frac{\vec{\mu}_y(y) \cev{\mu}_y(y)}{\int \vec{\mu}_y(y) \cev{\mu}_y(y) \diff y}
\end{equation}


\subsubsection{Stationary point for $q(x_k, m=e_k)$}
\begin{equation}
    \begin{split}
        &\frac{\diff \mathrm{L}_{x_k}[q + \varepsilon \phi]}{\diff \varepsilon} \Bigg\vert_{\epsilon=0} \\
        &= \frac{\diff}{\diff \varepsilon} \Bigg[ - \int \big(q(x_k, m=e_k) + \varepsilon \phi(x_k) \big) \ln \big(q(x_k, m=e_k) + \varepsilon \phi(x_k)\big) \diff x_k \\
        &\qquad \qquad + \psi_{x_k} \left(\int \big(q(x_k, m=e_k) + \varepsilon \phi(x_k)\big) \diff x_k - q(m=e_k)\right) \\
        &\qquad \qquad + \int \lambda_{x_k}^\star(x_k) \left(\int q(x_k, \bm{s}, m=e_k) \diff \bm{s} - \big(q(x_k, m=e_k)+\varepsilon\phi(x_k)\big)\right)\diff x_k \\
        &\qquad \qquad + \int \lambda_{x_k}(x_k) \left(\int q(y, \bm{x}, m)\delta(m-e_k) \diff y\diff \bm{x}_{\backslash k} \diff m - \big(q(x_k, m=e_k) + \varepsilon \phi(x_k)\big)\right) \diff x_k \Bigg]_{\varepsilon=0} \\
        &= \Bigg[ - \int \phi(x_k) \ln \big(q(x_k, m=e_k) + \varepsilon \phi(x_k)\big)\diff x_k - \int \phi(x_k) \diff x_k + \psi_{x_k} \int \phi(x_k) \diff x_k \\
        &\qquad \qquad - \int \lambda_{x_k}^\star (x_k) \phi(x_k) \diff x_k  - \int \lambda_{x_k}(x_k) \phi(x_k) \diff x_k\Bigg]_{\varepsilon=0} \\
        &= \int \phi(x_k) \underbrace{\bigg( -\ln q(x_k, m=e_k) - 1 + \psi_{x_k} - \lambda^\star_{x_k}(x_k) - \lambda_{x_k}(x_k)\bigg)}_{\frac{\delta \mathrm{L}}{\delta q}} \diff x_k
    \end{split}
\end{equation}
\begin{equation}
    \frac{\delta \mathrm{L}}{\delta q} = -\ln q(x_k,m=e_k) - 1 +\psi_{x_k} -\lambda_{x_k}^\star(x_k) - \lambda_{x_k}(x_k) = 0
\end{equation}
\begin{equation}
    q(x_k,m=e_k) = \exp\{-1 + \psi_{x_k}\}\exp\{-\lambda_{x_k}^\star(x_k)\}\exp\{-\lambda_{x_k}(x_k)\}
\end{equation}
\begin{equation}
    q(x_k, m=e_k) = \frac{\vec{\mu}_{x_k}(x_k)\cev{\mu}_{x_k}(x_k)}{\exp\{1 - \psi_{x_k}\}}
\end{equation}
where
\begin{equation}
    \exp\{1-\psi_{x_k}\} = \frac{1}{q(m=e_k)}\int\vec{\mu}_{x_k}(x_k) \cev{\mu}_{x_k}(x_k) \diff x_k     
\end{equation}

\subsection{Message computations}

\subsubsection{Message towards $m$}
\begin{equation}
    q(m) = \int q(y, \bm{x}, m) \diff y \diff \bm{x}
\end{equation}
\begin{equation}
    \frac{\vec{\mu}_m(m)\cev{\mu}_m(m)}{\int \vec{\mu}_m(m)\cev{\mu}_m(m) \diff m} = \frac{\displaystyle \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff y \diff \bm{x}}{\displaystyle \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff y \diff \bm{x} \diff m}
\end{equation}
\begin{equation}
    \cev{\mu}_m(m) = Z  \prod_{k=1}^K \left(\int\vec{\mu}_{x_k}(x_k)f_k(y, x_k)\cev{\mu}_y(y) \diff y \diff x_k \right)^{m_k}
\end{equation}
where
\begin{equation}
    Z = \frac{\displaystyle\int \vec{\mu}_m(m)\cev{\mu}_m(m) \diff m }{\displaystyle \int \vec{\mu}_m(m)\cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff y \diff \bm{x} \diff m}
\end{equation}

\subsubsection{Message towards $y$}
\begin{equation}
    q(y) = \int q(y,\bm{x}, m) \diff \bm{x} \diff m
\end{equation}
\begin{equation}
    \frac{\vec{\mu}_y(y) \cev{\mu}_y(y)}{\int \vec{\mu}_y(y) \cev{\mu}_y(y) \diff y}
    =
    \frac{\displaystyle \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff \bm{x} \diff m}{\displaystyle \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff y \diff \bm{x} \diff m}
\end{equation}

\begin{equation}
    \vec{\mu}_y(y) = Z \int \vec{\mu}_m(m) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff \bm{x} \diff m
\end{equation}
where 
\begin{equation}
    Z = \frac{\int \vec{\mu}_y(y) \cev{\mu}_y(y) \diff y}{\displaystyle \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff y \diff \bm{x} \diff m}
\end{equation}

\subsubsection{Message towards $x_k$}
\begin{equation}
    q(x_k, m=e_k) = \int q(y, \bm{x}, m) \delta(m-e_k) \diff y \diff \bm{x}_{\backslash k} \diff m
\end{equation}
\begin{equation}
    \frac{\vec{\mu}(m=e_k)}{\int\vec{\mu}_{x_k}(x_k) \cev{\mu}_{x_k}(x_k) \diff x_k} \vec{\mu}_{x_k}(x_k) \cev{\mu}_{x_k}(x_k) = \frac{\displaystyle \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \delta(m-e_k) \diff y\diff \bm{x}_{\backslash k} \diff m}{\displaystyle \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff y \diff \bm{x} \diff m}
\end{equation}
\begin{equation}
    \cev{\mu}_{x_k}(x_k) = Z \vec{\mu}_m(m=e_k) \int f_k(y,x_k) \cev{\mu}_y(y) \diff y
\end{equation}
where 
\begin{equation}
    Z = \frac{\displaystyle \int \vec{\mu}_{x_k}(x_k) \cev{\mu}_{x_k}(x_k) \diff x_k}{\displaystyle \vec{\mu}(m=e_k)\int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(f_k(y, x_k) \vec{\mu}_{x_k}(x_k)\big)^{m_k} \diff y \diff \bm{x} \diff m}
\end{equation}











\newpage







































% \subsection{Variational posterior}
% \begin{equation}
%     q(y,\bm{x},m)
% \end{equation}

% \subsection{Node factorization}
% \begin{equation}
%     f(y, \bm{x}, m) = \prod_{k=1}^K f_k(y, x_k)^{m_k}
% \end{equation}

% \subsection{Node-local Bethe free energy}
% \begin{equation}
%     \begin{split}
%         \mathrm{F}[q,f] 
%         &= \int q_a(y, \bm{x}, m) \ln \frac{q_a(y,\bm{x},m)}{f_a(y, \bm{x}, m)} \diff y \diff \bm{x} \diff m \\
%         &= \int q_a(y, \bm{x}, m) \ln \frac{q_a(y,\bm{x},m)}{\prod_{k=1}^K f_k(y, x_k)^{m_k}} \diff y \diff \bm{x} \diff m
%     \end{split}
% \end{equation}

% \subsection{Constraints}
% \begin{equation}
%     \psi \left(\int q_a(y, \bm{x}, m) \diff y \diff \bm{x} \diff m - 1 \right)
% \end{equation}
% \begin{equation}
%     \int \lambda_m(m) \left(\int q_a(y, \bm{x}, m) \diff y \diff \bm{x} - q(m)\right)\diff m
% \end{equation}
% \begin{equation}
%     \int \lambda_y(y) \left(\int q_a(y, \bm{x}, m) \diff \bm{x} \diff m - q(y) \right) \diff y
% \end{equation}
% \begin{equation}
%     \int \prod_{k=1}^K \left(\int \lambda_k(x_k) \left(\int q_a(y,\bm{x}, m) \diff y \diff \bm{x}_{\backslash k} - q(x_k) \right)\diff x_k\right)^{m_k} \diff m
% \end{equation}

% \subsection{Lagrangian}
% \begin{equation}
%     \begin{split}
%         \mathrm{L}[q,f]
%         &= \int q_a(y, \bm{x}, m) \ln \frac{q_a(y,\bm{x},m)}{\prod_{k=1}^K f_k(y, x_k)^{m_k}} \diff y \diff \bm{x} \diff m \\
%         &\qquad + \psi \left(\int q_a(y, \bm{x}, m) \diff y \diff \bm{x} \diff m - 1 \right) \\
%         &\qquad + \int \lambda_m(m) \left(\int q_a(y, \bm{x}, m) \diff y \diff \bm{x} - q(m)\right)\diff m \\
%         &\qquad + \int \lambda_y(y) \left(\int q_a(y, \bm{x}, m) \diff \bm{x} \diff m - q(y) \right) \diff y \\
%         &\qquad + \int \prod_{k=1}^K \left(\int \lambda_k(x_k) \left(\int q_a(y,\bm{x}, m) \diff y \diff \bm{x}_{\backslash k} - q(x_k) \right)\diff x_k\right)^{m_k}\diff m
%     \end{split}
% \end{equation}

% \subsection{Functional derivative with respect to $q_a(y, x, m)$}
% \begin{equation}
%     \begin{split}
%         &\frac{\diff\mathrm{L}[q_a(y, \bm{x}, m) + \varepsilon \phi(y, \bm{x},m)]}{\diff \varepsilon}\Bigg\vert_{\varepsilon=0} \\
%         &= \frac{\diff}{\diff \varepsilon} \Bigg[ \int \big(q_a(y, \bm{x}, m) + \varepsilon \phi(y, \bm{x},m)\big) \ln \frac{\big(q_a(y, \bm{x}, m) + \varepsilon \phi(y, \bm{x},m)\big)}{\prod_{k=1}^K f_k(y, x_k)^{m_k}} \diff y \diff \bm{x} \diff m \\
%         &\qquad + \psi \left(\int \big(q_a(y, \bm{x}, m) + \varepsilon \phi(y, \bm{x},m)\big) \diff y \diff \bm{x} \diff m - 1 \right) \\
%         &\qquad + \int \lambda_m(m) \left(\int \big(q_a(y, \bm{x}, m) + \varepsilon \phi(y, \bm{x},m)\big) \diff y \diff \bm{x} - q(m)\right)\diff m \\
%         &\qquad + \int \lambda_y(y) \left(\int \big(q_a(y, \bm{x}, m) + \varepsilon \phi(y, \bm{x},m)\big) \diff \bm{x} \diff m - q(y) \right) \diff y \\
%         &\qquad + \int \prod_{k=1}^K \left(\int \lambda_k(x_k) \left(\int \big(q_a(y, \bm{x}, m) + \varepsilon \phi(y, \bm{x},m)\big) \diff y \diff \bm{x}_{\backslash k} - q(x_k) \right)\diff x_k\right)^{m_k} \diff m\Bigg]_{\varepsilon=0} \\
%         & = \Bigg[ \int \phi(y, \bm{x},m) \ln \frac{\big(q_a(y, \bm{x}, m) + \varepsilon \phi(y, \bm{x},m)\big)}{\prod_{k=1}^K f_k(y, x_k)^{m_k}} \diff y \diff \bm{x} \diff m \\
%         &\qquad + \int \phi(y, \bm{x}, m)\diff y \diff \bm{x} \diff m\\
%         &\qquad + \psi \left(\int \phi(y, \bm{x},m) \diff y \diff \bm{x} \diff m \right) \\
%         &\qquad + \int \lambda_m(m) \left(\int \phi(y, \bm{x},m) \diff y \diff \bm{x}\right)\diff m \\
%         &\qquad + \int \lambda_y(y) \left(\int \phi(y, \bm{x},m) \diff \bm{x} \diff m \right) \diff y \\
%         &\qquad + \int \prod_{k=1}^K \left(\int \lambda_k(x_k) \left(\int \phi(y, \bm{x},m) \diff y \diff \bm{x}_{\backslash k} \right)\diff x_k\right)^{m_k} \diff m \Bigg]_{\varepsilon=0} \\
%         &= \int \phi(y, \bm{x},m) \underbrace{\Bigg( \ln q_a(y, \bm{x}, m) - \ln \prod_{k=1}^K f_k(y,x_k)^{m_k} + 1 + \psi + \lambda_m(m) + \lambda_y(y) + \prod_{k=1}^K \lambda_k(x_k)^{m_k}\Bigg)}_{\frac{\delta \mathrm{L}}{\delta q_a}} \diff y\diff \bm{x} \diff m
%     \end{split}
% \end{equation}

% \begin{equation}
%     \ln q_a(y, \bm{x}, m) - \ln \prod_{k=1}^K f_k(y,x_k)^{m_k} + 1 + \psi + \lambda_m(m) + \lambda_y(y) + \prod_{k=1}^K \lambda_k(x_k)^{m_k}
% \end{equation}

% \begin{equation}
%     q_a(y, \bm{x}, m) = \exp\{-1 -\psi\} \exp\{-\lambda_m(m)\} \exp\{\lambda_y(y)\}\prod_{k=1}^K \big(f_k(y,x_k)\exp\{-\lambda_k(x_k)\}\big)^{m_k}
% \end{equation}

% \begin{equation}
%     q_a(y, \bm{x}, m) = \exp\{-1-\psi\} \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(\vec{\mu}_k(x_k) f_k(y,x_k)\big)^{m_k}
% \end{equation}
% where
% \begin{equation}
%     \exp\{1 + \psi\} = \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(\vec{\mu}_k(x_k) f_k(y,x_k)\big)^{m_k} \diff y \diff \bm{x} \diff m  
% \end{equation} 

% \subsection{Message towards $y$}
% From the stationary solutions of the edge-specific Lagrangian
% \begin{equation}
%     q(y) = \frac{\vec{\mu}_y(y) \cev{\mu}_y(y)}{\int \vec{\mu}_y(y)\cev{\mu}_y(y) \diff y}
% \end{equation}
% From the marginalization constraint
% \begin{equation}
%     \begin{split}
%         q(y)
%         &= \int q_a(y, \bm{x}, m) \diff \bm{x} \diff m \\
%         &\propto \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(\vec{\mu}_k(x_k) f_k(y,x_k)\big)^{m_k} \diff \bm{x} \diff m \\
%         &= \cev{\mu}_y(y) \int \sum_{k=1}^K \vec{\mu}_m(e_k) \vec{\mu}_k(x_k) f_k(y,x_k) \diff \bm{x} \\
%         &= \cev{\mu}_y(y) \left(\sum_{k=1}^K \vec{\mu}_m(e_k) \int \vec{\mu}_k(x_k) f_k(y,x_k) \diff x_k\right)
%     \end{split}
% \end{equation}
% From this we observe
% \begin{equation}
%     \vec{\mu}_y(y) \propto \sum_{k=1}^K \vec{\mu}_m(e_k) \int \vec{\mu}_k(x_k) f_k(y,x_k) \diff x_k
% \end{equation}
% which resembles a (scaled) mixture model distribution.

% \subsection{Message towards $m$}
% From the stationary solution of the edge-specific Lagrangian
% \begin{equation}
%     q(m) = \frac{\vec{\mu}_m(m) \cev{\mu}_m(m)}{\int \vec{\mu}_m(m) \cev{\mu}_m(m) \diff m}
% \end{equation}
% From the marginalization constraint
% \begin{equation}
%     \begin{split}
%         q(m)
%         &= \int q_a(y, \bm{x},m) \diff y \diff \bm{x} \\
%         &\propto \int \vec{\mu}_m(m) \cev{\mu}_y(y) \prod_{k=1}^K \big(\vec{\mu}_k(x_k) f_k(y,x_k)\big)^{m_k} \diff y \diff \bm{x}\\
%         &= \vec{\mu}_m(m) \prod_{k=1}^K \left(\int \vec{\mu}_k(x_k) f_k(y,x_k)\cev{\mu}_y(y) \diff x_k \diff y\right)^{m_k}
%     \end{split}
% \end{equation}
% From this we observe
% \begin{equation}
%     \cev{\mu}_m(m) = \prod_{k=1}^K \left(\int \vec{\mu}_k(x_k) f_k(y,x_k) \cev{\mu}_y(y) \diff x_k \diff y\right)^{m_k}
% \end{equation}
% which resembles a (scaled) categorical distribution.

% \subsection{ Message towards $x_j$}
% From the stationary solution of the edge-specific Lagrangian
% \begin{equation}
%     q(x_j) = \frac{\vec{\mu}_{x_j}(x_j) \cev{\mu}_{x_j}(x_j)}{\int \vec{\mu}_{x_j}(x_j) \cev{\mu}_{x_j}(x_j) \diff x_j}
% \end{equation}
% From the marginalization constraint
% \begin{equation}
%     \begin{split}
%         q(x_j)
%         &= \int q_a(y, \bm{x}, m=e_j) \diff y \diff \bm{x}_{\backslash j}\\
%         &\propto \int \vec{\mu}_m(e_j) \cev{\mu}_y(y) \vec{\mu}_k(x_k) f_k(y,x_k) \diff y \\
%         &= \vec{\mu}_{x_j}(x_j) \vec{\mu}_m(e_j) \int f_j(y,x_j) \cev{\mu}_y(y) \diff y
%     \end{split}
% \end{equation}

% From this we observe
% \begin{equation}
%     \cev{\mu}_{x_k}(x_k) = \vec{\mu}_m(e_k) \int f_k(y, x_k) \cev{\mu}_y(y) \diff y
% \end{equation}

% \subsection{Identities}
% \begin{equation}
%     \int q(m) \prod_{k=1}^K f_k(\ldots)^{m_k} \diff m = \sum_{k=1}^K q(e_k) f_k(\ldots)
% \end{equation}
% \begin{equation}
%     \int \prod_{k=1}^K f\big(\ldots, m, \ldots\big)^{m_k} \diff m = \sum_{k=1}^K f(\ldots, m=e_k, \ldots)
% \end{equation}






















% \section{Derivations}

% \subsection{Variational posterior}
% \begin{equation}
%     q_a(y, \bm{x}, m) = q(m) q(y, \bm{x}\midi m) = q(m)\prod_{k=1}^K q_k(y, x_k)^{m_k}
% \end{equation}

% \subsection{Node factorization}
% \begin{equation}
%     f_a(y, \bm{x}, m) = \prod_{k=1}^K f_k(y, x_k)^{m_k}
% \end{equation}

% \subsection{Node-local Bethe free energy}
% \begin{equation}
% \begin{split}
%     \mathrm{F}[q_a,f_a] 
%     &= \int q_a(y, \bm{x}, m) \ln \frac{q_a(y, \bm{x}, m)}{f_a(y, \bm{x}, m)} \, \mathrm{d}y \, \mathrm{d}\bm{x} \, \mathrm{d}m \\
%     &= \sum_{k=1}^K \int q(m_k)\prod_{k=1}^K q_k(y, x_k)^{m_k} \ln \left(\frac{q(m_k)\prod_{k=1}^K q_k(y, x_k)^{m_k}}{\prod_{k=1}^K f_k(y,x_k)^{m_k}} \right)\, \mathrm{d}y \, \mathrm{d}\bm{x} \\
%     &= \sum_{k=1}^K q(m_k) \ln q(m_k) + \sum_{k=1}^K q(m_k) \int q_k(y,x_k) \ln q_k(y,x_k) \mathrm{d}y \mathrm{d}x_k \\
%     &\qquad - \sum_{k=1}^K q(m_k) \int q_k(y,x_k)\ln f_k(y, x_k) \mathrm{d}y \, \mathrm{d}x_k
% \end{split}
% \end{equation}


% \subsection{Constraints}
% Normalization constraints
% \begin{equation}
%     \lambda_m\left(\int q(m) \mathrm{d}m  - 1\right)
% \end{equation}
% \begin{equation}
%     \sum_{k=1}^K \lambda_k \left(\int q_k(y, x_k) \mathrm{d}y\, \mathrm{d}x_k - 1\right)
% \end{equation}

% Marginalization constraint
% \begin{equation}
%     \int \lambda_y(y) \left(\int q_a(y, \bm{x},m) \mathrm{d}\bm{x} \, \mathrm{d}m - q(y)\right) \mathrm{d}y
% \end{equation}
% \begin{equation}
%     \sum_{k=1}^K \int \lambda_{x_k}(x_k) \left(\int q_k(y,x_k) \mathrm{d}y  -q(x_k)\right)\mathrm{d}x_k
% \end{equation}
% \begin{equation}
%     \int \lambda_m(m) \left(\int q_a(y, \bm{x}, m)\mathrm{d}y \mathrm{d}\bm{x} - q(m)\right) \mathrm{d}m
% \end{equation}

% \subsection{Lagrangian}
% \begin{equation}
% \begin{split}
%     \mathrm{L}[q_a, f_a] 
%     &= \mathrm{F}[q_a, f_a] + \lambda_m\left(\sum_{k=1}^K q(m_k) -1\right) + \sum_{k=1}^K \lambda_k\left(\int q_k(y, x_k) \mathrm{d}y\mathrm{d}x_k - 1\right) \\
%     &\qquad + \int \lambda_y(y) \left(\sum_{k=1}^K\int q_a(y, \bm{x}, m_k)\mathrm{d}x_k - q(y)\right)\mathrm{d}y \\
%     &\qquad + \sum_{k=1}^K \int \lambda_{x_k}(x_k) \left(\int q_k(y,x_k) \mathrm{d}y  -q(x_k)\right)\mathrm{d}x_k \\
%     &\qquad + \int \lambda_m(m) \left(\int q_a(y, \bm{x}, m)\mathrm{d}y \mathrm{d}\bm{x} - q(m)\right) \mathrm{d}m
% \end{split}
% \end{equation}

% \subsection{Functional derivatives}

% \subsubsection{With respect to $q(m)$}
% \begin{equation}
%     \begin{split}
%         &\frac{\mathrm{d}\mathrm{L}[q(m) + \varepsilon\phi(m)]}{\mathrm{d}\varepsilon} \Bigg\vert_{\varepsilon = 0} \\
%         &\quad = \frac{\mathrm{d}}{\mathrm{d}\varepsilon} \Bigg[\sum_{k=1}^K \big(q(m_k) + \varepsilon \phi(m_k)\big) \ln \big(q(m_k) + \varepsilon \phi(m_k)\big) \\ 
%         &\qquad \qquad + \sum_{k=1}^K \big(q(m_k) + \varepsilon \phi(m_k)\big) \int q_k(y, x_k) \ln q_k(y,x_k) \mathrm{d}y \mathrm{d}x_k \\
%         &\qquad \qquad - \sum_{k=1}^K \big(q(m_k) + \varepsilon \phi(m_k)\big)\int q_k(y, x_k) \ln f_k(y,x_k) \mathrm{d}y\mathrm{d}x_k \\
%         &\qquad \qquad + \lambda_m \left(\sum_{k=1}^K \big(q(m_k) + \varepsilon \phi(m_k)\big) - 1\right) \\
%         &\qquad \qquad + \sum_{k=1}^K \lambda_m(m_k) \left(\int q_a(y, \bm{x}, m_k)\mathrm{d}y\mathrm{d}\bm{x} - \big(q(m_k) - \varepsilon \phi(m_k)\big)\right) + C\Bigg]_{\varepsilon=0} \\
%         &\quad = \Bigg[ \sum_{k=1}^K \phi(m_k)\ln \big(q(m_k) + \varepsilon \phi(m_k)\big) + \sum_{k=1}^K \phi(m_k) + \sum_{k=1}^K \phi(m_k)\int q_k(y, x_k) \ln q_k(y, x_k) \mathrm{d}y\mathrm{d}x_k \\
%         &\qquad \qquad - \sum_{k=1}^K \phi(m_k) \int q_k(y, x_k) \ln f_k(y,x_k) \mathrm{d}y\mathrm{d}x_k + \lambda_m \sum_{k=1}^K \phi(m_k) + \sum_{k=1}^K \lambda_m(m_k)\phi(m_k)\Bigg]_{\varepsilon=0} \\
%         &\quad = \int \phi(m) \underbrace{\left(\ln q(m) + 1 + \sum_{k=1}^K \left(\int q_k(y,x_k)\ln \frac{q_k(y, x_k)}{f_k(y,x_k)}\mathrm{d}y\mathrm{d}x_k\right)^{m_k} + \lambda_m + \lambda_m(m) \right)}_{\frac{\delta\mathrm{L}}{\delta q(m)}}
%     \end{split}
% \end{equation}

% \begin{equation}
%     q(m) = \exp\left\{-1-\lambda_m\right\}\exp\left\{-\lambda_m(m)\right\}\prod_{k=1}^K \left(\exp\left\{ - \int q_k(y,x_k) \ln \frac{q_k(y,x_k)}{f_k(y,x_k)} \mathrm{d}y\mathrm{d}x_k\right\}\right)^{m_k}
% \end{equation}


% \subsubsection{With respect to $q(y)$}
% \begin{equation}
%     \begin{split}
%         &\frac{\mathrm{d}\mathrm{L}[q(y) + \varepsilon \phi(y)]}{\mathrm{d}\varepsilon}\Bigg\vert_{\varepsilon=0}\\
%         &\quad = \frac{\mathrm{d}}{\mathrm{d}\varepsilon}\Bigg[\Bigg]_{\varepsilon=0} \\
%         &\quad = \int \phi(y) \left(\ln q(y) + 1 + \lambda_y + \lambda_y(y)  \prod_{k=1}^K \lambda_m(e_k) \ln \int \exp\{-\lambda_{x_k}(x_k)\}f_k(y,x_k)\mathrm{d}x_k\right) \\
%         &\quad = \int \phi(y) \underbrace{\left(\ln q(y) + 1 + \lambda_y + \lambda_y(y)   + \ln\left(\sum_{k=1}^K \lambda_m(e_k) \int \exp\{-\lambda_{x_k}(x_k)\}f_k(y,x_k)\mathrm{d}x_k\right)\right)}_{\frac{\delta\mathrm{L}}{\delta q(y)}} \mathrm{d}y \\
%     \end{split}
% \end{equation}

% \begin{equation}
%     q(y) = \exp\{-1-\lambda_y\}\exp\left\{-\lambda_y(y)\right\} \sum_{k=1}^K \left(\exp\{-\lambda_m(e_k)\}\int \exp\left\{-\lambda_{x_k}(x_k)\right\} f_k(y,x_k)\mathrm{d}x_k \right)
% \end{equation}

% \begin{equation}
%     \boxed{
%         q(y) = \frac{\displaystyle \cev{\mu}_y(y) \sum_{k=1}^K \left(\vec{\mu}_m(e_k)\int \vec{\mu}_{x_k}(x_k)f_k(y,x_k)\mathrm{d}x_k\right) }{\displaystyle \int\cev{\mu}_y(y) \sum_{k=1}^K \left(\vec{\mu}_m(e_k)\int \vec{\mu}_{x_k}(x_k)f_k(y,x_k)\mathrm{d}x_k \right)\mathrm{d}y}
%     }
% \end{equation}

% \subsubsection{With respect to $q(y)$ (approach 2)}

% \begin{equation}
%     \begin{split}
%         &\frac{\mathrm{d}\mathrm{L}[q(y) + \varepsilon \phi(y)]}{\mathrm{d}\varepsilon} \Bigg\vert_{\varepsilon=0} \\
%         &\quad = \\
%         &\quad = \frac{\mathrm{d}}{\mathrm{d}\varepsilon} \Bigg[\Bigg]_{\varepsilon=0} \\
%         &\quad = \int \phi(y) \underbrace{\left( \ln q(y) + 1 + \lambda_y + \ln \left(\sum_{k=1}^K \exp\{-\lambda_m(e_k)\}\int q_k(y, x_k) \mathrm{d}x_k\right)\right)}_{\frac{\delta \mathrm{L}}{\delta q(y)}} \mathrm{d}y
%     \end{split}
% \end{equation}

% \begin{equation}
%     q(y) = \exp\{-1 - \lambda_y\} \sum_{k=1}^K \exp\left\{-\lambda_m(e_k)\right\} \int q_k(y,x_k) \mathrm{d}x_k
% \end{equation}

% \begin{equation}
%     \boxed{
%         q(y) = \frac{\displaystyle \sum_{k=1}^K \vec{\mu}_m(e_k) \int q_k(y,x_k)\mathrm{d}x_k}{ \displaystyle \int \sum_{k=1}^K \lambda_m(e_k) \int q_k(y, x_k)\mathrm{d}x_k \mathrm{d}y}
%     }
% \end{equation}

% \subsubsection{With respect to $q(y)$ approach 3}

% \begin{equation}
%     q(y) = \exp\{-1 - \lambda_y\}
% \end{equation}
% \begin{equation}
%     q(y) \propto \sum_m \left(\vec{\mu}_m(m) \prod_{k=1}^K \left(\int q_k(y,x_k)\mathrm{d}x_k\right)^{[m=k]}\right)
% \end{equation}
% \begin{equation}
%     q(y) \propto \sum_{k=1}^K \left(\vec{\mu}_m(k) \prod_{n=1}^K \left( \int q_n(y,x_n) \mathrm{d}x_n\right)^{[n=k]}\right)
% \end{equation}
% \begin{equation}
%     q(y) \propto \sum_{k=1}^K \left(\vec{\mu}_m(k) \int q_k(y,x_k) \mathrm{d}x_k\right)
% \end{equation}
% % \begin{equation}
% %     \boxed{
% %         q(y) = \frac{\displaystyle \prod_{k=1}^K\vec{\mu}_m(m_k=1)^{m_k}\prod_{k=1}^K\left(\int q_k(y,x_k)\mathrm{d}x_k \right)^{m_k} }{Z}
% %     }
% % \end{equation}

% \subsubsection{With respect to $q(m)$}

% \begin{equation}
%     \boxed{
%         q(m) = \frac{\displaystyle \vec{\mu}_m(m)\left(\prod_{k=1}^K \exp\left\{\right\}^{m_k} \right)}{\displaystyle}
%     }
% \end{equation}


% \subsubsection{With respect to $q(x_k)$}

% \begin{equation}
%     \boxed{
%         q(x_k) = \frac{\lambda_{x_k}(x_k) }{\int \lambda_{x_k}(x_k) }
%     }
% \end{equation}

==> styling/journalnames.tex <==
%%Updated on 17 November 2022
%,% Website Name,%,%,% Website Name,%%,% Full Name,%%,% Short Name,%%,% DOI abbr,%%,% ISSN,% \continuouspages
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{acoustics}{\gdef\@journal{acoustics}\gdef\@journalfull{Acoustics}\gdef\@journalshort{Acoustics}\gdef\@doiabbr{acoustics}\gdef\@ISSN{2624-599X}\gdef\@continuouspages{yes}}
\DeclareOption{actuators}{\gdef\@journal{actuators}\gdef\@journalfull{Actuators}\gdef\@journalshort{Actuators}\gdef\@doiabbr{act}\gdef\@ISSN{2076-0825}}
\DeclareOption{addictions}{\gdef\@journal{addictions}\gdef\@journalfull{Addictions}\gdef\@journalshort{Addictions}\gdef\@doiabbr{}\gdef\@ISSN{0006-0006}}
\DeclareOption{admsci}{\gdef\@journal{admsci}\gdef\@journalfull{Administrative Sciences}\gdef\@journalshort{Adm. Sci.}\gdef\@doiabbr{admsci}\gdef\@ISSN{2076-3387}}
\DeclareOption{adolescents}{\gdef\@journal{adolescents}\gdef\@journalfull{Adolescents}\gdef\@journalshort{Adolescents}\gdef\@doiabbr{adolescents}\gdef\@ISSN{2673-7051}\gdef\@continuouspages{yes}}
\DeclareOption{aerobiology}{\gdef\@journal{aerobiology}\gdef\@journalfull{Aerobiology}\gdef\@journalshort{Aerobiology}\gdef\@doiabbr{aerobiology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{aerospace}{\gdef\@journal{aerospace}\gdef\@journalfull{Aerospace}\gdef\@journalshort{Aerospace}\gdef\@doiabbr{aerospace}\gdef\@ISSN{2226-4310}}
\DeclareOption{agriculture}{\gdef\@journal{agriculture}\gdef\@journalfull{Agriculture}\gdef\@journalshort{Agriculture}\gdef\@doiabbr{agriculture}\gdef\@ISSN{2077-0472}}
\DeclareOption{agriengineering}{\gdef\@journal{agriengineering}\gdef\@journalfull{AgriEngineering}\gdef\@journalshort{AgriEngineering}\gdef\@doiabbr{agriengineering}\gdef\@ISSN{2624-7402}\gdef\@continuouspages{yes}}
\DeclareOption{agrochemicals}{\gdef\@journal{agrochemicals}\gdef\@journalfull{Agrochemicals}\gdef\@journalshort{Agrochemicals}\gdef\@doiabbr{agrochemicals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{agronomy}{\gdef\@journal{agronomy}\gdef\@journalfull{Agronomy}\gdef\@journalshort{Agronomy}\gdef\@doiabbr{agronomy}\gdef\@ISSN{2073-4395}}
\DeclareOption{ai}{\gdef\@journal{ai}\gdef\@journalfull{AI}\gdef\@journalshort{AI}\gdef\@doiabbr{ai}\gdef\@ISSN{2673-2688}\gdef\@continuouspages{yes}}
\DeclareOption{air}{\gdef\@journal{air}\gdef\@journalfull{Air}\gdef\@journalshort{Air}\gdef\@doiabbr{air}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{algorithms}{\gdef\@journal{algorithms}\gdef\@journalfull{Algorithms}\gdef\@journalshort{Algorithms}\gdef\@doiabbr{a}\gdef\@ISSN{1999-4893}}
\DeclareOption{allergies}{\gdef\@journal{allergies}\gdef\@journalfull{Allergies}\gdef\@journalshort{Allergies}\gdef\@doiabbr{allergies}\gdef\@ISSN{2313-5786}}
\DeclareOption{alloys}{\gdef\@journal{alloys}\gdef\@journalfull{Alloys}\gdef\@journalshort{Alloys}\gdef\@doiabbr{alloys}\gdef\@ISSN{2674-063X}\gdef\@continuouspages{yes}}
\DeclareOption{analytica}{\gdef\@journal{analytica}\gdef\@journalfull{Analytica}\gdef\@journalshort{Analytica}\gdef\@doiabbr{analytica}\gdef\@ISSN{2673-4532}\gdef\@continuouspages{yes}}
\DeclareOption{analytics}{\gdef\@journal{analytics}\gdef\@journalfull{Analytics}\gdef\@journalshort{Analytics}\gdef\@doiabbr{analytics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{anatomia}{\gdef\@journal{anatomia}\gdef\@journalfull{Anatomia}\gdef\@journalshort{Anatomia}\gdef\@doiabbr{anatomia}\gdef\@ISSN{2813-0545}\gdef\@continuouspages{yes}}
\DeclareOption{animals}{\gdef\@journal{animals}\gdef\@journalfull{Animals}\gdef\@journalshort{Animals}\gdef\@doiabbr{ani}\gdef\@ISSN{2076-2615}}
\DeclareOption{antibiotics}{\gdef\@journal{antibiotics}\gdef\@journalfull{Antibiotics}\gdef\@journalshort{Antibiotics}\gdef\@doiabbr{antibiotics}\gdef\@ISSN{2079-6382}}
\DeclareOption{antibodies}{\gdef\@journal{antibodies}\gdef\@journalfull{Antibodies}\gdef\@journalshort{Antibodies}\gdef\@doiabbr{antib}\gdef\@ISSN{2073-4468}}
\DeclareOption{antioxidants}{\gdef\@journal{antioxidants}\gdef\@journalfull{Antioxidants}\gdef\@journalshort{Antioxidants}\gdef\@doiabbr{antiox}\gdef\@ISSN{2076-3921}}
\DeclareOption{applbiosci}{\gdef\@journal{applbiosci}\gdef\@journalfull{Applied Biosciences}\gdef\@journalshort{Appl. Biosci.}\gdef\@doiabbr{applbiosci}\gdef\@ISSN{2813-0464}\gdef\@continuouspages{yes}}
\DeclareOption{appliedchem}{\gdef\@journal{appliedchem}\gdef\@journalfull{AppliedChem}\gdef\@journalshort{AppliedChem}\gdef\@doiabbr{appliedchem}\gdef\@ISSN{2673-9623}\gdef\@continuouspages{yes}}
\DeclareOption{appliedmath}{\gdef\@journal{appliedmath}\gdef\@journalfull{AppliedMath}\gdef\@journalshort{AppliedMath}\gdef\@doiabbr{appliedmath}\gdef\@ISSN{2673-9909}\gdef\@continuouspages{yes}}
\DeclareOption{applmech}{\gdef\@journal{applmech}\gdef\@journalfull{Applied Mechanics}\gdef\@journalshort{Appl. Mech.}\gdef\@doiabbr{applmech}\gdef\@ISSN{2673-3161}\gdef\@continuouspages{yes}}
\DeclareOption{applmicrobiol}{\gdef\@journal{applmicrobiol}\gdef\@journalfull{Applied Microbiology}\gdef\@journalshort{Appl. Microbiol.}\gdef\@doiabbr{applmicrobiol}\gdef\@ISSN{2673-8007}\gdef\@continuouspages{yes}}
\DeclareOption{applnano}{\gdef\@journal{applnano}\gdef\@journalfull{Applied Nano}\gdef\@journalshort{Appl. Nano}\gdef\@doiabbr{applnano}\gdef\@ISSN{2673-3501}\gdef\@continuouspages{yes}}
\DeclareOption{applsci}{\gdef\@journal{applsci}\gdef\@journalfull{Applied Sciences}\gdef\@journalshort{Appl. Sci.}\gdef\@doiabbr{app}\gdef\@ISSN{2076-3417}}
\DeclareOption{aquacj}{\gdef\@journal{aquacj}\gdef\@journalfull{Aquaculture Journal}\gdef\@journalshort{Aquac. J.}\gdef\@doiabbr{aj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{architecture}{\gdef\@journal{architecture}\gdef\@journalfull{Architecture}\gdef\@journalshort{Architecture}\gdef\@doiabbr{architecture}\gdef\@ISSN{2673-8945}\gdef\@continuouspages{yes}}
\DeclareOption{arm}{\gdef\@journal{arm}\gdef\@journalfull{Advances in Respiratory Medicine}\gdef\@journalshort{Adv. Respir. Med.}\gdef\@doiabbr{arm}\gdef\@ISSN{2543-6031}\gdef\@continuouspages{yes}}
\DeclareOption{arthropoda}{\gdef\@journal{arthropoda}\gdef\@journalfull{Arthropoda}\gdef\@journalshort{Arthropoda}\gdef\@doiabbr{arthropoda}\gdef\@ISSN{2813-3323}\gdef\@continuouspages{yes}}
\DeclareOption{arts}{\gdef\@journal{arts}\gdef\@journalfull{Arts}\gdef\@journalshort{Arts}\gdef\@doiabbr{arts}\gdef\@ISSN{2076-0752}}
\DeclareOption{asc}{\gdef\@journal{asc}\gdef\@journalfull{Automatic Systems and Control}\gdef\@journalshort{Autom. Syst. Control}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{asi}{\gdef\@journal{asi}\gdef\@journalfull{Applied System Innovation}\gdef\@journalshort{Appl. Syst. Innov.}\gdef\@doiabbr{asi}\gdef\@ISSN{2571-5577}}
\DeclareOption{astronomy}{\gdef\@journal{astronomy}\gdef\@journalfull{Astronomy}\gdef\@journalshort{Astronomy}\gdef\@doiabbr{astronomy}\gdef\@ISSN{2674-0346}\gdef\@continuouspages{yes}}
\DeclareOption{atmosphere}{\gdef\@journal{atmosphere}\gdef\@journalfull{Atmosphere}\gdef\@journalshort{Atmosphere}\gdef\@doiabbr{atmos}\gdef\@ISSN{2073-4433}}
\DeclareOption{atoms}{\gdef\@journal{atoms}\gdef\@journalfull{Atoms}\gdef\@journalshort{Atoms}\gdef\@doiabbr{atoms}\gdef\@ISSN{2218-2004}}
\DeclareOption{audiolres}{\gdef\@journal{audiolres}\gdef\@journalfull{Audiology Research}\gdef\@journalshort{Audiol. Res.}\gdef\@doiabbr{audiolres}\gdef\@ISSN{2039-4349}\gdef\@continuouspages{yes}}
\DeclareOption{automation}{\gdef\@journal{automation}\gdef\@journalfull{Automation}\gdef\@journalshort{Automation}\gdef\@doiabbr{automation}\gdef\@ISSN{2673-4052}\gdef\@continuouspages{yes}}
\DeclareOption{axioms}{\gdef\@journal{axioms}\gdef\@journalfull{Axioms}\gdef\@journalshort{Axioms}\gdef\@doiabbr{axioms}\gdef\@ISSN{2075-1680}}
\DeclareOption{bacteria}{\gdef\@journal{bacteria}\gdef\@journalfull{Bacteria}\gdef\@journalshort{Bacteria}\gdef\@doiabbr{bacteria}\gdef\@ISSN{2674-1334}\gdef\@continuouspages{yes}}
\DeclareOption{batteries}{\gdef\@journal{batteries}\gdef\@journalfull{Batteries}\gdef\@journalshort{Batteries}\gdef\@doiabbr{batteries}\gdef\@ISSN{2313-0105}}
\DeclareOption{bdcc}{\gdef\@journal{bdcc}\gdef\@journalfull{Big Data and Cognitive Computing}\gdef\@journalshort{Big Data Cogn. Comput.}\gdef\@doiabbr{bdcc}\gdef\@ISSN{2504-2289}}
\DeclareOption{behavsci}{\gdef\@journal{behavsci}\gdef\@journalfull{Behavioral Sciences}\gdef\@journalshort{Behav. Sci.}\gdef\@doiabbr{bs}\gdef\@ISSN{2076-328X}}
\DeclareOption{beverages}{\gdef\@journal{beverages}\gdef\@journalfull{Beverages}\gdef\@journalshort{Beverages}\gdef\@doiabbr{beverages}\gdef\@ISSN{2306-5710}}
\DeclareOption{biochem}{\gdef\@journal{biochem}\gdef\@journalfull{BioChem}\gdef\@journalshort{BioChem}\gdef\@doiabbr{biochem}\gdef\@ISSN{2673-6411}\gdef\@continuouspages{yes}}
\DeclareOption{bioengineering}{\gdef\@journal{bioengineering}\gdef\@journalfull{Bioengineering}\gdef\@journalshort{Bioengineering}\gdef\@doiabbr{bioengineering}\gdef\@ISSN{2306-5354}}
\DeclareOption{biologics}{\gdef\@journal{biologics}\gdef\@journalfull{Biologics}\gdef\@journalshort{Biologics}\gdef\@doiabbr{biologics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biology}{\gdef\@journal{biology}\gdef\@journalfull{Biology}\gdef\@journalshort{Biology}\gdef\@doiabbr{biology}\gdef\@ISSN{2079-7737}}
\DeclareOption{biomass}{\gdef\@journal{biomass}\gdef\@journalfull{Biomass}\gdef\@journalshort{Biomass}\gdef\@doiabbr{biomass}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomechanics}{\gdef\@journal{biomechanics}\gdef\@journalfull{Biomechanics}\gdef\@journalshort{Biomechanics}\gdef\@doiabbr{biomechanics}\gdef\@ISSN{2673-7078}\gdef\@continuouspages{yes}}
\DeclareOption{biomed}{\gdef\@journal{biomed}\gdef\@journalfull{BioMed}\gdef\@journalshort{BioMed}\gdef\@doiabbr{biomed}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomedicines}{\gdef\@journal{biomedicines}\gdef\@journalfull{Biomedicines}\gdef\@journalshort{Biomedicines}\gdef\@doiabbr{biomedicines}\gdef\@ISSN{2227-9059}}
\DeclareOption{biomedinformatics}{\gdef\@journal{biomedinformatics}\gdef\@journalfull{Biomedinformatics}\gdef\@journalshort{Biomedinformatics}\gdef\@doiabbr{biomedinformatics}\gdef\@ISSN{2673-7426}\gdef\@continuouspages{yes}}
\DeclareOption{biomimetics}{\gdef\@journal{biomimetics}\gdef\@journalfull{Biomimetics}\gdef\@journalshort{Biomimetics}\gdef\@doiabbr{biomimetics}\gdef\@ISSN{2313-7673}}
\DeclareOption{biomolecules}{\gdef\@journal{biomolecules}\gdef\@journalfull{Biomolecules}\gdef\@journalshort{Biomolecules}\gdef\@doiabbr{biom}\gdef\@ISSN{2218-273X}}
\DeclareOption{biophysica}{\gdef\@journal{biophysica}\gdef\@journalfull{Biophysica}\gdef\@journalshort{Biophysica}\gdef\@doiabbr{biophysica}\gdef\@ISSN{2673-4125}\gdef\@continuouspages{yes}}
\DeclareOption{biosensors}{\gdef\@journal{biosensors}\gdef\@journalfull{Biosensors}\gdef\@journalshort{Biosensors}\gdef\@doiabbr{bios}\gdef\@ISSN{2079-6374}}
\DeclareOption{biotech}{\gdef\@journal{biotech}\gdef\@journalfull{BioTech}\gdef\@journalshort{BioTech}\gdef\@doiabbr{biotech}\gdef\@ISSN{2673-6284}}
\DeclareOption{birds}{\gdef\@journal{birds}\gdef\@journalfull{Birds}\gdef\@journalshort{Birds}\gdef\@doiabbr{birds}\gdef\@ISSN{2673-6004}\gdef\@continuouspages{yes}}
\DeclareOption{bloods}{\gdef\@journal{bloods}\gdef\@journalfull{Bloods}\gdef\@journalshort{Bloods}\gdef\@doiabbr{bloods}\gdef\@ISSN{2673-415X}}
\DeclareOption{blsf}{\gdef\@journal{blsf}\gdef\@journalfull{Biology and Life Sciences Forum}\gdef\@journalshort{Biol. Life Sci. Forum}\gdef\@doiabbr{blsf	}\gdef\@ISSN{2673-9976}}
\DeclareOption{brainsci}{\gdef\@journal{brainsci}\gdef\@journalfull{Brain Sciences}\gdef\@journalshort{Brain Sci.}\gdef\@doiabbr{brainsci}\gdef\@ISSN{2076-3425}}
\DeclareOption{breath}{\gdef\@journal{breath}\gdef\@journalfull{Breath}\gdef\@journalshort{Breath}\gdef\@doiabbr{breath}\gdef\@ISSN{}}
\DeclareOption{buildings}{\gdef\@journal{buildings}\gdef\@journalfull{Buildings}\gdef\@journalshort{Buildings}\gdef\@doiabbr{buildings}\gdef\@ISSN{2075-5309}}
\DeclareOption{businesses}{\gdef\@journal{businesses}\gdef\@journalfull{Businesses}\gdef\@journalshort{Businesses}\gdef\@doiabbr{businesses}\gdef\@ISSN{2673-7116}\gdef\@continuouspages{yes}}
\DeclareOption{cancers}{\gdef\@journal{cancers}\gdef\@journalfull{Cancers}\gdef\@journalshort{Cancers}\gdef\@doiabbr{cancers}\gdef\@ISSN{2072-6694}}
\DeclareOption{carbon}{\gdef\@journal{carbon}\gdef\@journalfull{C}\gdef\@journalshort{C}\gdef\@doiabbr{c}\gdef\@ISSN{2311-5629}}
\DeclareOption{cardiogenetics}{\gdef\@journal{cardiogenetics}\gdef\@journalfull{Cardiogenetics}\gdef\@journalshort{Cardiogenetics}\gdef\@doiabbr{cardiogenetics}\gdef\@ISSN{2035-8148}\gdef\@continuouspages{yes}}
\DeclareOption{catalysts}{\gdef\@journal{catalysts}\gdef\@journalfull{Catalysts}\gdef\@journalshort{Catalysts}\gdef\@doiabbr{catal}\gdef\@ISSN{2073-4344}}
\DeclareOption{cells}{\gdef\@journal{cells}\gdef\@journalfull{Cells}\gdef\@journalshort{Cells}\gdef\@doiabbr{cells}\gdef\@ISSN{2073-4409}}
\DeclareOption{ceramics}{\gdef\@journal{ceramics}\gdef\@journalfull{Ceramics}\gdef\@journalshort{Ceramics}\gdef\@doiabbr{ceramics}\gdef\@ISSN{2571-6131}\gdef\@continuouspages{yes}}
\DeclareOption{challenges}{\gdef\@journal{challenges}\gdef\@journalfull{Challenges}\gdef\@journalshort{Challenges}\gdef\@doiabbr{challe}\gdef\@ISSN{2078-1547}}
\DeclareOption{chemengineering}{\gdef\@journal{chemengineering}\gdef\@journalfull{ChemEngineering}\gdef\@journalshort{ChemEngineering}\gdef\@doiabbr{chemengineering}\gdef\@ISSN{2305-7084}}
\DeclareOption{chemistry}{\gdef\@journal{chemistry}\gdef\@journalfull{Chemistry}\gdef\@journalshort{Chemistry}\gdef\@doiabbr{chemistry}\gdef\@ISSN{2624-8549}\gdef\@continuouspages{yes}}
\DeclareOption{chemosensors}{\gdef\@journal{chemosensors}\gdef\@journalfull{Chemosensors}\gdef\@journalshort{Chemosensors}\gdef\@doiabbr{chemosensors}\gdef\@ISSN{2227-9040}}
\DeclareOption{chemproc}{\gdef\@journal{chemproc}\gdef\@journalfull{Chemistry Proceedings}\gdef\@journalshort{Chem. Proc.}\gdef\@doiabbr{chemproc}\gdef\@ISSN{2673-4583}}
\DeclareOption{children}{\gdef\@journal{children}\gdef\@journalfull{Children}\gdef\@journalshort{Children}\gdef\@doiabbr{children}\gdef\@ISSN{2227-9067}}
\DeclareOption{chips}{\gdef\@journal{chips}\gdef\@journalfull{Chips}\gdef\@journalshort{Chips}\gdef\@doiabbr{chips}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{cimb}{\gdef\@journal{cimb}\gdef\@journalfull{Current Issues in Molecular Biology}\gdef\@journalshort{Curr. Issues Mol. Biol.}\gdef\@doiabbr{cimb}\gdef\@ISSN{1467-3045}\gdef\@continuouspages{yes}}
\DeclareOption{civileng}{\gdef\@journal{civileng}\gdef\@journalfull{CivilEng}\gdef\@journalshort{CivilEng}\gdef\@doiabbr{civileng}\gdef\@ISSN{2673-4109}\gdef\@continuouspages{yes}}
\DeclareOption{cleantechnol}{\gdef\@journal{cleantechnol}\gdef\@journalfull{Clean Technologies}\gdef\@journalshort{Clean Technol.}\gdef\@doiabbr{cleantechnol}\gdef\@ISSN{2571-8797}\gdef\@continuouspages{yes}}
\DeclareOption{climate}{\gdef\@journal{climate}\gdef\@journalfull{Climate}\gdef\@journalshort{Climate}\gdef\@doiabbr{cli}\gdef\@ISSN{2225-1154}}
\DeclareOption{clinpract}{\gdef\@journal{clinpract}\gdef\@journalfull{Clinics and Practice}\gdef\@journalshort{Clin. Pract.}\gdef\@doiabbr{clinpract}\gdef\@ISSN{2039-7283}\gdef\@continuouspages{yes}}
\DeclareOption{clockssleep}{\gdef\@journal{clockssleep}\gdef\@journalfull{Clocks \& Sleep}\gdef\@journalshort{Clocks\&Sleep}\gdef\@doiabbr{clockssleep}\gdef\@ISSN{2624-5175}\gdef\@continuouspages{yes}}
\DeclareOption{cmd}{\gdef\@journal{cmd}\gdef\@journalfull{Corrosion and Materials Degradation}\gdef\@journalshort{Corros. Mater. Degrad.}\gdef\@doiabbr{cmd}\gdef\@ISSN{2624-5558}\gdef\@continuouspages{yes}}
\DeclareOption{coasts}{\gdef\@journal{coasts}\gdef\@journalfull{Coasts}\gdef\@journalshort{Coasts}\gdef\@doiabbr{coasts}\gdef\@ISSN{2673-964X}\gdef\@continuouspages{yes}}
\DeclareOption{coatings}{\gdef\@journal{coatings}\gdef\@journalfull{Coatings}\gdef\@journalshort{Coatings}\gdef\@doiabbr{coatings}\gdef\@ISSN{2079-6412}}
\DeclareOption{colloids}{\gdef\@journal{colloids}\gdef\@journalfull{Colloids Interfaces}\gdef\@journalshort{Colloids Interfaces}\gdef\@doiabbr{colloids}\gdef\@ISSN{2504-5377}}
\DeclareOption{colorants}{\gdef\@journal{colorants}\gdef\@journalfull{Colorants}\gdef\@journalshort{Colorants}\gdef\@doiabbr{colorants}\gdef\@ISSN{2079-6447}\gdef\@continuouspages{yes}}
\DeclareOption{commodities}{\gdef\@journal{commodities}\gdef\@journalfull{Commodities}\gdef\@journalshort{Commodities}\gdef\@doiabbr{commodities}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{compounds}{\gdef\@journal{compounds}\gdef\@journalfull{Compounds}\gdef\@journalshort{Compounds}\gdef\@doiabbr{compounds}\gdef\@ISSN{2673-6918}\gdef\@continuouspages{yes}}
\DeclareOption{computation}{\gdef\@journal{computation}\gdef\@journalfull{Computation}\gdef\@journalshort{Computation}\gdef\@doiabbr{computation}\gdef\@ISSN{2079-3197}}
\DeclareOption{computers}{\gdef\@journal{computers}\gdef\@journalfull{Computers}\gdef\@journalshort{Computers}\gdef\@doiabbr{computers}\gdef\@ISSN{2073-431X}}
\DeclareOption{condensedmatter}{\gdef\@journal{condensedmatter}\gdef\@journalfull{Condensed Matter}\gdef\@journalshort{Condens. Matter}\gdef\@doiabbr{condmat}\gdef\@ISSN{2410-3896}}
\DeclareOption{conservation}{\gdef\@journal{conservation}\gdef\@journalfull{Conservation}\gdef\@journalshort{Conservation}\gdef\@doiabbr{conservation}\gdef\@ISSN{2673-7159}\gdef\@continuouspages{yes}}
\DeclareOption{constrmater}{\gdef\@journal{constrmater}\gdef\@journalfull{Construction Materials}\gdef\@journalshort{Constr. Mater.}\gdef\@doiabbr{constrmater}\gdef\@ISSN{2673-7108}\gdef\@continuouspages{yes}}
\DeclareOption{cosmetics}{\gdef\@journal{cosmetics}\gdef\@journalfull{Cosmetics}\gdef\@journalshort{Cosmetics}\gdef\@doiabbr{cosmetics}\gdef\@ISSN{2079-9284}}
\DeclareOption{covid}{\gdef\@journal{covid}\gdef\@journalfull{COVID}\gdef\@journalshort{COVID}\gdef\@doiabbr{covid}\gdef\@ISSN{2673-8112}\gdef\@continuouspages{yes}}
\DeclareOption{crops}{\gdef\@journal{crops}\gdef\@journalfull{Crops}\gdef\@journalshort{Crops}\gdef\@doiabbr{crops}\gdef\@ISSN{2673-7655}\gdef\@continuouspages{yes}}
\DeclareOption{cryptography}{\gdef\@journal{cryptography}\gdef\@journalfull{Cryptography}\gdef\@journalshort{Cryptography}\gdef\@doiabbr{cryptography}\gdef\@ISSN{2410-387X}}
\DeclareOption{crystals}{\gdef\@journal{crystals}\gdef\@journalfull{Crystals}\gdef\@journalshort{Crystals}\gdef\@doiabbr{cryst}\gdef\@ISSN{2073-4352}}
\DeclareOption{csmf}{\gdef\@journal{csmf}\gdef\@journalfull{Computer Sciences \& Mathematics Forum}\gdef\@journalshort{Comput. Sci. Math. Forum}\gdef\@doiabbr{csmf}\gdef\@ISSN{2813-0324}}
\DeclareOption{ctn}{\gdef\@journal{ctn}\gdef\@journalfull{Clinical and Translational Neuroscience}\gdef\@journalshort{Clin. Transl. Neurosci.}\gdef\@doiabbr{ctn}\gdef\@ISSN{2514-183X}}
\DeclareOption{curroncol}{\gdef\@journal{curroncol}\gdef\@journalfull{Current Oncology}\gdef\@journalshort{Curr. Oncol.}\gdef\@doiabbr{curroncol}\gdef\@ISSN{1718-7729}\gdef\@continuouspages{yes}}
\DeclareOption{cyber}{\gdef\@journal{cyber}\gdef\@journalfull{Cyber}\gdef\@journalshort{Cyber}\gdef\@doiabbr{cyber}\gdef\@ISSN{2624-800X}}
\DeclareOption{dairy}{\gdef\@journal{dairy}\gdef\@journalfull{Dairy}\gdef\@journalshort{Dairy}\gdef\@doiabbr{dairy}\gdef\@ISSN{2624-862X}\gdef\@continuouspages{yes}}
\DeclareOption{data}{\gdef\@journal{data}\gdef\@journalfull{Data}\gdef\@journalshort{Data}\gdef\@doiabbr{data}\gdef\@ISSN{2306-5729}}
\DeclareOption{ddc}{\gdef\@journal{ddc}\gdef\@journalfull{Drugs and Drug Candidates}\gdef\@journalshort{Drugs Drug Candidates}\gdef\@doiabbr{ddc}\gdef\@ISSN{2813-2998}\gdef\@continuouspages{yes}}
\DeclareOption{dentistry}{\gdef\@journal{dentistry}\gdef\@journalfull{Dentistry Journal}\gdef\@journalshort{Dent. J.}\gdef\@doiabbr{dj}\gdef\@ISSN{2304-6767}}
\DeclareOption{dermato}{\gdef\@journal{dermato}\gdef\@journalfull{Dermato}\gdef\@journalshort{Dermato}\gdef\@doiabbr{dermato}\gdef\@ISSN{2673-6179}\gdef\@continuouspages{yes}}
\DeclareOption{dermatopathology}{\gdef\@journal{dermatopathology}\gdef\@journalfull{Dermatopathology}\gdef\@journalshort{Dermatopathology}\gdef\@doiabbr{dermatopathology}\gdef\@ISSN{2296-3529}\gdef\@continuouspages{yes}}
\DeclareOption{designs}{\gdef\@journal{designs}\gdef\@journalfull{Designs}\gdef\@journalshort{Designs}\gdef\@doiabbr{designs}\gdef\@ISSN{2411-9660}}
\DeclareOption{devices}{\gdef\@journal{devices}\gdef\@journalfull{Devices}\gdef\@journalshort{Devices}\gdef\@doiabbr{devices}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{diabetology}{\gdef\@journal{diabetology}\gdef\@journalfull{Diabetology}\gdef\@journalshort{Diabetology}\gdef\@doiabbr{diabetology}\gdef\@ISSN{2673-4540}\gdef\@continuouspages{yes}}
\DeclareOption{diagnostics}{\gdef\@journal{diagnostics}\gdef\@journalfull{Diagnostics}\gdef\@journalshort{Diagnostics}\gdef\@doiabbr{diagnostics}\gdef\@ISSN{2075-4418}}
\DeclareOption{dietetics}{\gdef\@journal{dietetics}\gdef\@journalfull{Dietetics}\gdef\@journalshort{Dietetics}\gdef\@doiabbr{dietetics}\gdef\@ISSN{2674-0311}\gdef\@continuouspages{yes}}
\DeclareOption{digital}{\gdef\@journal{digital}\gdef\@journalfull{Digital}\gdef\@journalshort{Digital}\gdef\@doiabbr{digital}\gdef\@ISSN{2673-6470}\gdef\@continuouspages{yes}}
\DeclareOption{disabilities}{\gdef\@journal{disabilities}\gdef\@journalfull{Disabilities}\gdef\@journalshort{Disabilities}\gdef\@doiabbr{disabilities}\gdef\@ISSN{2673-7272}\gdef\@continuouspages{yes}}
\DeclareOption{diseases}{\gdef\@journal{diseases}\gdef\@journalfull{Diseases}\gdef\@journalshort{Diseases}\gdef\@doiabbr{diseases}\gdef\@ISSN{2079-9721}}
\DeclareOption{diversity}{\gdef\@journal{diversity}\gdef\@journalfull{Diversity}\gdef\@journalshort{Diversity}\gdef\@doiabbr{d}\gdef\@ISSN{1424-2818}}
\DeclareOption{dna}{\gdef\@journal{dna}\gdef\@journalfull{DNA}\gdef\@journalshort{DNA}\gdef\@doiabbr{dna}\gdef\@ISSN{2673-8856}\gdef\@continuouspages{yes}}
\DeclareOption{drones}{\gdef\@journal{drones}\gdef\@journalfull{Drones}\gdef\@journalshort{Drones}\gdef\@doiabbr{drones}\gdef\@ISSN{2504-446X}}
\DeclareOption{dynamics}{\gdef\@journal{dynamics}\gdef\@journalfull{Dynamics}\gdef\@journalshort{Dynamics}\gdef\@doiabbr{dynamics}\gdef\@ISSN{2673-8716}\gdef\@continuouspages{yes}}
\DeclareOption{earth}{\gdef\@journal{earth}\gdef\@journalfull{Earth}\gdef\@journalshort{Earth}\gdef\@doiabbr{earth}\gdef\@ISSN{2673-4834}\gdef\@continuouspages{yes}}
\DeclareOption{ebj}{\gdef\@journal{ebj}\gdef\@journalfull{European Burn Journal}\gdef\@journalshort{Eur. Burn J.}\gdef\@doiabbr{ebj}\gdef\@ISSN{2673-1991}\gdef\@continuouspages{yes}}
\DeclareOption{ecologies}{\gdef\@journal{ecologies}\gdef\@journalfull{Ecologies}\gdef\@journalshort{Ecologies}\gdef\@doiabbr{ecologies}\gdef\@ISSN{2673-4133}\gdef\@continuouspages{yes}}
\DeclareOption{econometrics}{\gdef\@journal{econometrics}\gdef\@journalfull{Econometrics}\gdef\@journalshort{Econometrics}\gdef\@doiabbr{econometrics}\gdef\@ISSN{2225-1146}}
\DeclareOption{economies}{\gdef\@journal{economies}\gdef\@journalfull{Economies}\gdef\@journalshort{Economies}\gdef\@doiabbr{economies}\gdef\@ISSN{2227-7099}}
\DeclareOption{education}{\gdef\@journal{education}\gdef\@journalfull{Education Sciences}\gdef\@journalshort{Educ. Sci.}\gdef\@doiabbr{educsci}\gdef\@ISSN{2227-7102}}
\DeclareOption{ejihpe}{\gdef\@journal{ejihpe}\gdef\@journalfull{European Journal of Investigation in Health Psychology and Education}\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}\gdef\@doiabbr{ejihpe}\gdef\@ISSN{2254-9625}\gdef\@continuouspages{yes}}
\DeclareOption{electricity}{\gdef\@journal{electricity}\gdef\@journalfull{Electricity}\gdef\@journalshort{Electricity}\gdef\@doiabbr{electricity}\gdef\@ISSN{2673-4826}\gdef\@continuouspages{yes}}
\DeclareOption{electrochem}{\gdef\@journal{electrochem}\gdef\@journalfull{Electrochem}\gdef\@journalshort{Electrochem}\gdef\@doiabbr{electrochem}\gdef\@ISSN{2673-3293}\gdef\@continuouspages{yes}}
\DeclareOption{electronicmat}{\gdef\@journal{electronicmat}\gdef\@journalfull{Electronic Materials}\gdef\@journalshort{Electron. Mater.}\gdef\@doiabbr{electronicmat}\gdef\@ISSN{2673-3978}\gdef\@continuouspages{yes}}
\DeclareOption{electronics}{\gdef\@journal{electronics}\gdef\@journalfull{Electronics}\gdef\@journalshort{Electronics}\gdef\@doiabbr{electronics}\gdef\@ISSN{2079-9292}}
\DeclareOption{encyclopedia}{\gdef\@journal{encyclopedia}\gdef\@journalfull{Encyclopedia}\gdef\@journalshort{Encyclopedia}\gdef\@doiabbr{encyclopedia}\gdef\@ISSN{2673-8392}\gdef\@continuouspages{yes}}
\DeclareOption{endocrines}{\gdef\@journal{endocrines}\gdef\@journalfull{Endocrines}\gdef\@journalshort{Endocrines}\gdef\@doiabbr{endocrines}\gdef\@ISSN{2673-396X}\gdef\@continuouspages{yes}}
\DeclareOption{energies}{\gdef\@journal{energies}\gdef\@journalfull{Energies}\gdef\@journalshort{Energies}\gdef\@doiabbr{en}\gdef\@ISSN{1996-1073}}
\DeclareOption{eng}{\gdef\@journal{eng}\gdef\@journalfull{Eng-Advances in Engineering}\gdef\@journalshort{Eng}\gdef\@doiabbr{eng}\gdef\@ISSN{2673-4117}\gdef\@continuouspages{yes}}
\DeclareOption{engproc}{\gdef\@journal{engproc}\gdef\@journalfull{Engineering Proceedings}\gdef\@journalshort{Eng. Proc.}\gdef\@doiabbr{engproc}\gdef\@ISSN{2673-4591}}
%\DeclareOption{ent}{\gdef\@journal{ent}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{entomology}{\gdef\@journal{entomology}\gdef\@journalfull{Entomology}\gdef\@journalshort{Entomology}\gdef\@doiabbr{entomology}\gdef\@ISSN{2813-0502}\gdef\@continuouspages{yes}}	
\DeclareOption{entropy}{\gdef\@journal{entropy}\gdef\@journalfull{Entropy}\gdef\@journalshort{Entropy}\gdef\@doiabbr{e}\gdef\@ISSN{1099-4300}}
\DeclareOption{environments}{\gdef\@journal{environments}\gdef\@journalfull{Environments}\gdef\@journalshort{Environments}\gdef\@doiabbr{environments}\gdef\@ISSN{2076-3298}}
\DeclareOption{environsciproc}{\gdef\@journal{environsciproc}\gdef\@journalfull{Environmental Sciences Proceedings}\gdef\@journalshort{Environ. Sci. Proc.}\gdef\@doiabbr{environsciproc}\gdef\@ISSN{2673-4931}}
\DeclareOption{epidemiologia}{\gdef\@journal{epidemiologia}\gdef\@journalfull{Epidemiologia}\gdef\@journalshort{Epidemiologia}\gdef\@doiabbr{epidemiologia}\gdef\@ISSN{2673-3986}\gdef\@continuouspages{yes}}
\DeclareOption{epigenomes}{\gdef\@journal{epigenomes}\gdef\@journalfull{Epigenomes}\gdef\@journalshort{Epigenomes}\gdef\@doiabbr{epigenomes}\gdef\@ISSN{2075-4655}}
\DeclareOption{est}{\gdef\@journal{est}\gdef\@journalfull{Electrochemical Science and Technology}\gdef\@journalshort{Electrochem. Sci. Technol.}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{fermentation}{\gdef\@journal{fermentation}\gdef\@journalfull{Fermentation}\gdef\@journalshort{Fermentation}\gdef\@doiabbr{fermentation}\gdef\@ISSN{2311-5637}}
\DeclareOption{fibers}{\gdef\@journal{fibers}\gdef\@journalfull{Fibers}\gdef\@journalshort{Fibers}\gdef\@doiabbr{fib}\gdef\@ISSN{2079-6439}}
\DeclareOption{fintech}{\gdef\@journal{fintech}\gdef\@journalfull{FinTech}\gdef\@journalshort{FinTech}\gdef\@doiabbr{fintech}\gdef\@ISSN{2674-1032}\gdef\@continuouspages{yes}}
\DeclareOption{fire}{\gdef\@journal{fire}\gdef\@journalfull{Fire}\gdef\@journalshort{Fire}\gdef\@doiabbr{fire}\gdef\@ISSN{2571-6255}}
\DeclareOption{fishes}{\gdef\@journal{fishes}\gdef\@journalfull{Fishes}\gdef\@journalshort{Fishes}\gdef\@doiabbr{fishes}\gdef\@ISSN{2410-3888}}
\DeclareOption{fluids}{\gdef\@journal{fluids}\gdef\@journalfull{Fluids}\gdef\@journalshort{Fluids}\gdef\@doiabbr{fluids}\gdef\@ISSN{2311-5521}}
\DeclareOption{foods}{\gdef\@journal{foods}\gdef\@journalfull{Foods}\gdef\@journalshort{Foods}\gdef\@doiabbr{foods}\gdef\@ISSN{2304-8158}}
\DeclareOption{forecasting}{\gdef\@journal{forecasting}\gdef\@journalfull{Forecasting}\gdef\@journalshort{Forecasting}\gdef\@doiabbr{forecast}\gdef\@ISSN{2571-9394}\gdef\@continuouspages{yes}}
\DeclareOption{forensicsci}{\gdef\@journal{forensicsci}\gdef\@journalfull{Forensic Sciences}\gdef\@journalshort{Forensic Sci.}\gdef\@doiabbr{forensicsci}\gdef\@ISSN{2673-6756}\gdef\@continuouspages{yes}}
\DeclareOption{forests}{\gdef\@journal{forests}\gdef\@journalfull{Forests}\gdef\@journalshort{Forests}\gdef\@doiabbr{f}\gdef\@ISSN{1999-4907}}
\DeclareOption{foundations}{\gdef\@journal{foundations}\gdef\@journalfull{Foundations}\gdef\@journalshort{Foundations}\gdef\@doiabbr{foundations}\gdef\@ISSN{2673-9321}\gdef\@continuouspages{yes}}
\DeclareOption{fractalfract}{\gdef\@journal{fractalfract}\gdef\@journalfull{Fractal and Fractional}\gdef\@journalshort{Fractal Fract.}\gdef\@doiabbr{fractalfract}\gdef\@ISSN{2504-3110}}
\DeclareOption{fuels}{\gdef\@journal{fuels}\gdef\@journalfull{Fuels}\gdef\@journalshort{Fuels}\gdef\@doiabbr{fuels}\gdef\@ISSN{2673-3994}\gdef\@continuouspages{yes}}
\DeclareOption{future}{\gdef\@journal{future}\gdef\@journalfull{Future}\gdef\@journalshort{Future}\gdef\@doiabbr{future}\gdef\@ISSN{2813-2882}\gdef\@continuouspages{yes}}
\DeclareOption{futureinternet}{\gdef\@journal{futureinternet}\gdef\@journalfull{Future Internet}\gdef\@journalshort{Future Internet}\gdef\@doiabbr{fi}\gdef\@ISSN{1999-5903}}
%\DeclareOption{futureparasites}{\gdef\@journal{futureparasites}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{futurepharmacol}{\gdef\@journal{futurepharmacol}\gdef\@journalfull{Future Pharmacology}\gdef\@journalshort{Future Pharmacol.}\gdef\@doiabbr{futurepharmacol}\gdef\@ISSN{2673-9879}\gdef\@continuouspages{yes}}
\DeclareOption{futurephys}{\gdef\@journal{futurephys}\gdef\@journalfull{Future Physics}\gdef\@journalshort{Future Phys.}\gdef\@doiabbr{futurephys}\gdef\@ISSN{2624-6503}}
\DeclareOption{futuretransp}{\gdef\@journal{futuretransp}\gdef\@journalfull{Future Transportation}\gdef\@journalshort{Future Transp.}\gdef\@doiabbr{futuretransp}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{galaxies}{\gdef\@journal{galaxies}\gdef\@journalfull{Galaxies}\gdef\@journalshort{Galaxies}\gdef\@doiabbr{galaxies}\gdef\@ISSN{2075-4434}}
\DeclareOption{games}{\gdef\@journal{games}\gdef\@journalfull{Games}\gdef\@journalshort{Games}\gdef\@doiabbr{g}\gdef\@ISSN{2073-4336}}
\DeclareOption{gases}{\gdef\@journal{gases}\gdef\@journalfull{Gases}\gdef\@journalshort{Gases}\gdef\@doiabbr{gases}\gdef\@ISSN{2673-5628}\gdef\@continuouspages{yes}}
\DeclareOption{gastroent}{\gdef\@journal{gastroent}\gdef\@journalfull{Gastroenterology Insights}\gdef\@journalshort{Gastroenterol. Insights}\gdef\@doiabbr{gastroent}\gdef\@ISSN{2036-7422}\gdef\@continuouspages{yes}}
\DeclareOption{gastrointestdisord}{\gdef\@journal{gastrointestdisord}\gdef\@journalfull{Gastrointestinal Disorders}\gdef\@journalshort{Gastrointest. Disord.}\gdef\@doiabbr{gidisord}\gdef\@ISSN{2624-5647}\gdef\@continuouspages{yes}}
\DeclareOption{gels}{\gdef\@journal{gels}\gdef\@journalfull{Gels}\gdef\@journalshort{Gels}\gdef\@doiabbr{gels}\gdef\@ISSN{2310-2861}}
\DeclareOption{genealogy}{\gdef\@journal{genealogy}\gdef\@journalfull{Genealogy}\gdef\@journalshort{Genealogy}\gdef\@doiabbr{genealogy}\gdef\@ISSN{2313-5778}}
\DeclareOption{genes}{\gdef\@journal{genes}\gdef\@journalfull{Genes}\gdef\@journalshort{Genes}\gdef\@doiabbr{genes}\gdef\@ISSN{2073-4425}}
\DeclareOption{geographies}{\gdef\@journal{geographies}\gdef\@journalfull{Geographies}\gdef\@journalshort{Geographies}\gdef\@doiabbr{geographies}\gdef\@ISSN{2673-7086}\gdef\@continuouspages{yes}}
\DeclareOption{geohazards}{\gdef\@journal{geohazards}\gdef\@journalfull{GeoHazards}\gdef\@journalshort{GeoHazards}\gdef\@doiabbr{geohazards}\gdef\@ISSN{2624-795X}\gdef\@continuouspages{yes}}
\DeclareOption{geomatics}{\gdef\@journal{geomatics}\gdef\@journalfull{Geomatics}\gdef\@journalshort{Geomatics}\gdef\@doiabbr{geomatics}\gdef\@ISSN{2673-7418}\gdef\@continuouspages{yes}}
\DeclareOption{geosciences}{\gdef\@journal{geosciences}\gdef\@journalfull{Geosciences}\gdef\@journalshort{Geosciences}\gdef\@doiabbr{geosciences}\gdef\@ISSN{2076-3263}}
\DeclareOption{geotechnics}{\gdef\@journal{geotechnics}\gdef\@journalfull{Geotechnics}\gdef\@journalshort{Geotechnics}\gdef\@doiabbr{geotechnics}\gdef\@ISSN{2673-7094}\gdef\@continuouspages{yes}}
\DeclareOption{geriatrics}{\gdef\@journal{geriatrics}\gdef\@journalfull{Geriatrics}\gdef\@journalshort{Geriatrics}\gdef\@doiabbr{geriatrics}\gdef\@ISSN{2308-3417}}
\DeclareOption{grasses}{\gdef\@journal{grasses}\gdef\@journalfull{Grasses}\gdef\@journalshort{Grasses}\gdef\@doiabbr{grasses}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{gucdd}{\gdef\@journal{gucdd}\gdef\@journalfull{Gout, Urate, and Crystal Deposition Disease}\gdef\@journalshort{Gout Urate Cryst. Depos. Dis.}\gdef\@doiabbr{gucdd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hazardousmatters}{\gdef\@journal{hazardousmatters}\gdef\@journalfull{Hazardous Matters}\gdef\@journalshort{Hazard. Matters}\gdef\@doiabbr{}\gdef\@ISSN{0014-0014}}
\DeclareOption{healthcare}{\gdef\@journal{healthcare}\gdef\@journalfull{Healthcare}\gdef\@journalshort{Healthcare}\gdef\@doiabbr{healthcare}\gdef\@ISSN{2227-9032}}
\DeclareOption{hearts}{\gdef\@journal{hearts}\gdef\@journalfull{Hearts}\gdef\@journalshort{Hearts}\gdef\@doiabbr{hearts}\gdef\@ISSN{2673-3846}\gdef\@continuouspages{yes}}
\DeclareOption{hemato}{\gdef\@journal{hemato}\gdef\@journalfull{Hemato}\gdef\@journalshort{Hemato}\gdef\@doiabbr{hemato}\gdef\@ISSN{2673-6357}\gdef\@continuouspages{yes}}
\DeclareOption{hematolrep}{\gdef\@journal{hematolrep}\gdef\@journalfull{Hematology Reports}\gdef\@journalshort{Hematol. Rep.}\gdef\@doiabbr{hematolrep}\gdef\@ISSN{2038-8330}\gdef\@continuouspages{yes}}
\DeclareOption{heritage}{\gdef\@journal{heritage}\gdef\@journalfull{Heritage}\gdef\@journalshort{Heritage}\gdef\@doiabbr{heritage}\gdef\@ISSN{2571-9408}\gdef\@continuouspages{yes}}
\DeclareOption{higheredu}{\gdef\@journal{higheredu}\gdef\@journalfull{Trends in Higher Education}\gdef\@journalshort{Trends High. Educ.}\gdef\@doiabbr{higheredu}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{highthroughput}{\gdef\@journal{highthroughput}\gdef\@journalfull{High-Throughput}\gdef\@journalshort{High-Throughput}\gdef\@doiabbr{ht}\gdef\@ISSN{2571-5135}}
\DeclareOption{histories}{\gdef\@journal{histories}\gdef\@journalfull{Histories}\gdef\@journalshort{Histories}\gdef\@doiabbr{histories}\gdef\@ISSN{2409-9252}\gdef\@continuouspages{yes}}
\DeclareOption{horticulturae}{\gdef\@journal{horticulturae}\gdef\@journalfull{Horticulturae}\gdef\@journalshort{Horticulturae}\gdef\@doiabbr{horticulturae}\gdef\@ISSN{2311-7524}}
\DeclareOption{hospitals}{\gdef\@journal{hospitals}\gdef\@journalfull{Hospitals}\gdef\@journalshort{Hospitals}\gdef\@doiabbr{hospitals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{humanities}{\gdef\@journal{humanities}\gdef\@journalfull{Humanities}\gdef\@journalshort{Humanities}\gdef\@doiabbr{h}\gdef\@ISSN{2076-0787}}
\DeclareOption{humans}{\gdef\@journal{humans}\gdef\@journalfull{Humans}\gdef\@journalshort{Humans}\gdef\@doiabbr{humans}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hydrobiology}{\gdef\@journal{hydrobiology}\gdef\@journalfull{Hydrobiology}\gdef\@journalshort{Hydrobiology	}\gdef\@doiabbr{hydrobiology}\gdef\@ISSN{2673-9917}\gdef\@continuouspages{yes}}
\DeclareOption{hydrogen}{\gdef\@journal{hydrogen}\gdef\@journalfull{Hydrogen}\gdef\@journalshort{Hydrogen}\gdef\@doiabbr{hydrogen}\gdef\@ISSN{2673-4141}\gdef\@continuouspages{yes}}
\DeclareOption{hydrology}{\gdef\@journal{hydrology}\gdef\@journalfull{Hydrology}\gdef\@journalshort{Hydrology}\gdef\@doiabbr{hydrology}\gdef\@ISSN{2306-5338}}
\DeclareOption{hygiene}{\gdef\@journal{hygiene}\gdef\@journalfull{Hygiene}\gdef\@journalshort{Hygiene}\gdef\@doiabbr{hygiene}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{idr}{\gdef\@journal{idr}\gdef\@journalfull{Infectious Disease Reports}\gdef\@journalshort{Infect. Dis. Rep.}\gdef\@doiabbr{idr}\gdef\@ISSN{2036-7449}\gdef\@continuouspages{yes}}
\DeclareOption{ijerph}{\gdef\@journal{ijerph}\gdef\@journalfull{International Journal of Environmental Research and Public Health}\gdef\@journalshort{Int. J. Environ. Res. Public Health}\gdef\@doiabbr{ijerph}\gdef\@ISSN{1660-4601}}
\DeclareOption{ijfs}{\gdef\@journal{ijfs}\gdef\@journalfull{International Journal of Financial Studies}\gdef\@journalshort{Int. J. Financial Stud.}\gdef\@doiabbr{ijfs}\gdef\@ISSN{2227-7072}}
\DeclareOption{ijgi}{\gdef\@journal{ijgi}\gdef\@journalfull{ISPRS International Journal of Geo-Information}\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}\gdef\@doiabbr{ijgi}\gdef\@ISSN{2220-9964}}
\DeclareOption{ijms}{\gdef\@journal{ijms}\gdef\@journalfull{International Journal of Molecular Sciences}\gdef\@journalshort{Int. J. Mol. Sci.}\gdef\@doiabbr{ijms}\gdef\@ISSN{1422-0067}}
\DeclareOption{ijns}{\gdef\@journal{ijns}\gdef\@journalfull{International Journal of Neonatal Screening}\gdef\@journalshort{Int. J. Neonatal Screen.}\gdef\@doiabbr{ijns}\gdef\@ISSN{2409-515X}}
\DeclareOption{ijpb}{\gdef\@journal{ijpb}\gdef\@journalfull{International Journal of Plant Biology}\gdef\@journalshort{Int. J. Plant Biol.}\gdef\@doiabbr{ijpb}\gdef\@ISSN{2037-0164}\gdef\@continuouspages{yes}}
\DeclareOption{ijtm}{\gdef\@journal{ijtm}\gdef\@journalfull{International Journal of Translational Medicine}\gdef\@journalshort{Int. J. Transl. Med.}\gdef\@doiabbr{ijtm}\gdef\@ISSN{2673-8937}\gdef\@continuouspages{yes}}
\DeclareOption{ijtpp}{\gdef\@journal{ijtpp}\gdef\@journalfull{International Journal of Turbomachinery Propulsion and Power}\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}\gdef\@doiabbr{ijtpp}\gdef\@ISSN{2504-186X}}
\DeclareOption{ime}{\gdef\@journal{ime}\gdef\@journalfull{International Medical Education}\gdef\@journalshort{Int. Med. Educ.}\gdef\@doiabbr{ime}\gdef\@ISSN{2813-141X}\gdef\@continuouspages{yes}}
\DeclareOption{immuno}{\gdef\@journal{immuno}\gdef\@journalfull{Immuno}\gdef\@journalshort{Immuno}\gdef\@doiabbr{immuno}\gdef\@ISSN{2673-5601}\gdef\@continuouspages{yes}}
\DeclareOption{informatics}{\gdef\@journal{informatics}\gdef\@journalfull{Informatics}\gdef\@journalshort{Informatics}\gdef\@doiabbr{informatics}\gdef\@ISSN{2227-9709}}
\DeclareOption{information}{\gdef\@journal{information}\gdef\@journalfull{Information}\gdef\@journalshort{Information}\gdef\@doiabbr{info}\gdef\@ISSN{2078-2489}}
\DeclareOption{infrastructures}{\gdef\@journal{infrastructures}\gdef\@journalfull{Infrastructures}\gdef\@journalshort{Infrastructures}\gdef\@doiabbr{infrastructures}\gdef\@ISSN{2412-3811}}
\DeclareOption{inorganics}{\gdef\@journal{inorganics}\gdef\@journalfull{Inorganics}\gdef\@journalshort{Inorganics}\gdef\@doiabbr{inorganics}\gdef\@ISSN{2304-6740}}
\DeclareOption{insects}{\gdef\@journal{insects}\gdef\@journalfull{Insects}\gdef\@journalshort{Insects}\gdef\@doiabbr{insects}\gdef\@ISSN{2075-4450}}
\DeclareOption{instruments}{\gdef\@journal{instruments}\gdef\@journalfull{Instruments}\gdef\@journalshort{Instruments}\gdef\@doiabbr{instruments}\gdef\@ISSN{2410-390X}}
\DeclareOption{inventions}{\gdef\@journal{inventions}\gdef\@journalfull{Inventions}\gdef\@journalshort{Inventions}\gdef\@doiabbr{inventions}\gdef\@ISSN{2411-5134}}
\DeclareOption{iot}{\gdef\@journal{iot}\gdef\@journalfull{IoT}\gdef\@journalshort{IoT}\gdef\@doiabbr{iot}\gdef\@ISSN{2624-831X}\gdef\@continuouspages{yes}}
\DeclareOption{j}{\gdef\@journal{j}\gdef\@journalfull{J}\gdef\@journalshort{J}\gdef\@doiabbr{j}\gdef\@ISSN{2571-8800}\gdef\@continuouspages{yes}}
\DeclareOption{jal}{\gdef\@journal{jal}\gdef\@journalfull{Journal of Ageing and Longevity}\gdef\@journalshort{J. Ageing Longev.}\gdef\@doiabbr{jal}\gdef\@ISSN{2673-9259}\gdef\@continuouspages{yes}}
\DeclareOption{jcdd}{\gdef\@journal{jcdd}\gdef\@journalfull{Journal of Cardiovascular Development and Disease}\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}\gdef\@doiabbr{jcdd}\gdef\@ISSN{2308-3425}}
\DeclareOption{jcm}{\gdef\@journal{jcm}\gdef\@journalfull{Journal of Clinical Medicine}\gdef\@journalshort{J. Clin. Med.}\gdef\@doiabbr{jcm}\gdef\@ISSN{2077-0383}}
\DeclareOption{jcp}{\gdef\@journal{jcp}\gdef\@journalfull{Journal of Cybersecurity and Privacy}\gdef\@journalshort{J. Cybersecur. Priv.}\gdef\@doiabbr{jcp}\gdef\@ISSN{2624-800X}\gdef\@continuouspages{yes}}
\DeclareOption{jcs}{\gdef\@journal{jcs}\gdef\@journalfull{Journal of Composites Science}\gdef\@journalshort{J. Compos. Sci.}\gdef\@doiabbr{jcs}\gdef\@ISSN{2504-477X}}
\DeclareOption{jcto}{\gdef\@journal{jcto}\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}\gdef\@doiabbr{jcto}\gdef\@ISSN{2813-1053}\gdef\@continuouspages{yes}}
\DeclareOption{jdb}{\gdef\@journal{jdb}\gdef\@journalfull{Journal of Developmental Biology}\gdef\@journalshort{J. Dev. Biol.}\gdef\@doiabbr{jdb}\gdef\@ISSN{2221-3759}}
\DeclareOption{jeta}{\gdef\@journal{jeta}\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}\gdef\@journalshort{J. Exp. Theor. Anal.}\gdef\@doiabbr{jeta}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jfb}{\gdef\@journal{jfb}\gdef\@journalfull{Journal of Functional Biomaterials}\gdef\@journalshort{J. Funct. Biomater.}\gdef\@doiabbr{jfb}\gdef\@ISSN{2079-4983}}
\DeclareOption{jfmk}{\gdef\@journal{jfmk}\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}\gdef\@doiabbr{jfmk}\gdef\@ISSN{2411-5142}}
\DeclareOption{jimaging}{\gdef\@journal{jimaging}\gdef\@journalfull{Journal of Imaging}\gdef\@journalshort{J. Imaging}\gdef\@doiabbr{jimaging}\gdef\@ISSN{2313-433X}}
\DeclareOption{jintelligence}{\gdef\@journal{jintelligence}\gdef\@journalfull{Journal of Intelligence}\gdef\@journalshort{J. Intell.}\gdef\@doiabbr{jintelligence}\gdef\@ISSN{2079-3200}}
\DeclareOption{jlpea}{\gdef\@journal{jlpea}\gdef\@journalfull{Journal of Low Power Electronics and Applications}\gdef\@journalshort{J. Low Power Electron. Appl.}\gdef\@doiabbr{jlpea}\gdef\@ISSN{2079-9268}}
\DeclareOption{jmmp}{\gdef\@journal{jmmp}\gdef\@journalfull{Journal of Manufacturing and Materials Processing}\gdef\@journalshort{J. Manuf. Mater. Process.}\gdef\@doiabbr{jmmp}\gdef\@ISSN{2504-4494}}
\DeclareOption{jmp}{\gdef\@journal{jmp}\gdef\@journalfull{Journal of Molecular Pathology}\gdef\@journalshort{J. Mol. Pathol.}\gdef\@doiabbr{jmp}\gdef\@ISSN{2673-5261}\gdef\@continuouspages{yes}}
\DeclareOption{jmse}{\gdef\@journal{jmse}\gdef\@journalfull{Journal of Marine Science and Engineering}\gdef\@journalshort{J. Mar. Sci. Eng.}\gdef\@doiabbr{jmse}\gdef\@ISSN{2077-1312}}
\DeclareOption{jne}{\gdef\@journal{jne}\gdef\@journalfull{Journal of Nuclear Engineering}\gdef\@journalshort{J. Nucl. Eng.}\gdef\@doiabbr{jne}\gdef\@ISSN{2673-4362}\gdef\@continuouspages{yes}}
\DeclareOption{jnt}{\gdef\@journal{jnt}\gdef\@journalfull{Journal of Nanotheranostics}\gdef\@journalshort{J. Nanotheranostics}\gdef\@doiabbr{jnt}\gdef\@ISSN{2624-845X}\gdef\@continuouspages{yes}}
\DeclareOption{jof}{\gdef\@journal{jof}\gdef\@journalfull{Journal of Fungi}\gdef\@journalshort{J. Fungi}\gdef\@doiabbr{jof}\gdef\@ISSN{2309-608X}}
\DeclareOption{joitmc}{\gdef\@journal{joitmc}\gdef\@journalfull{Journal of Open Innovation: Technology Market and Complexity}\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}\gdef\@doiabbr{joitmc}\gdef\@ISSN{2199-8531}}
\DeclareOption{jor}{\gdef\@journal{jor}\gdef\@journalfull{Journal of Respiration}\gdef\@journalshort{J. Respir.}\gdef\@doiabbr{jor}\gdef\@ISSN{2673-527X}\gdef\@continuouspages{yes}}
\DeclareOption{journalmedia}{\gdef\@journal{journalmedia}\gdef\@journalfull{Journalism and Media}\gdef\@journalshort{Journal. Media}\gdef\@doiabbr{journalmedia}\gdef\@ISSN{2673-5172}\gdef\@continuouspages{yes}}
\DeclareOption{jox}{\gdef\@journal{jox}\gdef\@journalfull{Journal of Xenobiotics}\gdef\@journalshort{J. Xenobiot.}\gdef\@doiabbr{jox}\gdef\@ISSN{2039-4713}\gdef\@continuouspages{yes}}
\DeclareOption{jpm}{\gdef\@journal{jpm}\gdef\@journalfull{Journal of Personalized Medicine}\gdef\@journalshort{J. Pers. Med.}\gdef\@doiabbr{jpm}\gdef\@ISSN{2075-4426}}
\DeclareOption{jrfm}{\gdef\@journal{jrfm}\gdef\@journalfull{Journal of Risk and Financial Management}\gdef\@journalshort{J. Risk Financial Manag.}\gdef\@doiabbr{jrfm}\gdef\@ISSN{1911-8074}}
\DeclareOption{jsan}{\gdef\@journal{jsan}\gdef\@journalfull{Journal of Sensor and Actuator Networks}\gdef\@journalshort{J. Sens. Actuator Netw.}\gdef\@doiabbr{jsan}\gdef\@ISSN{2224-2708}}
\DeclareOption{jtaer}{\gdef\@journal{jtaer}\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}\gdef\@doiabbr{jtaer}\gdef\@ISSN{0718-1876}\gdef\@continuouspages{yes}}
\DeclareOption{jvd}{\gdef\@journal{jvd}\gdef\@journalfull{Journal of Vascular Diseases}\gdef\@journalshort{JVD}\gdef\@doiabbr{jvd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jzbg}{\gdef\@journal{jzbg}\gdef\@journalfull{Journal of Zoological and Botanical Gardens}\gdef\@journalshort{J. Zool. Bot. Gard.}\gdef\@doiabbr{jzbg}\gdef\@ISSN{2673-5636}\gdef\@continuouspages{yes}}
%\DeclareOption{kidney}{\gdef\@journal{kidney}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kidneydial}{\gdef\@journal{kidneydial}\gdef\@journalfull{Kidney and Dialysis}\gdef\@journalshort{Kidney Dial.}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kinasesphosphatases}{\gdef\@journal{kinasesphosphatases}\gdef\@journalfull{Kinases and Phosphatases}\gdef\@journalshort{Kinases Phosphatases}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{knowledge}{\gdef\@journal{knowledge}\gdef\@journalfull{Knowledge}\gdef\@journalshort{Knowledge}\gdef\@doiabbr{knowledge}\gdef\@ISSN{2673-9585}\gdef\@continuouspages{yes}}
\DeclareOption{land}{\gdef\@journal{land}\gdef\@journalfull{Land}\gdef\@journalshort{Land}\gdef\@doiabbr{land}\gdef\@ISSN{2073-445X}}
\DeclareOption{languages}{\gdef\@journal{languages}\gdef\@journalfull{Languages}\gdef\@journalshort{Languages}\gdef\@doiabbr{languages}\gdef\@ISSN{2226-471X}}
\DeclareOption{laws}{\gdef\@journal{laws}\gdef\@journalfull{Laws}\gdef\@journalshort{Laws}\gdef\@doiabbr{laws}\gdef\@ISSN{2075-471X}}
\DeclareOption{life}{\gdef\@journal{life}\gdef\@journalfull{Life}\gdef\@journalshort{Life}\gdef\@doiabbr{life}\gdef\@ISSN{2075-1729}}
\DeclareOption{liquids}{\gdef\@journal{liquids}\gdef\@journalfull{Liquids}\gdef\@journalshort{Liquids}\gdef\@doiabbr{liquids}\gdef\@ISSN{2673-8015}\gdef\@continuouspages{yes}}
\DeclareOption{literature}{\gdef\@journal{literature}\gdef\@journalfull{Literature}\gdef\@journalshort{Literature}\gdef\@doiabbr{literature}\gdef\@ISSN{2410-9789}\gdef\@continuouspages{yes}}
\DeclareOption{livers}{\gdef\@journal{livers}\gdef\@journalfull{Livers}\gdef\@journalshort{Livers}\gdef\@doiabbr{livers}\gdef\@ISSN{2673-4389}\gdef\@continuouspages{yes}}
\DeclareOption{logics}{\gdef\@journal{logics}\gdef\@journalfull{Logics}\gdef\@journalshort{Logics}\gdef\@doiabbr{logics}\gdef\@ISSN{2813-0405}\gdef\@continuouspages{yes}}
\DeclareOption{logistics}{\gdef\@journal{logistics}\gdef\@journalfull{Logistics}\gdef\@journalshort{Logistics}\gdef\@doiabbr{logistics}\gdef\@ISSN{2305-6290}}
\DeclareOption{lubricants}{\gdef\@journal{lubricants}\gdef\@journalfull{Lubricants}\gdef\@journalshort{Lubricants}\gdef\@doiabbr{lubricants}\gdef\@ISSN{2075-4442}}
\DeclareOption{lymphatics}{\gdef\@journal{lymphatics}\gdef\@journalfull{Lymphatics}\gdef\@journalshort{Lymphatics}\gdef\@doiabbr{lymphatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}	
\DeclareOption{machines}{\gdef\@journal{machines}\gdef\@journalfull{Machines}\gdef\@journalshort{Machines}\gdef\@doiabbr{machines}\gdef\@ISSN{2075-1702}}
\DeclareOption{macromol}{\gdef\@journal{macromol}\gdef\@journalfull{Macromol}\gdef\@journalshort{Macromol}\gdef\@doiabbr{macromol}\gdef\@ISSN{2673-6209}\gdef\@continuouspages{yes}}
\DeclareOption{magnetism}{\gdef\@journal{magnetism}\gdef\@journalfull{Magnetism}\gdef\@journalshort{Magnetism}\gdef\@doiabbr{magnetism}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{magnetochemistry}{\gdef\@journal{magnetochemistry}\gdef\@journalfull{Magnetochemistry}\gdef\@journalshort{Magnetochemistry}\gdef\@doiabbr{magnetochemistry}\gdef\@ISSN{2312-7481}}
\DeclareOption{make}{\gdef\@journal{make}\gdef\@journalfull{Machine Learning and Knowledge Extraction}\gdef\@journalshort{Mach. Learn. Knowl. Extr.}\gdef\@doiabbr{make}\gdef\@ISSN{2504-4990}\gdef\@continuouspages{yes}}
\DeclareOption{marinedrugs}{\gdef\@journal{marinedrugs}\gdef\@journalfull{Marine Drugs}\gdef\@journalshort{Mar. Drugs}\gdef\@doiabbr{md}\gdef\@ISSN{1660-3397}}
\DeclareOption{materials}{\gdef\@journal{materials}\gdef\@journalfull{Materials}\gdef\@journalshort{Materials}\gdef\@doiabbr{ma}\gdef\@ISSN{1996-1944}}
\DeclareOption{materproc}{\gdef\@journal{materproc}\gdef\@journalfull{Materials Proceedings}\gdef\@journalshort{Mater. Proc.}\gdef\@doiabbr{materproc}\gdef\@ISSN{2673-4605}}
\DeclareOption{mathematics}{\gdef\@journal{mathematics}\gdef\@journalfull{Mathematics}\gdef\@journalshort{Mathematics}\gdef\@doiabbr{math}\gdef\@ISSN{2227-7390}}
\DeclareOption{mca}{\gdef\@journal{mca}\gdef\@journalfull{Mathematical and Computational Applications}\gdef\@journalshort{Math. Comput. Appl.}\gdef\@doiabbr{mca}\gdef\@ISSN{2297-8747}}
\DeclareOption{measurements}{\gdef\@journal{measurements}\gdef\@journalfull{Measurements}\gdef\@journalshort{Measurements}\gdef\@doiabbr{measurements}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{medicina}{\gdef\@journal{medicina}\gdef\@journalfull{Medicina}\gdef\@journalshort{Medicina}\gdef\@doiabbr{medicina}\gdef\@ISSN{1648-9144}}
\DeclareOption{medicines}{\gdef\@journal{medicines}\gdef\@journalfull{Medicines}\gdef\@journalshort{Medicines}\gdef\@doiabbr{medicines}\gdef\@ISSN{2305-6320}}
\DeclareOption{medsci}{\gdef\@journal{medsci}\gdef\@journalfull{Medical Sciences}\gdef\@journalshort{Med. Sci.}\gdef\@doiabbr{medsci}\gdef\@ISSN{2076-3271}}
\DeclareOption{membranes}{\gdef\@journal{membranes}\gdef\@journalfull{Membranes}\gdef\@journalshort{Membranes}\gdef\@doiabbr{membranes}\gdef\@ISSN{2077-0375}}
\DeclareOption{merits}{\gdef\@journal{merits}\gdef\@journalfull{Merits}\gdef\@journalshort{Merits}\gdef\@doiabbr{merits}\gdef\@ISSN{2673-8104}\gdef\@continuouspages{yes}}
\DeclareOption{metabolites}{\gdef\@journal{metabolites}\gdef\@journalfull{Metabolites}\gdef\@journalshort{Metabolites}\gdef\@doiabbr{metabo}\gdef\@ISSN{2218-1989}}
\DeclareOption{metals}{\gdef\@journal{metals}\gdef\@journalfull{Metals}\gdef\@journalshort{Metals}\gdef\@doiabbr{met}\gdef\@ISSN{2075-4701}}
\DeclareOption{meteorology}{\gdef\@journal{meteorology}\gdef\@journalfull{Meteorology}\gdef\@journalshort{Meteorology}\gdef\@doiabbr{meteorology}\gdef\@ISSN{2674-0494}\gdef\@continuouspages{yes}}
\DeclareOption{methane}{\gdef\@journal{methane}\gdef\@journalfull{Methane}\gdef\@journalshort{Methane}\gdef\@doiabbr{methane}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{metrology}{\gdef\@journal{metrology}\gdef\@journalfull{Metrology}\gdef\@journalshort{Metrology}\gdef\@doiabbr{metrology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{micro}{\gdef\@journal{micro}\gdef\@journalfull{Micro}\gdef\@journalshort{Micro}\gdef\@doiabbr{micro}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{microarrays}{\gdef\@journal{microarrays}\gdef\@journalfull{Microarrays}\gdef\@journalshort{Microarrays}\gdef\@doiabbr{microarrays}\gdef\@ISSN{2076-3905}}
\DeclareOption{microbiolres}{\gdef\@journal{microbiolres}\gdef\@journalfull{Microbiology Research}\gdef\@journalshort{Microbiol. Res.}\gdef\@doiabbr{microbiolres}\gdef\@ISSN{2036-7481}\gdef\@continuouspages{yes}}
\DeclareOption{micromachines}{\gdef\@journal{micromachines}\gdef\@journalfull{Micromachines}\gdef\@journalshort{Micromachines}\gdef\@doiabbr{mi}\gdef\@ISSN{2072-666X}}
\DeclareOption{microorganisms}{\gdef\@journal{microorganisms}\gdef\@journalfull{Microorganisms}\gdef\@journalshort{Microorganisms}\gdef\@doiabbr{microorganisms}\gdef\@ISSN{2076-2607}}
\DeclareOption{microplastics}{\gdef\@journal{microplastics}\gdef\@journalfull{Microplastics}\gdef\@journalshort{Microplastics}\gdef\@doiabbr{microplastics}\gdef\@ISSN{2673-8929}\gdef\@continuouspages{yes}}
\DeclareOption{minerals}{\gdef\@journal{minerals}\gdef\@journalfull{Minerals}\gdef\@journalshort{Minerals}\gdef\@doiabbr{min}\gdef\@ISSN{2075-163X}}
\DeclareOption{mining}{\gdef\@journal{mining}\gdef\@journalfull{Mining}\gdef\@journalshort{Mining}\gdef\@doiabbr{mining}\gdef\@ISSN{2673-6489}\gdef\@continuouspages{yes}}
\DeclareOption{modelling}{\gdef\@journal{modelling}\gdef\@journalfull{Modelling}\gdef\@journalshort{Modelling}\gdef\@doiabbr{modelling}\gdef\@ISSN{2673-3951}\gdef\@continuouspages{yes}}
\DeclareOption{molbank}{\gdef\@journal{molbank}\gdef\@journalfull{Molbank}\gdef\@journalshort{Molbank}\gdef\@doiabbr{M}\gdef\@ISSN{1422-8599}}
\DeclareOption{molecules}{\gdef\@journal{molecules}\gdef\@journalfull{Molecules}\gdef\@journalshort{Molecules}\gdef\@doiabbr{molecules}\gdef\@ISSN{1420-3049}}
\DeclareOption{mps}{\gdef\@journal{mps}\gdef\@journalfull{Methods and Protocols}\gdef\@journalshort{Methods Protoc.}\gdef\@doiabbr{mps}\gdef\@ISSN{2409-9279}}
\DeclareOption{msf}{\gdef\@journal{msf}\gdef\@journalfull{Medical Sciences Forum}\gdef\@journalshort{Med. Sci. Forum}\gdef\@doiabbr{msf}\gdef\@ISSN{2673-9992}}
\DeclareOption{mti}{\gdef\@journal{mti}\gdef\@journalfull{Multimodal Technologies and Interaction}\gdef\@journalshort{Multimodal Technol. Interact.}\gdef\@doiabbr{mti}\gdef\@ISSN{2414-4088}}
\DeclareOption{muscles}{\gdef\@journal{muscles}\gdef\@journalfull{Muscles}\gdef\@journalshort{Muscles}\gdef\@doiabbr{muscles}\gdef\@ISSN{2813-0413}\gdef\@continuouspages{yes}}
\DeclareOption{nanoenergyadv}{\gdef\@journal{nanoenergyadv}\gdef\@journalfull{Nanoenergy Advances}\gdef\@journalshort{Nanoenergy Adv.}\gdef\@doiabbr{nanoenergyadv}\gdef\@ISSN{2673-706X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomanufacturing}{\gdef\@journal{nanomanufacturing}\gdef\@journalfull{Nanomanufacturing}\gdef\@journalshort{Nanomanufacturing}\gdef\@doiabbr{nanomanufacturing}\gdef\@ISSN{2673-687X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomaterials}{\gdef\@journal{nanomaterials}\gdef\@journalfull{Nanomaterials}\gdef\@journalshort{Nanomaterials}\gdef\@doiabbr{nano}\gdef\@ISSN{2079-4991}}
\DeclareOption{ncrna}{\gdef\@journal{ncrna}\gdef\@journalfull{Non-Coding RNA}\gdef\@journalshort{Non-Coding RNA}\gdef\@doiabbr{ncrna}\gdef\@ISSN{2311-553X}}
\DeclareOption{ndt}{\gdef\@journal{ndt}\gdef\@journalfull{NDT}\gdef\@journalshort{NDT}\gdef\@doiabbr{ndt}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{network}{\gdef\@journal{network}\gdef\@journalfull{Network}\gdef\@journalshort{Network}\gdef\@doiabbr{network}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{neuroglia}{\gdef\@journal{neuroglia}\gdef\@journalfull{Neuroglia}\gdef\@journalshort{Neuroglia}\gdef\@doiabbr{neuroglia}\gdef\@ISSN{2571-6980}\gdef\@continuouspages{yes}}
\DeclareOption{neurolint}{\gdef\@journal{neurolint}\gdef\@journalfull{Neurology International}\gdef\@journalshort{Neurol. Int.}\gdef\@doiabbr{neurolint}\gdef\@ISSN{2035-8377}\gdef\@continuouspages{yes}}
\DeclareOption{neurosci}{\gdef\@journal{neurosci}\gdef\@journalfull{NeuroSci}\gdef\@journalshort{NeuroSci}\gdef\@doiabbr{neurosci}\gdef\@ISSN{2673-4087}\gdef\@continuouspages{yes}}
\DeclareOption{nitrogen}{\gdef\@journal{nitrogen}\gdef\@journalfull{Nitrogen}\gdef\@journalshort{Nitrogen}\gdef\@doiabbr{nitrogen}\gdef\@ISSN{2504-3129}\gdef\@continuouspages{yes}}
\DeclareOption{notspecified}{\gdef\@journal{notspecified}\gdef\@journalfull{Journal Not Specified}\gdef\@journalshort{Journal Not Specified}\gdef\@doiabbr{}\gdef\@ISSN{}}
%%\DeclareOption{nri}{\gdef\@journal{nri}\gdef\@journalfull{Natural Resources Informatics}\gdef\@journalshort{Nat. Resour. Inform.}\gdef\@doiabbr{nri}\gdef\@ISSN{2673-981X}\gdef\@continuouspages{yes}}
\DeclareOption{nursrep}{\gdef\@journal{nursrep}\gdef\@journalfull{Nursing Reports}\gdef\@journalshort{Nurs. Rep.}\gdef\@doiabbr{nursrep}\gdef\@ISSN{2039-4403}\gdef\@continuouspages{yes}}
\DeclareOption{nutraceuticals}{\gdef\@journal{nutraceuticals}\gdef\@journalfull{Nutraceuticals}\gdef\@journalshort{Nutraceuticals}\gdef\@doiabbr{nutraceuticals}\gdef\@ISSN{1661-3821}\gdef\@continuouspages{yes}}
\DeclareOption{nutrients}{\gdef\@journal{nutrients}\gdef\@journalfull{Nutrients}\gdef\@journalshort{Nutrients}\gdef\@doiabbr{nu}\gdef\@ISSN{2072-6643}}
\DeclareOption{obesities}{\gdef\@journal{obesities}\gdef\@journalfull{Obesities}\gdef\@journalshort{Obesities}\gdef\@doiabbr{obesities}\gdef\@ISSN{2673-4168}\gdef\@continuouspages{yes}}
\DeclareOption{oceans}{\gdef\@journal{oceans}\gdef\@journalfull{Oceans}\gdef\@journalshort{Oceans}\gdef\@doiabbr{oceans}\gdef\@ISSN{2673-1924}\gdef\@continuouspages{yes}}
\DeclareOption{ohbm}{\gdef\@journal{ohbm}\gdef\@journalfull{Journal of Otorhinolaryngology Hearing and Balance Medicine}\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}\gdef\@doiabbr{ohbm}\gdef\@ISSN{2504-463X}}
\DeclareOption{onco}{\gdef\@journal{onco}\gdef\@journalfull{Onco}\gdef\@journalshort{Onco}\gdef\@doiabbr{onco}\gdef\@ISSN{2673-7523}\gdef\@continuouspages{yes}}
%\DeclareOption{oncopathology}{\gdef\@journal{oncopathology}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{optics}{\gdef\@journal{optics}\gdef\@journalfull{Optics}\gdef\@journalshort{Optics}\gdef\@doiabbr{opt}\gdef\@ISSN{2673-3269}\gdef\@continuouspages{yes}}
\DeclareOption{oral}{\gdef\@journal{oral}\gdef\@journalfull{Oral}\gdef\@journalshort{Oral}\gdef\@doiabbr{oral}\gdef\@ISSN{2673-6373}\gdef\@continuouspages{yes}}
\DeclareOption{organics}{\gdef\@journal{organics}\gdef\@journalfull{Organics}\gdef\@journalshort{Organics}\gdef\@doiabbr{org}\gdef\@ISSN{2673-401X}\gdef\@continuouspages{yes}}
\DeclareOption{organoids}{\gdef\@journal{organoids}\gdef\@journalfull{Organoids}\gdef\@journalshort{Organoids}\gdef\@doiabbr{organoids}\gdef\@ISSN{2674-1172}\gdef\@continuouspages{yes}}
\DeclareOption{osteology}{\gdef\@journal{osteology}\gdef\@journalfull{Osteology}\gdef\@journalshort{Osteology}\gdef\@doiabbr{osteology}\gdef\@ISSN{2673-4036}\gdef\@continuouspages{yes}}
\DeclareOption{oxygen}{\gdef\@journal{oxygen}\gdef\@journalfull{Oxygen}\gdef\@journalshort{Oxygen}\gdef\@doiabbr{oxygen}\gdef\@ISSN{2673-9801}\gdef\@continuouspages{yes}}
\DeclareOption{parasites}{\gdef\@journal{parasites}\gdef\@journalfull{Parasites}\gdef\@journalshort{Parasites}\gdef\@doiabbr{parasites}\gdef\@ISSN{2673-5946}}
\DeclareOption{parasitologia}{\gdef\@journal{parasitologia}\gdef\@journalfull{Parasitologia}\gdef\@journalshort{Parasitologia}\gdef\@doiabbr{parasitologia}\gdef\@ISSN{2673-6772}\gdef\@continuouspages{yes}}
\DeclareOption{particles}{\gdef\@journal{particles}\gdef\@journalfull{Particles}\gdef\@journalshort{Particles}\gdef\@doiabbr{particles}\gdef\@ISSN{2571-712X}\gdef\@continuouspages{yes}}
\DeclareOption{pathogens}{\gdef\@journal{pathogens}\gdef\@journalfull{Pathogens}\gdef\@journalshort{Pathogens}\gdef\@doiabbr{pathogens}\gdef\@ISSN{2076-0817}}
\DeclareOption{pathophysiology}{\gdef\@journal{pathophysiology}\gdef\@journalfull{Pathophysiology}\gdef\@journalshort{Pathophysiology}\gdef\@doiabbr{pathophysiology}\gdef\@ISSN{0928-4680}\gdef\@continuouspages{yes}}
\DeclareOption{pediatrrep}{\gdef\@journal{pediatrrep}\gdef\@journalfull{Pediatric Reports}\gdef\@journalshort{Pediatr. Rep.}\gdef\@doiabbr{pediatric}\gdef\@ISSN{2036-7503}\gdef\@continuouspages{yes}}
\DeclareOption{pharmaceuticals}{\gdef\@journal{pharmaceuticals}\gdef\@journalfull{Pharmaceuticals}\gdef\@journalshort{Pharmaceuticals}\gdef\@doiabbr{ph}\gdef\@ISSN{1424-8247}}
\DeclareOption{pharmaceutics}{\gdef\@journal{pharmaceutics}\gdef\@journalfull{Pharmaceutics}\gdef\@journalshort{Pharmaceutics}\gdef\@doiabbr{pharmaceutics}\gdef\@ISSN{1999-4923}}
\DeclareOption{pharmacoepidemiology}{\gdef\@journal{pharmacoepidemiology}\gdef\@journalfull{Pharmacoepidemiology}\gdef\@journalshort{Pharmacoepidemiology}\gdef\@doiabbr{pharma}\gdef\@ISSN{2813-0618}\gdef\@continuouspages{yes}}
\DeclareOption{pharmacy}{\gdef\@journal{pharmacy}\gdef\@journalfull{Pharmacy}\gdef\@journalshort{Pharmacy}\gdef\@doiabbr{pharmacy}\gdef\@ISSN{2226-4787}}
\DeclareOption{philosophies}{\gdef\@journal{philosophies}\gdef\@journalfull{Philosophies}\gdef\@journalshort{Philosophies}\gdef\@doiabbr{philosophies}\gdef\@ISSN{2409-9287}}
\DeclareOption{photochem}{\gdef\@journal{photochem}\gdef\@journalfull{Photochem}\gdef\@journalshort{Photochem}\gdef\@doiabbr{photochem}\gdef\@ISSN{2673-7256}\gdef\@continuouspages{yes}}
\DeclareOption{photonics}{\gdef\@journal{photonics}\gdef\@journalfull{Photonics}\gdef\@journalshort{Photonics}\gdef\@doiabbr{photonics}\gdef\@ISSN{2304-6732}}
\DeclareOption{phycology}{\gdef\@journal{phycology}\gdef\@journalfull{Phycology}\gdef\@journalshort{Phycology}\gdef\@doiabbr{phycology}\gdef\@ISSN{2673-9410}\gdef\@continuouspages{yes}}
\DeclareOption{physchem}{\gdef\@journal{physchem}\gdef\@journalfull{Physchem}\gdef\@journalshort{Physchem}\gdef\@doiabbr{physchem}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{physics}{\gdef\@journal{physics}\gdef\@journalfull{Physics}\gdef\@journalshort{Physics}\gdef\@doiabbr{physics}\gdef\@ISSN{2624-8174}\gdef\@continuouspages{yes}}
\DeclareOption{physiologia}{\gdef\@journal{physiologia}\gdef\@journalfull{Physiologia}\gdef\@journalshort{Physiologia}\gdef\@doiabbr{physiologia}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{plants}{\gdef\@journal{plants}\gdef\@journalfull{Plants}\gdef\@journalshort{Plants}\gdef\@doiabbr{plants}\gdef\@ISSN{2223-7747}}
\DeclareOption{plasma}{\gdef\@journal{plasma}\gdef\@journalfull{Plasma}\gdef\@journalshort{Plasma}\gdef\@doiabbr{plasma}\gdef\@ISSN{2571-6182}\gdef\@continuouspages{yes}}
\DeclareOption{platforms}{\gdef\@journal{platforms}\gdef\@journalfull{Platforms}\gdef\@journalshort{Platforms}\gdef\@doiabbr{platforms}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{pollutants}{\gdef\@journal{pollutants}\gdef\@journalfull{Pollutants}\gdef\@journalshort{Pollutants}\gdef\@doiabbr{pollutants}\gdef\@ISSN{2673-4672}\gdef\@continuouspages{yes}}
\DeclareOption{polymers}{\gdef\@journal{polymers}\gdef\@journalfull{Polymers}\gdef\@journalshort{Polymers}\gdef\@doiabbr{polym}\gdef\@ISSN{2073-4360}}
\DeclareOption{polysaccharides}{\gdef\@journal{polysaccharides}\gdef\@journalfull{Polysaccharides}\gdef\@journalshort{Polysaccharides}\gdef\@doiabbr{polysaccharides}\gdef\@ISSN{2673-4176}\gdef\@continuouspages{yes}}
\DeclareOption{poultry}{\gdef\@journal{poultry}\gdef\@journalfull{Poultry}\gdef\@journalshort{Poultry}\gdef\@doiabbr{poultry}\gdef\@ISSN{2674-1164}\gdef\@continuouspages{yes}}
\DeclareOption{powders}{\gdef\@journal{powders}\gdef\@journalfull{Powders}\gdef\@journalshort{Powders}\gdef\@doiabbr{powders}\gdef\@ISSN{2674-0516}\gdef\@continuouspages{yes}}
\DeclareOption{preprints}{\gdef\@journal{preprints}\gdef\@journalfull{Preprints}\gdef\@journalshort{Preprints}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{proceedings}{\gdef\@journal{proceedings}\gdef\@journalfull{Proceedings}\gdef\@journalshort{Proceedings}\gdef\@doiabbr{proceedings}\gdef\@ISSN{2504-3900}}
\DeclareOption{processes}{\gdef\@journal{processes}\gdef\@journalfull{Processes}\gdef\@journalshort{Processes}\gdef\@doiabbr{pr}\gdef\@ISSN{2227-9717}}
\DeclareOption{prosthesis}{\gdef\@journal{prosthesis}\gdef\@journalfull{Prosthesis}\gdef\@journalshort{Prosthesis}\gdef\@doiabbr{prosthesis}\gdef\@ISSN{2673-1592}\gdef\@continuouspages{yes}}
\DeclareOption{proteomes}{\gdef\@journal{proteomes}\gdef\@journalfull{Proteomes}\gdef\@journalshort{Proteomes}\gdef\@doiabbr{proteomes}\gdef\@ISSN{2227-7382}}
\DeclareOption{psf}{\gdef\@journal{psf}\gdef\@journalfull{Physical Sciences Forum}\gdef\@journalshort{Phys. Sci. Forum}\gdef\@doiabbr{psf}\gdef\@ISSN{2673-9984}}
\DeclareOption{psych}{\gdef\@journal{psych}\gdef\@journalfull{Psych}\gdef\@journalshort{Psych}\gdef\@doiabbr{psych}\gdef\@ISSN{2624-8611}\gdef\@continuouspages{yes}}
\DeclareOption{psychiatryint}{\gdef\@journal{psychiatryint}\gdef\@journalfull{Psychiatry International}\gdef\@journalshort{Psychiatry Int.}\gdef\@doiabbr{psychiatryint}\gdef\@ISSN{2673-5318}\gdef\@continuouspages{yes}}
\DeclareOption{psychoactives}{\gdef\@journal{psychoactives}\gdef\@journalfull{Psychoactives}\gdef\@journalshort{Psychoactives}\gdef\@doiabbr{psychoactives}\gdef\@ISSN{2813-1851}\gdef\@continuouspages{yes}}
\DeclareOption{publications}{\gdef\@journal{publications}\gdef\@journalfull{Publications}\gdef\@journalshort{Publications}\gdef\@doiabbr{publications}\gdef\@ISSN{2304-6775}}
\DeclareOption{quantumrep}{\gdef\@journal{quantumrep}\gdef\@journalfull{Quantum Reports}\gdef\@journalshort{Quantum Rep.}\gdef\@doiabbr{quantum}\gdef\@ISSN{2624-960X}\gdef\@continuouspages{yes}}
\DeclareOption{quaternary}{\gdef\@journal{quaternary}\gdef\@journalfull{Quaternary}\gdef\@journalshort{Quaternary}\gdef\@doiabbr{quat}\gdef\@ISSN{2571-550X}}
\DeclareOption{qubs}{\gdef\@journal{qubs}\gdef\@journalfull{Quantum Beam Science}\gdef\@journalshort{Quantum Beam Sci.}\gdef\@doiabbr{qubs}\gdef\@ISSN{2412-382X}}
\DeclareOption{radiation}{\gdef\@journal{radiation}\gdef\@journalfull{Radiation}\gdef\@journalshort{Radiation}\gdef\@doiabbr{radiation}\gdef\@ISSN{2673-592X}\gdef\@continuouspages{yes}}
\DeclareOption{reactions}{\gdef\@journal{reactions}\gdef\@journalfull{Reactions}\gdef\@journalshort{Reactions}\gdef\@doiabbr{reactions}\gdef\@ISSN{2624-781X}\gdef\@continuouspages{yes}}
\DeclareOption{receptors}{\gdef\@journal{receptors}\gdef\@journalfull{Receptors}\gdef\@journalshort{Receptors}\gdef\@doiabbr{receptors}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{recycling}{\gdef\@journal{recycling}\gdef\@journalfull{Recycling}\gdef\@journalshort{Recycling}\gdef\@doiabbr{recycling}\gdef\@ISSN{2313-4321}}
\DeclareOption{regeneration}{\gdef\@journal{regeneration}\gdef\@journalfull{Regeneration}\gdef\@journalshort{Regeneration}\gdef\@doiabbr{regeneration}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{religions}{\gdef\@journal{religions}\gdef\@journalfull{Religions}\gdef\@journalshort{Religions}\gdef\@doiabbr{rel}\gdef\@ISSN{2077-1444}}
\DeclareOption{remotesensing}{\gdef\@journal{remotesensing}\gdef\@journalfull{Remote Sensing}\gdef\@journalshort{Remote Sens.}\gdef\@doiabbr{rs}\gdef\@ISSN{2072-4292}}
\DeclareOption{reports}{\gdef\@journal{reports}\gdef\@journalfull{Reports}\gdef\@journalshort{Reports}\gdef\@doiabbr{reports}\gdef\@ISSN{2571-841X}}
\DeclareOption{reprodmed}{\gdef\@journal{reprodmed}\gdef\@journalfull{Reproductive Medicine}\gdef\@journalshort{Reprod. Med.}\gdef\@doiabbr{reprodmed}\gdef\@ISSN{2673-3897}\gdef\@continuouspages{yes}}
\DeclareOption{resources}{\gdef\@journal{resources}\gdef\@journalfull{Resources}\gdef\@journalshort{Resources}\gdef\@doiabbr{resources}\gdef\@ISSN{2079-9276}}
\DeclareOption{rheumato}{\gdef\@journal{rheumato}\gdef\@journalfull{Rheumato}\gdef\@journalshort{Rheumato}\gdef\@doiabbr{rheumato}\gdef\@ISSN{2674-0621}\gdef\@continuouspages{yes}}
\DeclareOption{risks}{\gdef\@journal{risks}\gdef\@journalfull{Risks}\gdef\@journalshort{Risks}\gdef\@doiabbr{risks}\gdef\@ISSN{2227-9091}}
\DeclareOption{robotics}{\gdef\@journal{robotics}\gdef\@journalfull{Robotics}\gdef\@journalshort{Robotics}\gdef\@doiabbr{robotics}\gdef\@ISSN{2218-6581}}
\DeclareOption{ruminants}{\gdef\@journal{ruminants}\gdef\@journalfull{Ruminants}\gdef\@journalshort{Ruminants}\gdef\@doiabbr{ruminants}\gdef\@ISSN{2673-933X}\gdef\@continuouspages{yes}}
\DeclareOption{safety}{\gdef\@journal{safety}\gdef\@journalfull{Safety}\gdef\@journalshort{Safety}\gdef\@doiabbr{safety}\gdef\@ISSN{2313-576X}}
\DeclareOption{sci}{\gdef\@journal{sci}\gdef\@journalfull{Sci}\gdef\@journalshort{Sci}\gdef\@doiabbr{sci}\gdef\@ISSN{2413-4155}}
\DeclareOption{scipharm}{\gdef\@journal{scipharm}\gdef\@journalfull{Scientia Pharmaceutica}\gdef\@journalshort{Sci. Pharm.}\gdef\@doiabbr{scipharm}\gdef\@ISSN{2218-0532}}
\DeclareOption{sclerosis}{\gdef\@journal{sclerosis}\gdef\@journalfull{Sclerosis}\gdef\@journalshort{Sclerosis}\gdef\@doiabbr{sclerosis}\gdef\@ISSN{2813-3064}\gdef\@continuouspages{yes}}
\DeclareOption{seeds}{\gdef\@journal{seeds}\gdef\@journalfull{Seeds}\gdef\@journalshort{Seeds}\gdef\@doiabbr{seeds}\gdef\@ISSN{2674-1024}\gdef\@continuouspages{yes}}
\DeclareOption{sensors}{\gdef\@journal{sensors}\gdef\@journalfull{Sensors}\gdef\@journalshort{Sensors}\gdef\@doiabbr{s}\gdef\@ISSN{1424-8220}}
\DeclareOption{separations}{\gdef\@journal{separations}\gdef\@journalfull{Separations}\gdef\@journalshort{Separations}\gdef\@doiabbr{separations}\gdef\@ISSN{2297-8739}}
\DeclareOption{sexes}{\gdef\@journal{sexes}\gdef\@journalfull{Sexes}\gdef\@journalshort{Sexes}\gdef\@doiabbr{sexes}\gdef\@ISSN{2411-5118}\gdef\@continuouspages{yes}}
\DeclareOption{signals}{\gdef\@journal{signals}\gdef\@journalfull{Signals}\gdef\@journalshort{Signals}\gdef\@doiabbr{signals}\gdef\@ISSN{2624-6120}\gdef\@continuouspages{yes}}
\DeclareOption{sinusitis}{\gdef\@journal{sinusitis}\gdef\@journalfull{Sinusitis}\gdef\@journalshort{Sinusitis}\gdef\@doiabbr{sinusitis}\gdef\@ISSN{2309-107X}\gdef\@continuouspages{yes}}
\DeclareOption{skins}{\gdef\@journal{skins}\gdef\@journalfull{Skins}\gdef\@journalshort{Skins}\gdef\@doiabbr{skins}\gdef\@ISSN{}}
\DeclareOption{smartcities}{\gdef\@journal{smartcities}\gdef\@journalfull{Smart Cities}\gdef\@journalshort{Smart Cities}\gdef\@doiabbr{smartcities}\gdef\@ISSN{2624-6511}\gdef\@continuouspages{yes}}
\DeclareOption{sna}{\gdef\@journal{sna}\gdef\@journalfull{Sinusitis and Asthma}\gdef\@journalshort{Sinusitis Asthma}\gdef\@doiabbr{sna}\gdef\@ISSN{2624-7003}}
\DeclareOption{societies}{\gdef\@journal{societies}\gdef\@journalfull{Societies}\gdef\@journalshort{Societies}\gdef\@doiabbr{soc}\gdef\@ISSN{2075-4698}}
\DeclareOption{socsci}{\gdef\@journal{socsci}\gdef\@journalfull{Social Sciences}\gdef\@journalshort{Soc. Sci.}\gdef\@doiabbr{socsci}\gdef\@ISSN{2076-0760}}
\DeclareOption{software}{\gdef\@journal{software}\gdef\@journalfull{Software}\gdef\@journalshort{Software}\gdef\@doiabbr{software}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{soilsystems}{\gdef\@journal{soilsystems}\gdef\@journalfull{Soil Systems}\gdef\@journalshort{Soil Syst.}\gdef\@doiabbr{soilsystems}\gdef\@ISSN{2571-8789}}
\DeclareOption{solar}{\gdef\@journal{solar}\gdef\@journalfull{Solar}\gdef\@journalshort{Solar}\gdef\@doiabbr{solar}\gdef\@ISSN{2673-9941}\gdef\@continuouspages{yes}}
\DeclareOption{solids}{\gdef\@journal{solids}\gdef\@journalfull{Solids}\gdef\@journalshort{Solids}\gdef\@doiabbr{solids}\gdef\@ISSN{2673-6497}\gdef\@continuouspages{yes}}
\DeclareOption{spectroscj}{\gdef\@journal{spectroscj}\gdef\@journalfull{Spectroscopy Journal}\gdef\@journalshort{Spectrosc. J.}\gdef\@doiabbr{spectroscj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{sports}{\gdef\@journal{sports}\gdef\@journalfull{Sports}\gdef\@journalshort{Sports}\gdef\@doiabbr{sports}\gdef\@ISSN{2075-4663}}
\DeclareOption{standards}{\gdef\@journal{standards}\gdef\@journalfull{Standards}\gdef\@journalshort{Standards}\gdef\@doiabbr{standards}\gdef\@ISSN{2305-6703}\gdef\@continuouspages{yes}}
\DeclareOption{stats}{\gdef\@journal{stats}\gdef\@journalfull{Stats}\gdef\@journalshort{Stats}\gdef\@doiabbr{stats}\gdef\@ISSN{2571-905X}\gdef\@continuouspages{yes}}
\DeclareOption{std}{\gdef\@journal{std}\gdef\@journalfull{Surgical Techniques Development}\gdef\@journalshort{Surg. Tech. Dev.}\gdef\@doiabbr{std}\gdef\@ISSN{2038-9582}\gdef\@continuouspages{yes}}
\DeclareOption{stresses}{\gdef\@journal{stresses}\gdef\@journalfull{Stresses}\gdef\@journalshort{Stresses}\gdef\@doiabbr{stresses}\gdef\@ISSN{2673-7140}\gdef\@continuouspages{yes}}
\DeclareOption{surfaces}{\gdef\@journal{surfaces}\gdef\@journalfull{Surfaces}\gdef\@journalshort{Surfaces}\gdef\@doiabbr{surfaces}\gdef\@ISSN{2571-9637}\gdef\@continuouspages{yes}}
\DeclareOption{surgeries}{\gdef\@journal{surgeries}\gdef\@journalfull{Surgeries}\gdef\@journalshort{Surgeries}\gdef\@doiabbr{surgeries}\gdef\@ISSN{2017-2017}\gdef\@continuouspages{yes}}
\DeclareOption{suschem}{\gdef\@journal{suschem}\gdef\@journalfull{Sustainable Chemistry}\gdef\@journalshort{Sustain. Chem.}\gdef\@doiabbr{suschem}\gdef\@ISSN{2673-4079}\gdef\@continuouspages{yes}}
\DeclareOption{sustainability}{\gdef\@journal{sustainability}\gdef\@journalfull{Sustainability}\gdef\@journalshort{Sustainability}\gdef\@doiabbr{su}\gdef\@ISSN{2071-1050}}
\DeclareOption{symmetry}{\gdef\@journal{symmetry}\gdef\@journalfull{Symmetry}\gdef\@journalshort{Symmetry}\gdef\@doiabbr{sym}\gdef\@ISSN{2073-8994}}
\DeclareOption{synbio}{\gdef\@journal{synbio}\gdef\@journalfull{Synbio}\gdef\@journalshort{Synbio}\gdef\@doiabbr{synbio}\gdef\@ISSN{2674-0583}\gdef\@continuouspages{yes}}
\DeclareOption{systems}{\gdef\@journal{systems}\gdef\@journalfull{Systems}\gdef\@journalshort{Systems}\gdef\@doiabbr{systems}\gdef\@ISSN{2079-8954}}
\DeclareOption{targets}{\gdef\@journal{targets}\gdef\@journalfull{Targets}\gdef\@journalshort{Targets}\gdef\@doiabbr{targets}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{taxonomy}{\gdef\@journal{taxonomy}\gdef\@journalfull{Taxonomy}\gdef\@journalshort{Taxonomy}\gdef\@doiabbr{taxonomy}\gdef\@ISSN{2673-6500}\gdef\@continuouspages{yes}}
\DeclareOption{technologies}{\gdef\@journal{technologies}\gdef\@journalfull{Technologies}\gdef\@journalshort{Technologies}\gdef\@doiabbr{technologies}\gdef\@ISSN{2227-7080}}
\DeclareOption{telecom}{\gdef\@journal{telecom}\gdef\@journalfull{Telecom}\gdef\@journalshort{Telecom}\gdef\@doiabbr{telecom}\gdef\@ISSN{2673-4001}\gdef\@continuouspages{yes}}
\DeclareOption{test}{\gdef\@journal{test}\gdef\@journalfull{Test}\gdef\@journalshort{Test}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{textiles}{\gdef\@journal{textiles}\gdef\@journalfull{Textiles}\gdef\@journalshort{Textiles}\gdef\@doiabbr{textiles}\gdef\@ISSN{2673-7248}\gdef\@continuouspages{yes}}
\DeclareOption{thalassrep}{\gdef\@journal{thalassrep}\gdef\@journalfull{Thalassemia Reports}\gdef\@journalshort{Thalass. Rep.}\gdef\@doiabbr{thalassrep}\gdef\@ISSN{2039-4365}\gdef\@continuouspages{yes}}
\DeclareOption{thermo}{\gdef\@journal{thermo}\gdef\@journalfull{Thermo}\gdef\@journalshort{Thermo}\gdef\@doiabbr{thermo}\gdef\@ISSN{2673-7264}\gdef\@continuouspages{yes}}
\DeclareOption{tomography}{\gdef\@journal{tomography}\gdef\@journalfull{Tomography}\gdef\@journalshort{Tomography}\gdef\@doiabbr{tomography}\gdef\@ISSN{2379-139X}\gdef\@continuouspages{yes}}
\DeclareOption{tourismhosp}{\gdef\@journal{tourismhosp}\gdef\@journalfull{Tourism and Hospitality}\gdef\@journalshort{Tour. Hosp.}\gdef\@doiabbr{tourhosp}\gdef\@ISSN{2673-5768}\gdef\@continuouspages{yes}}
\DeclareOption{toxics}{\gdef\@journal{toxics}\gdef\@journalfull{Toxics}\gdef\@journalshort{Toxics}\gdef\@doiabbr{toxics}\gdef\@ISSN{2305-6304}}
\DeclareOption{toxins}{\gdef\@journal{toxins}\gdef\@journalfull{Toxins}\gdef\@journalshort{Toxins}\gdef\@doiabbr{toxins}\gdef\@ISSN{2072-6651}}
\DeclareOption{transplantology}{\gdef\@journal{transplantology}\gdef\@journalfull{Transplantology}\gdef\@journalshort{Transplantology}\gdef\@doiabbr{transplantology}\gdef\@ISSN{2673-3943}\gdef\@continuouspages{yes}}
\DeclareOption{transportation}{\gdef\@journal{transportation}\gdef\@journalfull{Transportation}\gdef\@journalshort{Transportation}\gdef\@doiabbr{transportation}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{traumacare}{\gdef\@journal{traumacare}\gdef\@journalfull{Trauma Care}\gdef\@journalshort{Trauma Care}\gdef\@doiabbr{traumacare}\gdef\@ISSN{2673-866X}\gdef\@continuouspages{yes}}
\DeclareOption{traumas}{\gdef\@journal{traumas}\gdef\@journalfull{Traumas}\gdef\@journalshort{Traumas}\gdef\@doiabbr{traumas}\gdef\@ISSN{2673-7477}\gdef\@continuouspages{yes}}
\DeclareOption{tropicalmed}{\gdef\@journal{tropicalmed}\gdef\@journalfull{Tropical Medicine and Infectious Disease}\gdef\@journalshort{Trop. Med. Infect. Dis.}\gdef\@doiabbr{tropicalmed}\gdef\@ISSN{2414-6366}}
\DeclareOption{universe}{\gdef\@journal{universe}\gdef\@journalfull{Universe}\gdef\@journalshort{Universe}\gdef\@doiabbr{universe}\gdef\@ISSN{2218-1997}}
\DeclareOption{urbansci}{\gdef\@journal{urbansci}\gdef\@journalfull{Urban Science}\gdef\@journalshort{Urban Sci.}\gdef\@doiabbr{urbansci}\gdef\@ISSN{2413-8851}}
\DeclareOption{uro}{\gdef\@journal{uro}\gdef\@journalfull{Uro}\gdef\@journalshort{Uro}\gdef\@doiabbr{uro}\gdef\@ISSN{2673-4397}\gdef\@continuouspages{yes}}
\DeclareOption{vaccines}{\gdef\@journal{vaccines}\gdef\@journalfull{Vaccines}\gdef\@journalshort{Vaccines}\gdef\@doiabbr{vaccines}\gdef\@ISSN{2076-393X}}
\DeclareOption{vehicles}{\gdef\@journal{vehicles}\gdef\@journalfull{Vehicles}\gdef\@journalshort{Vehicles}\gdef\@doiabbr{vehicles}\gdef\@ISSN{2624-8921}\gdef\@continuouspages{yes}}
\DeclareOption{venereology}{\gdef\@journal{venereology}\gdef\@journalfull{Venereology}\gdef\@journalshort{Venereology}\gdef\@doiabbr{venereology}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{vetsci}{\gdef\@journal{vetsci}\gdef\@journalfull{Veterinary Sciences}\gdef\@journalshort{Vet. Sci.}\gdef\@doiabbr{vetsci}\gdef\@ISSN{2306-7381}}
\DeclareOption{vibration}{\gdef\@journal{vibration}\gdef\@journalfull{Vibration}\gdef\@journalshort{Vibration}\gdef\@doiabbr{vibration}\gdef\@ISSN{2571-631X}\gdef\@continuouspages{yes}}
\DeclareOption{virtualworlds}{\gdef\@journal{virtualworlds}\gdef\@journalfull{Virtual Worlds}\gdef\@journalshort{Virtual Worlds}\gdef\@doiabbr{virtualworlds}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{viruses}{\gdef\@journal{viruses}\gdef\@journalfull{Viruses}\gdef\@journalshort{Viruses}\gdef\@doiabbr{v}\gdef\@ISSN{1999-4915}}
\DeclareOption{vision}{\gdef\@journal{vision}\gdef\@journalfull{Vision}\gdef\@journalshort{Vision}\gdef\@doiabbr{vision}\gdef\@ISSN{2411-5150}}
\DeclareOption{waste}{\gdef\@journal{waste}\gdef\@journalfull{Waste}\gdef\@journalshort{Waste}\gdef\@doiabbr{waste}\gdef\@ISSN{2813-0391}\gdef\@continuouspages{yes}}
\DeclareOption{water}{\gdef\@journal{water}\gdef\@journalfull{Water}\gdef\@journalshort{Water}\gdef\@doiabbr{w}\gdef\@ISSN{2073-4441}}
\DeclareOption{wem}{\gdef\@journal{wem}\gdef\@journalfull{Wildlife Ecology and Management}\gdef\@journalshort{Wildl. Ecol. Manag.}\gdef\@doiabbr{}\gdef\@ISSN{1234-4321}}
\DeclareOption{wevj}{\gdef\@journal{wevj}\gdef\@journalfull{World Electric Vehicle Journal}\gdef\@journalshort{World Electr. Veh. J.}\gdef\@doiabbr{wevj}\gdef\@ISSN{2032-6653}}
\DeclareOption{wind}{\gdef\@journal{wind}\gdef\@journalfull{Wind}\gdef\@journalshort{Wind}\gdef\@doiabbr{wind}\gdef\@ISSN{2674-032X}\gdef\@continuouspages{yes}}
\DeclareOption{women}{\gdef\@journal{women}\gdef\@journalfull{Women}\gdef\@journalshort{Women}\gdef\@doiabbr{women}\gdef\@ISSN{2673-4184}\gdef\@continuouspages{yes}}
\DeclareOption{world}{\gdef\@journal{world}\gdef\@journalfull{World}\gdef\@journalshort{World}\gdef\@doiabbr{world}\gdef\@ISSN{2673-4060}\gdef\@continuouspages{yes}}
\DeclareOption{youth}{\gdef\@journal{youth}\gdef\@journalfull{Youth}\gdef\@journalshort{Youth}\gdef\@doiabbr{youth}\gdef\@ISSN{2673-995X}\gdef\@continuouspages{yes}}
\DeclareOption{zoonoticdis}{\gdef\@journal{zoonoticdis}\gdef\@journalfull{Zoonotic Diseases}\gdef\@journalshort{Zoonotic Dis.}\gdef\@doiabbr{zoonoticdis}\gdef\@ISSN{2813-0227}\gdef\@continuouspages{yes}}

